The Conflict Graph Design: Estimating Causal Effects under Arbitrary Neighborhood Interference

A fundamental problem in network experiments is selecting an appropriate experimental design in order to precisely estimate a given causal effect of interest. In this work, we propose the Conflict Graph Design, a general approach for constructing experiment designs under network interference with the goal of precisely estimating a pre-specified causal effect. A central aspect of our approach is the notion of a conflict graph, which captures the fundamental unobservability associated with the causal effect and the underlying network. In order to estimate effects, we propose a modified Horvitz--Thompson estimator. We show that its variance under the Conflict Graph Design is bounded as $O(\lambda(H) / n )$, where $\lambda(H)$ is the largest eigenvalue of the adjacency matrix of the conflict graph. These rates depend on both the underlying network and the particular causal effect under investigation. Not only does this yield the best known rates of estimation for several well-studied causal effects (e.g. the global and direct effects) but it also provides new methods for effects which have received less attention from the perspective of experiment design (e.g. spill-over effects). Finally, we construct conservative variance estimators which facilitate asymptotically valid confidence intervals for the causal effect of interest.

==> figs/docs/0b1c0124-1924-42a2-b7a2-3b8cbcde18de <==
{"id":"r0.17310102553932827","lines":[{"id":"n0.5679499344061233","blocks":[]},{"id":"n0.558178959968983","blocks":[{"id":"n0.6001033734294505","text":"\\diagram","type":"composite","elements":{"de9095049321079307":{"id":"de9095049321079307","lines":[{"id":"n0.37847194557334873","blocks":[{"id":"n0.8173616299020627","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.2642474183020651","lines":[{"id":"n0.05274577397326374","blocks":[{"id":"n0.9903399949049001","text":"C"},{"id":"n0.22154638325913623","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.4027203507400057","lines":[{"id":"n0.10662952293171579","blocks":[{"id":"n0.02680898275355359","text":"1"}]}]}}}]}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"}}]}],"shape":{"data":{"p":{"x":16.5,"y":43.25}},"anchor":"left-top"},"isTextMode":true},"de2077433695074975":{"id":"de2077433695074975","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"C","id":"n0.5485033548075537"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.7779374190942374","text":"2"}],"id":"n0.3879917036651874"}],"id":"n0.30632466847757245"}},"id":"n0.161918749774689"}],"id":"n0.5885664465407561"}],"id":"n0.15660769854893397"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.8542675245737628"}],"id":"n0.37257011876238155"}],"shape":{"data":{"p":{"x":259,"y":41.75}},"anchor":"left-top"},"isTextMode":true},"de6886895542736242":{"id":"de6886895542736242","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"C","id":"n0.2655527650752849"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.602496383561339","text":"4"}],"id":"n0.9518200929480298"}],"id":"n0.7382691363478728"}},"id":"n0.5282750689530624"}],"id":"n0.7109956083693325"}],"id":"n0.5891824550535028"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.12261274443332293"}],"id":"n0.10729450860667655"}],"shape":{"data":{"p":{"x":17,"y":155.25}},"anchor":"left-top"},"isTextMode":true},"de23372261396630467":{"id":"de23372261396630467","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"C","id":"n0.09739356781894615"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.1863678456142197","text":"3"}],"id":"n0.8504737051847631"}],"id":"n0.715234299564669"}},"id":"n0.5916216636606122"}],"id":"n0.1412243450709818"}],"id":"n0.850004007476445"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.7609185275894892"}],"id":"n0.6043633827463295"}],"shape":{"data":{"p":{"x":260,"y":154.25}},"anchor":"left-top"},"isTextMode":true},"de7640294852788863":{"id":"de7640294852788863","lines":[{"id":"n0.39021212770707026","blocks":[{"id":"n0.6051019216866516","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.4687652084741485","lines":[{"id":"n0.30983372671147924","blocks":[{"id":"n0.9276240837071414","text":"r"},{"id":"n0.039225829037397686","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.7794322936368345","lines":[{"id":"n0.3670397477478393","blocks":[{"id":"n0.10610570199000557","text":"1"}]}]}}}]}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"}}]}],"shape":{"data":{"p":{"x":97.5,"y":63.25}},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true},"de7190152160930616":{"id":"de7190152160930616","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"r","id":"n0.21903927309540738"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"2","id":"n0.6733394728781099"}],"id":"n0.3127919382527904"}],"id":"n0.94237542778707"}},"id":"n0.4610064919862735"}],"id":"n0.7145959106157325"}],"id":"n0.46720787484409043"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.6586609379943333"}],"id":"n0.8582496664944308"}],"shape":{"data":{"p":{"x":189.5,"y":63.75}},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true},"de2876742192960988":{"id":"de2876742192960988","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"r","id":"n0.5270148040186657"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.2821744437906557","text":"3"}],"id":"n0.37458706505884365"}],"id":"n0.25361256503732"}},"id":"n0.9263031683602103"}],"id":"n0.31558516389168845"}],"id":"n0.9433409332242515"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.3831540065053469"}],"id":"n0.4152961937802164"}],"shape":{"data":{"p":{"x":189.5,"y":142.25}},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true},"de48315637169260817":{"id":"de48315637169260817","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"r","id":"n0.0034840555786561644"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.9729448651073798","text":"4"}],"id":"n0.4198732633483506"}],"id":"n0.04679790772268522"}},"id":"n0.5794761922555758"}],"id":"n0.40804362147372664"}],"id":"n0.10467993043349821"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.40442276987914205"}],"id":"n0.48283994517866313"}],"shape":{"data":{"p":{"x":97.5,"y":142.75}},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true}},"connections":[],"intersections":{"id":"di3676895024823952","items":[],"style":{}},"shapes":[{"id":"dp7718081377411163","type":"circle","data":{"p1":{"x":48,"y":19},"p2":{"x":123.5,"y":94.5}},"style":{"fillColor":[74,144,226,0.3],"strokeColor":"none"}},{"id":"dp33530477615229337","type":"circle","data":{"p1":{"x":49,"y":130.25},"p2":{"x":124.5,"y":205.75}},"style":{"fillColor":[74,144,226,0.3],"strokeColor":"none"}},{"id":"dp3491562982174694","type":"circle","data":{"p1":{"x":177,"y":130.25},"p2":{"x":252.5,"y":205.75}},"style":{"fillColor":[74,144,226,0.3],"strokeColor":"none"}},{"id":"dp22190782097635608","type":"circle","data":{"p1":{"x":176,"y":19},"p2":{"x":251.5,"y":94.5}},"style":{"fillColor":[74,144,226,0.3],"strokeColor":"none"}},{"id":"dg976553834096884","entities":[{"id":"dg8345616249547039","entities":[{"id":"dp9709813475701714","type":"circle","data":{"p1":{"x":59.75876777251196,"y":33.40063191153247},"p2":{"x":77.07630331753566,"y":50.71816745655617},"flipX":true},"style":{"thickness":2}},{"id":"dp9033594651891632","type":"circle","data":{"p1":{"x":59.75876777251196,"y":64.06729857819913},"p2":{"x":77.07630331753566,"y":81.38483412322284},"flipX":true},"style":{"thickness":2}},{"id":"dp406680639739734","type":"circle","data":{"p1":{"x":95.0921011058453,"y":33.40063191153247},"p2":{"x":112.409636650869,"y":50.71816745655617},"flipX":true},"style":{"thickness":2}},{"id":"dp8874766139474939","type":"circle","data":{"p1":{"x":95.0921011058453,"y":64.06729857819913},"p2":{"x":112.409636650869,"y":81.38483412322284},"flipX":true},"style":{"thickness":2}}]},{"id":"da8389243520195597","data":[{"x":68.41753554502381,"y":50.71816745655617},{"x":68.41753554502381,"y":64.06729857819914}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da6543772988428556","data":[{"x":77.07630331753566,"y":42.05939968404432},{"x":95.0921011058453,"y":42.05939968404432}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da6130380545342651","data":[{"x":77.07630331753566,"y":72.726066350711},{"x":95.0921011058453,"y":72.726066350711}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da969558600865803","data":[{"x":103.75086887835715,"y":50.71816745655617},{"x":103.75086887835715,"y":64.06729857819914}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da9083632251170299","data":[{"x":74.5,"y":47},{"x":97,"y":66.5}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da636995995265601","data":[{"x":97.5,"y":48.5},{"x":76,"y":67.5}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}}]},{"id":"dg6134669029365414","entities":[{"id":"dg12260249772547338","entities":[{"id":"dp6082018087754177","type":"circle","data":{"p1":{"x":59.75876777251196,"y":143.40063191153246},"p2":{"x":77.07630331753566,"y":160.71816745655616},"flipX":true},"style":{"thickness":2}},{"id":"dp9189998430996205","type":"circle","data":{"p1":{"x":59.75876777251196,"y":174.06729857819914},"p2":{"x":77.07630331753566,"y":191.38483412322284},"flipX":true},"style":{"thickness":2}},{"id":"dp5032608435231252","type":"circle","data":{"p1":{"x":95.0921011058453,"y":143.40063191153246},"p2":{"x":112.409636650869,"y":160.71816745655616},"flipX":true},"style":{"thickness":2}},{"id":"dp035041736174051596","type":"circle","data":{"p1":{"x":95.0921011058453,"y":174.06729857819914},"p2":{"x":112.409636650869,"y":191.38483412322284},"flipX":true},"style":{"thickness":2}}]},{"id":"da5324423314953974","data":[{"x":68.41753554502381,"y":160.71816745655616},{"x":68.41753554502381,"y":174.06729857819914}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da9355577748332022","data":[{"x":77.07630331753566,"y":152.0593996840443},{"x":95.0921011058453,"y":152.0593996840443}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da3811258107304456","data":[{"x":77.07630331753566,"y":182.726066350711},{"x":95.0921011058453,"y":182.726066350711}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da963609870869996","data":[{"x":103.75086887835715,"y":160.71816745655616},{"x":103.75086887835715,"y":174.06729857819914}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da8969172773108889","data":[{"x":74.5,"y":157},{"x":97,"y":176.5}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da9961047080355627","data":[{"x":97.5,"y":158.5},{"x":76,"y":177.5}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}}]},{"id":"dg10426482983372698","entities":[{"id":"dg6917905431930886","entities":[{"id":"dp9336242795537251","type":"circle","data":{"p1":{"x":187.758767772512,"y":33.40063191153247},"p2":{"x":205.0763033175357,"y":50.71816745655617},"flipX":true},"style":{"thickness":2}},{"id":"dp3603526364805869","type":"circle","data":{"p1":{"x":187.758767772512,"y":64.06729857819914},"p2":{"x":205.0763033175357,"y":81.38483412322284},"flipX":true},"style":{"thickness":2}},{"id":"dp6957147127688437","type":"circle","data":{"p1":{"x":223.0921011058453,"y":33.40063191153247},"p2":{"x":240.409636650869,"y":50.71816745655617},"flipX":true},"style":{"thickness":2}},{"id":"dp5745338736606542","type":"circle","data":{"p1":{"x":223.0921011058453,"y":64.06729857819914},"p2":{"x":240.409636650869,"y":81.38483412322284},"flipX":true},"style":{"thickness":2}}]},{"id":"da2927675158373184","data":[{"x":196.41753554502384,"y":50.71816745655617},{"x":196.41753554502384,"y":64.06729857819914}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da8810462022269949","data":[{"x":205.0763033175357,"y":42.05939968404432},{"x":223.0921011058453,"y":42.05939968404432}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da23688216128160633","data":[{"x":205.0763033175357,"y":72.726066350711},{"x":223.0921011058453,"y":72.726066350711}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da07591579029241546","data":[{"x":231.75086887835715,"y":50.71816745655617},{"x":231.75086887835715,"y":64.06729857819914}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da09945478604402935","data":[{"x":202.5,"y":47},{"x":225,"y":66.5}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da47399812345449344","data":[{"x":225.5,"y":48.5},{"x":204,"y":67.5}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}}]},{"id":"dg009351889488404597","entities":[{"id":"dg8514800717547131","entities":[{"id":"dp7047205304549833","type":"circle","data":{"p1":{"x":187.758767772512,"y":143.40063191153246},"p2":{"x":205.0763033175357,"y":160.71816745655616},"flipX":true},"style":{"thickness":2}},{"id":"dp08131426259067731","type":"circle","data":{"p1":{"x":187.758767772512,"y":174.06729857819914},"p2":{"x":205.0763033175357,"y":191.38483412322284},"flipX":true},"style":{"thickness":2}},{"id":"dp7176481592724147","type":"circle","data":{"p1":{"x":223.0921011058453,"y":143.40063191153246},"p2":{"x":240.409636650869,"y":160.71816745655616},"flipX":true},"style":{"thickness":2}},{"id":"dp14323836928426403","type":"circle","data":{"p1":{"x":223.0921011058453,"y":174.06729857819914},"p2":{"x":240.409636650869,"y":191.38483412322284},"flipX":true},"style":{"thickness":2}}]},{"id":"da41697811784221495","data":[{"x":196.41753554502384,"y":160.71816745655616},{"x":196.41753554502384,"y":174.06729857819914}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da5095997808408614","data":[{"x":205.0763033175357,"y":152.0593996840443},{"x":223.0921011058453,"y":152.0593996840443}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da6941135346335912","data":[{"x":205.0763033175357,"y":182.726066350711},{"x":223.0921011058453,"y":182.726066350711}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da44012037079652355","data":[{"x":231.75086887835715,"y":160.71816745655616},{"x":231.75086887835715,"y":174.06729857819914}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da9372241715743355","data":[{"x":202.5,"y":157},{"x":225,"y":176.5}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da8071289443871157","data":[{"x":225.5,"y":158.5},{"x":204,"y":177.5}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}}]},{"id":"da8263323339964819","data":[{"x":103.75086887835715,"y":81.38483412322284},{"x":103.75086887835715,"y":143.40063191153246}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da2144727057794753","data":[{"x":196.41753554502384,"y":81.38483412322284},{"x":196.41753554502384,"y":143.40063191153246}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da5596420020088526","data":[{"x":187.758767772512,"y":152.0593996840443},{"x":112.409636650869,"y":152.0593996840443}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da174208713446784","data":[{"x":187.758767772512,"y":72.726066350711},{"x":112.409636650869,"y":72.726066350711}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da6808188924630594","data":[{"x":190.5,"y":79},{"x":111,"y":146.5}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da4501801251790132","data":[{"x":110,"y":78},{"x":189.5,"y":146}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}}],"settings":{"grid":true}}]},{"id":"n0.6795144576834875","blocks":[],"style":null}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":251,"delayRenderCache":{"av":251,"map":{}}}

==> figs/docs/10076752-dc0a-4e00-a18f-3f8d6cc0b166 <==
{"id":"r0.08279460460498611","lines":[{"blocks":[{"text":"\\diagram","type":"composite","elements":{"de7871344337073147":{"id":"de7871344337073147","lines":[{"id":"n0.2723732373579588","blocks":[{"id":"n0.3899629754209666","text":"1"}]}],"shape":{"data":{"p":{"x":128.8643076797487,"y":153.30550394860256},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de4499113424059924":{"id":"de4499113424059924","lines":[{"blocks":[{"id":"n0.49044887366233647","text":"2"}],"id":"n0.41069676726116633"}],"shape":{"data":{"p":{"x":65.72367457392377,"y":60.256149897913346},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de2086775955506217":{"id":"de2086775955506217","lines":[{"blocks":[{"id":"n0.3519131667224691","text":"3"}],"id":"n0.8770032501598126"}],"shape":{"data":{"p":{"x":66.83140497928915,"y":256.32443164757996},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de7160414597950548":{"id":"de7160414597950548","lines":[{"blocks":[{"id":"n0.04563187760035525","text":"4"}],"id":"n0.7683514386481154"}],"shape":{"data":{"p":{"x":240.7450786216489,"y":54.71749787108662},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de7599504377955328":{"id":"de7599504377955328","lines":[{"blocks":[{"id":"n0.8872729056160837","text":"5"}],"id":"n0.09947692202455904"}],"shape":{"data":{"p":{"x":347.0871975367224,"y":145.55139111104518},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de17372933674316915":{"id":"de17372933674316915","lines":[{"blocks":[{"id":"n0.7646766119457067","text":"6"}],"id":"n0.02054469361661626"}],"shape":{"data":{"p":{"x":251.82238267530238,"y":245.24712759392654},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de3364084417588762":{"id":"de3364084417588762","lines":[{"blocks":[{"id":"n0.39970054743847916","text":"7"}],"id":"n0.8439301330962781"}],"shape":{"data":{"p":{"x":357.0567711850105,"y":296.2027262407325},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de5444591295012495":{"id":"de5444591295012495","lines":[{"id":"n0.4580006466033084","blocks":[{"id":"n0.004323116628885071","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.05583984904491435","lines":[{"id":"n0.44617432235220433","blocks":[{"text":"*","id":"n0.43338586099986753"}]}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"}}]}],"shape":{"data":{"p":{"x":127.33333333333331,"y":111.66666666666667}},"anchor":"left-top"},"isTextMode":true},"de802548674203766":{"id":"de802548674203766","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"*","id":"n0.9896969648167333"}],"id":"n0.3817875254865164"}],"id":"n0.051945564365197594"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.49399794010615783"}],"id":"n0.5374551986687637"}],"shape":{"data":{"p":{"x":66,"y":21.00000000000003}},"anchor":"left-top"},"isTextMode":true},"de27989278411412255":{"id":"de27989278411412255","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"e","id":"n0.8245846062169784"},{"id":"n0.04997805708594316","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.2664237119361701","lines":[{"id":"n0.13708560723019203","blocks":[{"id":"n0.28192195296787115","text":"1"}]}]}}}],"id":"n0.09448578603405733"}],"id":"n0.463838270242938"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.19972447943144744"}],"id":"n0.678015697771936"}],"shape":{"data":{"p":{"x":62,"y":297}},"anchor":"left-top","style":{"textColor":[247,31,31,1]}},"isTextMode":true},"de06696423087419645":{"id":"de06696423087419645","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"e","id":"n0.26444588881987285"},{"id":"n0.8069736513330608","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.05423249802915042","lines":[{"id":"n0.5592081902429427","blocks":[{"id":"n0.096192776191653","text":"0"}]}]}}}],"id":"n0.5203841070997659"}],"id":"n0.788862846109518"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.12799649499589982"}],"id":"n0.6217812849716962"}],"shape":{"data":{"p":{"x":238.33333333333334,"y":13.333333333333329}},"anchor":"left-top","style":{"textColor":[70,114,191,1]}},"isTextMode":true},"de5155124881847579":{"id":"de5155124881847579","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"*","id":"n0.38592678252046775"}],"id":"n0.613570980544254"}],"id":"n0.11508231035356742"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.11487753551802671"}],"id":"n0.6880967245552836"}],"shape":{"data":{"p":{"x":252.33333333333334,"y":282.66666666666663}},"anchor":"left-top"},"isTextMode":true},"de7809523776931049":{"id":"de7809523776931049","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"e","id":"n0.835245197708119"},{"id":"n0.8387877215078927","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.18073888371384506","lines":[{"id":"n0.025065779025482238","blocks":[{"id":"n0.1592803993990597","text":"1"}]}]}}}],"id":"n0.4565799495373377"}],"id":"n0.5839332056122035"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.9387918793546755"}],"id":"n0.41917277053077173"}],"shape":{"data":{"p":{"x":385.33333333333337,"y":143}},"anchor":"left-top","style":{"textColor":[247,31,31,1]}},"isTextMode":true},"de776647850708468":{"id":"de776647850708468","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"e","id":"n0.8467124494269882"},{"id":"n0.6084882383200159","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.25361597395188995","lines":[{"id":"n0.9342898372650021","blocks":[{"id":"n0.5484125663648771","text":"0"}]}]}}}],"id":"n0.03832700159051039"}],"id":"n0.663229180295934"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.2999014764803336"}],"id":"n0.8347610462180917"}],"shape":{"data":{"p":{"x":399.3333333333333,"y":294.99999999999994}},"anchor":"left-top","style":{"textColor":[70,114,191,1]}},"isTextMode":true}},"connections":[],"intersections":{"id":"di018738070182718003","items":[],"style":{}},"shapes":[{"id":"dp9194809774217807","type":"ellipse","data":{"p1":{"x":44.95402865523873,"y":42.85625299199422},"p2":{"x":100.49332049260892,"y":98.39554482936434}},"style":{"fillColor":"none"}},{"id":"dp39619755819664215","type":"ellipse","data":{"p1":{"x":45.52895517377332,"y":238.64630089431083},"p2":{"x":101.06824701114326,"y":294.1855927316803},"rotation":12.59},"style":{"fillColor":"none"}},{"id":"dp4361293174593055","type":"ellipse","data":{"p1":{"x":108.38664482631847,"y":135.74529364125738},"p2":{"x":163.92593666368901,"y":191.28458547862738},"rotation":11.34},"style":{"fillColor":[255,255,255,1]}},{"id":"dp5813278696059392","type":"ellipse","data":{"p1":{"x":336.79390961187244,"y":278.949097787917},"p2":{"x":392.33320144924306,"y":334.4883896252872},"rotation":1.24},"style":{"fillColor":"none"}},{"id":"dp8630472605711585","type":"ellipse","data":{"p1":{"x":231.22913809978522,"y":228.00619298050708},"p2":{"x":286.7684299371551,"y":283.5454848178769},"rotation":312.14},"style":{"fillColor":"none"}},{"id":"dp5262498625545986","type":"ellipse","data":{"p1":{"x":219.72524418472122,"y":37.96336472513116},"p2":{"x":275.26453602209136,"y":93.50265656250127}},"style":{"fillColor":"none"}},{"id":"dp7700773027809327","type":"ellipse","data":{"p1":{"x":325.31306594751015,"y":128.5497234540565},"p2":{"x":380.85235778488016,"y":184.0890152914266}},"style":{"fillColor":"none"}},{"id":"da001887233869708238","data":[{"x":66.0772921417317,"y":239.0773063107636},{"x":66.0772921417317,"y":97.28781442399901}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da11768708912263026","data":[{"x":120.3560820046338,"y":185.9062468532269},{"x":91.55509146513478,"y":245.7236887429557}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da07772422476887186","data":[{"x":87.12416984367336,"y":95.07235361326829},{"x":119.24835159926843,"y":142.7047610439783}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da2756115548754525","data":[{"x":359.62584956354925,"y":183.69078604249617},{"x":365.16450159037583,"y":278.9556009039161}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da19358377386624337","data":[{"x":149.15707254413283,"y":139.38156982788226},{"x":220.05181848751522,"y":72.91774550596136}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da14095226818886486","data":[{"x":275.4383387557826,"y":71.81001510059599},{"x":346.33308469916494,"y":129.4119961795941}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da752496222602268","data":[{"x":284.854047201388,"y":244.06209313490763},{"x":341.3482978750208,"y":180.92146002908285}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da9399128054077954","data":[{"x":158.57278098973836,"y":180.92146002908285},{"x":233.34458335189936,"y":244.06209313490763}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}}],"settings":{"grid":true,"diagramHeight":358.6640625},"id":"n0.8747205658874042"}],"id":"n0.30715207840350955"}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":176,"delayRenderCache":{"av":176,"map":{}}}

==> figs/docs/11d0505f-9063-4971-8769-566f082712a4 <==
{"id":"r0.3119784670515864","lines":[{"blocks":[{"text":"\\diagram","type":"composite","elements":{"de4281339955977923":{"id":"de4281339955977923","lines":[{"blocks":[{"text":"5","id":"n0.5344102028134672"}],"id":"n0.0982244435109405"}],"shape":{"data":{"p":{"x":128.8643076797487,"y":153.30550394860256},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de8405484805657062":{"id":"de8405484805657062","lines":[{"blocks":[{"text":"2","id":"n0.3902860814771909"}],"id":"n0.6078387356094048"}],"shape":{"data":{"p":{"x":65.72367457392377,"y":60.256149897913346},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de4789488018288992":{"id":"de4789488018288992","lines":[{"blocks":[{"text":"4","id":"n0.29362102753722286"}],"id":"n0.7910332801706008"}],"shape":{"data":{"p":{"x":66.83140497928915,"y":256.32443164757996},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de9613955447787148":{"id":"de9613955447787148","lines":[{"blocks":[{"text":"1","id":"n0.6623865553301433"}],"id":"n0.2805988959851755"}],"shape":{"data":{"p":{"x":240.7450786216489,"y":54.71749787108662},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de8630035298118479":{"id":"de8630035298118479","lines":[{"blocks":[{"text":"6","id":"n0.48052139080478184"}],"id":"n0.6003045614265143"}],"shape":{"data":{"p":{"x":347.0871975367224,"y":145.55139111104518},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de870067710200805":{"id":"de870067710200805","lines":[{"blocks":[{"text":"3","id":"n0.6033051576755062"}],"id":"n0.915354718241514"}],"shape":{"data":{"p":{"x":251.82238267530238,"y":245.24712759392654},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de4656668256011238":{"id":"de4656668256011238","lines":[{"blocks":[{"text":"7","id":"n0.27010490978724544"}],"id":"n0.3622127714490513"}],"shape":{"data":{"p":{"x":357.0567711850105,"y":296.2027262407325},"rotation":0},"anchor":"left-top"},"isTextMode":true}},"connections":[],"intersections":{"id":"di018738070182718003","items":[],"style":{}},"shapes":[{"id":"dp4409369659318194","type":"ellipse","data":{"p1":{"x":44.95402865523873,"y":42.85625299199422},"p2":{"x":100.49332049260892,"y":98.39554482936434}},"style":{"fillColor":[247,31,31,1]}},{"id":"dp42703326137044106","type":"ellipse","data":{"p1":{"x":45.52895517377332,"y":238.64630089431083},"p2":{"x":101.06824701114326,"y":294.1855927316803},"rotation":12.59},"style":{"fillColor":[247,31,31,1]}},{"id":"dp9226781062454623","type":"ellipse","data":{"p1":{"x":108.38664482631847,"y":135.74529364125738},"p2":{"x":163.92593666368901,"y":191.28458547862738},"rotation":11.34},"style":{"fillColor":[247,31,31,1]}},{"id":"dp9234520704516664","type":"ellipse","data":{"p1":{"x":336.79390961187244,"y":278.949097787917},"p2":{"x":392.33320144924306,"y":334.4883896252872},"rotation":1.24},"style":{"fillColor":[70,114,191,1]}},{"id":"dp3183470150339327","type":"ellipse","data":{"p1":{"x":231.22913809978522,"y":228.00619298050708},"p2":{"x":286.7684299371551,"y":283.5454848178769},"rotation":312.14},"style":{"fillColor":[70,114,191,1]}},{"id":"dp47376010022778847","type":"ellipse","data":{"p1":{"x":219.72524418472122,"y":37.96336472513116},"p2":{"x":275.26453602209136,"y":93.50265656250127}},"style":{"fillColor":[70,114,191,1]}},{"id":"dp33559197088136594","type":"ellipse","data":{"p1":{"x":325.31306594751015,"y":128.5497234540565},"p2":{"x":380.85235778488016,"y":184.0890152914266}},"style":{"fillColor":[70,114,191,1]}},{"id":"da6056666037437448","data":[{"x":66.0772921417317,"y":239.0773063107636},{"x":66.0772921417317,"y":97.28781442399901}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da02644929668289331","data":[{"x":120.3560820046338,"y":185.9062468532269},{"x":91.55509146513478,"y":245.7236887429557}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da2716897541043697","data":[{"x":87.12416984367336,"y":95.07235361326829},{"x":119.24835159926843,"y":142.7047610439783}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da09979586059498846","data":[{"x":359.62584956354925,"y":183.69078604249617},{"x":365.16450159037583,"y":278.9556009039161}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da5261018292698869","data":[{"x":149.15707254413283,"y":139.38156982788226},{"x":220.05181848751522,"y":72.91774550596136}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da04192212882086088","data":[{"x":275.4383387557826,"y":71.81001510059599},{"x":346.33308469916494,"y":129.4119961795941}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da6575100590837823","data":[{"x":284.854047201388,"y":244.06209313490763},{"x":341.3482978750208,"y":180.92146002908285}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da1878499477156954","data":[{"x":158.57278098973836,"y":180.92146002908285},{"x":233.34458335189936,"y":244.06209313490763}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da6107386369793153","data":[{"x":99,"y":61},{"x":219.72524418472125,"y":65.73301064381621}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2,"strokeColor":[0,0,0,1]}},{"id":"da547804609150343","data":[{"x":100.49332049260892,"y":70.62589891067928},{"x":247,"y":230}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2,"strokeColor":[0,0,0,1]}},{"id":"da7910015406572051","data":[{"x":102,"y":267},{"x":233,"y":265}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2,"strokeColor":[0,0,0,1]}},{"id":"da7302497609970906","data":[{"x":100,"y":260},{"x":240,"y":92}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2,"strokeColor":[0,0,0,1]}},{"id":"da8199483907786584","data":[{"x":161,"y":152},{"x":325.31306594751015,"y":156.31936937274156}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2,"strokeColor":[0,0,0,1]}},{"id":"da5142309557360307","data":[{"x":253,"y":93},{"x":259,"y":228}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2,"strokeColor":[0,0,0,1]}},{"id":"da8692420184562233","data":[{"x":263,"y":87},{"x":348,"y":285}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2,"strokeColor":[0,0,0,1]}},{"id":"da8733708275086898","data":[{"x":284,"y":267},{"x":336.80041272787156,"y":306.1177976467841}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2,"strokeColor":[0,0,0,1]}},{"id":"dp9735869331610174","type":"circle","data":{"p1":{"x":34.82262539326754,"y":31.724849730022996},"p2":{"x":110.62472375458012,"y":107.52694809133557}},"style":{"strokeType":{"type":"dash","pattern":[6,6]},"strokeColor":[247,31,31,0.5],"thickness":2}},{"id":"dp2881144121364341","type":"circle","data":{"p1":{"x":315.18166268553887,"y":117.41832019208528},"p2":{"x":390.98376104685144,"y":193.22041855339785}},"style":{"strokeType":{"type":"dash","pattern":[6,6]},"strokeColor":[70,114,191,0.5],"thickness":2}}],"settings":{"grid":true,"diagramHeight":358.6640625},"id":"n0.28901377736349465"}],"id":"n0.7831426104925614"}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":29,"delayRenderCache":{"av":29,"map":{}}}

==> figs/docs/1ab4a360-76c0-474c-99c7-66a86b960b82 <==
{"id":"r0.28521863390524915","lines":[{"id":"n0.06518260433361944","blocks":[]},{"id":"n0.6194212053376131","blocks":[{"id":"n0.6191531776013918","text":"\t"},{"id":"n0.07332230663346939","text":"\\diagram","type":"composite","elements":{"de15039028513302677":{"id":"de15039028513302677","lines":[{"id":"n0.5107313851872686","blocks":[{"id":"n0.42843794643142674","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.9060529032807887","lines":[{"id":"n0.19573768613661602","blocks":[{"id":"n0.5348227975507165","text":"U"}]}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"}}]}],"shape":{"data":{"p":{"x":319.95311666666663,"y":92.79166666666666}},"anchor":"bottom","settings":{"fontSize":"\\footnotesize"},"style":{"textColor":[0,0,0,1]}},"isTextMode":true},"de2056536707556802":{"id":"de2056536707556802","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.5939194986973031","text":"R"},{"id":"n0.6000189477842409","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.9481095209997417","lines":[{"id":"n0.20255343288436023","blocks":[{"id":"n0.6556129498897879","text":"d"}]}]}}}],"id":"n0.848091092695114"}],"id":"n0.03968552834638284"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.028048137251828864"}],"id":"n0.20536520778145428"}],"shape":{"data":{"p":{"x":480.8645833333333,"y":221.41666666666663}},"anchor":"top","settings":{"fontSize":"\\footnotesize"},"style":{"textColor":[0,0,0,1]}},"isTextMode":true},"de8507121270116855":{"id":"de8507121270116855","lines":[{"id":"n0.08652612109775304","blocks":[{"id":"n0.3749822100905851","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.6752865795068277","lines":[{"id":"n0.6856995060429103","blocks":[{"id":"n0.6509987067803147","text":"\\bigr","type":"composite","elements":{},"bracketName":"brace","size":"Big","isClose":true},{"id":"n0.40749939693789716","text":"d"},{"id":"n0.8378249234042816","text":"\\power","type":"composite","elements":{"powerValue":{"id":"n0.32540870314051495","lines":[{"id":"n0.21791442623215762","blocks":[{"id":"n0.837124943481472","text":"2"}]}]}}}]}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"}},{"id":"n0.32522147741758056","text":" nodes"}]}],"shape":{"data":{"p":{"x":569.5833333333334,"y":183.33333333333334}},"anchor":"left-top"},"isTextMode":true},"de27788409947776493":{"id":"de27788409947776493","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"\\bigr","type":"composite","elements":{},"bracketName":"brace","size":"Big","isClose":true,"id":"n0.7344591634201596"},{"id":"n0.68332261245975","text":"d"}],"id":"n0.7557516266998732"}],"id":"n0.8610858042888305"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.7161347467271861"},{"text":" nodes","id":"n0.8145059028898136"}],"id":"n0.3126632235315552"}],"shape":{"data":{"p":{"x":573.5833333333334,"y":88}},"anchor":"left-top"},"isTextMode":true},"de8042296701453001":{"id":"de8042296701453001","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"L","id":"n0.3735217842357319"},{"id":"n0.584377154227965","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.9934670018554183","lines":[{"id":"n0.28027619982182916","blocks":[{"id":"n0.5602947151307301","text":"1"}]}]}}}],"id":"n0.6649919718901361"}],"id":"n0.29760560092914445"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.8707198169795867"}],"id":"n0.3861278221330884"}],"shape":{"data":{"p":{"x":148.70833333333331,"y":221.41666666666663}},"anchor":"top","settings":{"fontSize":"\\footnotesize"},"style":{"textColor":[0,0,0,1]}},"isTextMode":true},"de2823275296323421":{"id":"de2823275296323421","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"\\bigr","type":"composite","elements":{},"bracketName":"brace","size":"Big","isClose":true,"id":"n0.7434924159305982"},{"text":"d","id":"n0.5602891477163346"},{"text":"\\power","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"id":"n0.33231862703560333","text":"3"}],"id":"n0.8913441967117193"}],"id":"n0.2183487671276494"}},"id":"n0.2536646657584536"}],"id":"n0.6766983729963553"}],"id":"n0.9845331990038118"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.32749390736131734"},{"text":" nodes","id":"n0.8581103628706842"}],"id":"n0.4167461259423897"}],"shape":{"data":{"p":{"x":569.5833333333334,"y":263.33333333333337}},"anchor":"left-top"},"isTextMode":true},"de1717068357981758":{"id":"de1717068357981758","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.20347167340390793","text":"C"}],"id":"n0.33370557773479625"}],"id":"n0.822331257214332"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.9006500698027698"}],"id":"n0.6065311056168564"}],"shape":{"data":{"p":{"x":475.0052333333333,"y":302.66666666666663}},"anchor":"top","settings":{"fontSize":"\\footnotesize"},"style":{"textColor":[0,0,0,1]}},"isTextMode":true},"de9071908877443866":{"id":"de9071908877443866","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"R","id":"n0.24507579195091722"},{"id":"n0.42597427041018765","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.024805576404810625","lines":[{"id":"n0.32650008460172586","blocks":[{"id":"n0.6476978928240014","text":"1"}]}]}}}],"id":"n0.37998696183881364"}],"id":"n0.43614208951185995"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.4013993032927835"}],"id":"n0.20294430598951874"}],"shape":{"data":{"p":{"x":244.86458333333331,"y":221.41666666666663}},"anchor":"top","settings":{"fontSize":"\\footnotesize"},"style":{"textColor":[0,0,0,1]}},"isTextMode":true},"de813048302240891":{"id":"de813048302240891","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.2690835593461963","text":"L"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"d","id":"n0.1527376185443745"}],"id":"n0.4084306146585581"}],"id":"n0.8172316097789597"}},"id":"n0.5017625238625336"}],"id":"n0.887985369790319"}],"id":"n0.8247928246950001"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.9827787633437781"}],"id":"n0.3346620188649496"}],"shape":{"data":{"p":{"x":383.3645833333333,"y":220.91666666666663}},"anchor":"top","settings":{"fontSize":"\\footnotesize"},"style":{"textColor":[0,0,0,1]}},"isTextMode":true},"de6013235778434128":{"id":"de6013235778434128","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"L=L","id":"n0.6857402933773286"},{"id":"n0.9854831592861905","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.37394619695126474","lines":[{"id":"n0.2218460567398287","blocks":[{"id":"n0.42484633970375285","text":"1"}]}]}}},{"id":"n0.37773372337218214","text":"∪⋯∪L"},{"id":"n0.6625323597587822","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.0856775768518303","lines":[{"id":"n0.26858329433308703","blocks":[{"id":"n0.9103682998118315","text":"d"}]}]}}}],"id":"n0.8539896367889854"}],"id":"n0.29292972845949994"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.16932078973822662"}],"id":"n0.4540363650855911"}],"shape":{"data":{"p":{"x":61.364583333333215,"y":136.9166666666666}},"anchor":"top","settings":{"fontSize":"\\footnotesize"},"style":{"textColor":[0,0,0,1]}},"isTextMode":true},"de1150022496576173":{"id":"de1150022496576173","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"R=R","id":"n0.7986414168304115"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"1","id":"n0.4943737003467894"}],"id":"n0.5443617425109886"}],"id":"n0.291465729142213"}},"id":"n0.2823665886685699"},{"text":"∪⋯∪R","id":"n0.8321098467559559"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"d","id":"n0.8928477938024549"}],"id":"n0.06596776793554293"}],"id":"n0.10868465137961059"}},"id":"n0.8805873972058432"}],"id":"n0.8452818300856076"}],"id":"n0.6127529916542673"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.5523218856503112"}],"id":"n0.3536861293008733"}],"shape":{"data":{"p":{"x":61.364583333333215,"y":157.4166666666666}},"anchor":"top","settings":{"fontSize":"\\footnotesize"},"style":{"textColor":[0,0,0,1]}},"isTextMode":true},"de4493783830603988":{"id":"de4493783830603988","lines":[{"id":"n0.5789419106206919","blocks":[{"id":"n0.14053065499663497","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.7783555987421398","lines":[{"id":"n0.8124787856003206","blocks":[{"id":"n0.7245028724160557","text":"l"}]}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"}}]}],"shape":{"data":{"p":{"x":241.9173775671407,"y":57.575434439178515}},"anchor":"center","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":false},"de8222484086618581":{"id":"de8222484086618581","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"r","id":"n0.640037785349018"}],"id":"n0.580376732388651"}],"id":"n0.15499019587715368"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.9056656102358663"}],"id":"n0.5111711335641822"}],"shape":{"data":{"p":{"x":412.9173775671407,"y":58.575434439178515}},"anchor":"center","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":false}},"connections":[],"intersections":{"id":"di30119318020760555","items":[],"style":{}},"shapes":[{"id":"dp6775323334711851","type":"doc-rounded-rect","data":{"p1":{"x":104.41353258370985,"y":188.8319115323856},"p2":{"x":190,"y":219.28688783570314},"cornerRadiusPercentage":1,"flipX":true},"style":{"fillColor":[74,144,226,0.3],"strokeColor":"none","strokeType":"."}},{"id":"dp6273853992007636","type":"doc-rounded-rect","data":{"p1":{"x":184.83332824707028,"y":94.5},"p2":{"x":454.5,"y":124.5},"flipX":true,"cornerRadiusPercentage":1},"style":{"fillColor":[74,144,226,0.3],"strokeType":".","strokeColor":"none"}},{"id":"dp9465494443833103","type":"circle","data":{"p1":{"x":233.25860979462885,"y":48.916666666666664},"p2":{"x":250.57614533965256,"y":66.23420221169036},"flipX":true},"style":{"thickness":2}},{"id":"dp8579067391001112","type":"ellipse","data":{"p1":{"x":417.1454976303319,"y":100.8832543443918},"p2":{"x":434.46303317535546,"y":118.20078988941547},"flipX":true},"style":{"thickness":2}},{"id":"da441223531627952","data":[{"x":329.6666666666667,"y":108.63443917851504},{"x":313.6666666666667,"y":108.63443917851504}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"da1106915686367067","data":[{"x":432.5,"y":115.16666603088379},{"x":504.1965876777252,"y":196.73396524486583}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"da2646109971355177","data":[{"x":425.80426540284367,"y":118.20078988941547},{"x":454.6965876777252,"y":196.73396524486583}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"da09711609278280009","data":[{"x":418.5,"y":114.66666603088379},{"x":355.6965876777252,"y":196.73396524486583}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"da9055635253679755","data":[{"x":425.80426540284367,"y":118.20078988941547},{"x":405.1965876777252,"y":196.73396524486583}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"dp5603243908746471","type":"circle","data":{"p1":{"x":204.30094786729865,"y":100.8832543443918},"p2":{"x":221.61848341232235,"y":118.2007898894155},"flipX":true},"style":{"thickness":2}},{"id":"dp01320910698982214","type":"circle","data":{"p1":{"x":113.03781990521333,"y":195.73396524486583},"p2":{"x":130.35535545023703,"y":213.05150078988953},"flipX":true},"style":{"thickness":2}},{"id":"da32847301341249957","data":[{"x":153.55924170616123,"y":204.39273301737768},{"x":136.16666666666666,"y":204.39273301737768}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"da3127696548597576","data":[{"x":220,"y":114.66666603088379},{"x":267.1965876777252,"y":196.73396524486583}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"da8859796406630904","data":[{"x":212.9597156398105,"y":118.2007898894155},{"x":217.69658767772518,"y":196.73396524486583}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"da6297628972213167","data":[{"x":206,"y":114.16666603088379},{"x":121.69658767772518,"y":195.73396524486583}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"da8019018837930725","data":[{"x":212.9597156398105,"y":118.2007898894155},{"x":171.19658767772518,"y":195.73396524486583}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"dp5243755645627607","type":"doc-rounded-rect","data":{"p1":{"x":70,"y":269.33191153238556},"p2":{"x":564.6666564941406,"y":299.78688783570317},"cornerRadiusPercentage":1,"flipX":true},"style":{"fillColor":[74,144,226,0.3],"strokeColor":"none","strokeType":"."}},{"id":"dp32684065962412046","type":"circle","data":{"p1":{"x":84.53781990521333,"y":276.23396524486583},"p2":{"x":101.85535545023703,"y":293.55150078988953},"flipX":true},"style":{"thickness":2}},{"id":"dp5726528615790015","type":"circle","data":{"p1":{"x":128.53781990521333,"y":276.23396524486583},"p2":{"x":145.85535545023703,"y":293.55150078988953},"flipX":true},"style":{"thickness":2}},{"id":"dp5632596861052938","type":"circle","data":{"p1":{"x":245.53781990521333,"y":276.23396524486583},"p2":{"x":262.855355450237,"y":293.55150078988953},"flipX":true},"style":{"thickness":2}},{"id":"dp8615186927048318","type":"circle","data":{"p1":{"x":288.5378199052133,"y":276.23396524486583},"p2":{"x":305.855355450237,"y":293.55150078988953},"flipX":true},"style":{"thickness":2}},{"id":"dp011758749371382216","type":"circle","data":{"p1":{"x":534.0378199052134,"y":276.23396524486583},"p2":{"x":551.3553554502371,"y":293.55150078988953},"flipX":true},"style":{"thickness":2}},{"id":"dp590606559413012","type":"circle","data":{"p1":{"x":487.5378199052133,"y":276.23396524486583},"p2":{"x":504.855355450237,"y":293.55150078988953},"flipX":true},"style":{"thickness":2}},{"id":"dp04682936877367494","type":"circle","data":{"p1":{"x":371.5378199052133,"y":276.23396524486583},"p2":{"x":388.855355450237,"y":293.55150078988953},"flipX":true},"style":{"thickness":2}},{"id":"dp47543350721521127","type":"circle","data":{"p1":{"x":327.0378199052133,"y":276.23396524486583},"p2":{"x":344.355355450237,"y":293.55150078988953},"flipX":true},"style":{"thickness":2}},{"id":"da6311575203734016","data":[{"x":123.05924170616123,"y":285.3927330173777},{"x":105.66666666666666,"y":285.3927330173777}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"da7382006730468686","data":[{"x":283.55924170616123,"y":285.3927330173777},{"x":266.16666666666663,"y":285.3927330173777}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"da1776440269123255","data":[{"x":364.55924170616123,"y":285.3927330173777},{"x":347.16666666666663,"y":285.3927330173777}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"da2395629736080198","data":[{"x":526.5592417061612,"y":285.3927330173777},{"x":509.16666666666663,"y":285.3927330173777}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"da48920268912054143","data":[{"x":225.55924170616123,"y":285.8927330173777},{"x":208.16666666666666,"y":285.8927330173777}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"da6132637019993894","data":[{"x":467.05924170616123,"y":285.8927330173777},{"x":449.66666666666663,"y":285.8927330173777}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"da6397913116600679","data":[{"x":121.69658767772518,"y":213.05150078988953},{"x":93.19658767772518,"y":276.23396524486583}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"da2237548185354986","data":[{"x":121.69658767772518,"y":213.05150078988953},{"x":137.19658767772518,"y":276.23396524486583}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"da3425751786158667","data":[{"x":217.69658767772518,"y":214.05150078988953},{"x":205.5,"y":279.6666660308838}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"da499819388709724","data":[{"x":217.69658767772518,"y":214.05150078988953},{"x":232.5,"y":280.1666660308838}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"da9396261526205891","data":[{"x":267.1965876777252,"y":214.05150078988953},{"x":254.19658767772518,"y":276.23396524486583}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"da37116591848272973","data":[{"x":267.1965876777252,"y":214.05150078988953},{"x":297.1965876777252,"y":276.23396524486583}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"da09660910798699496","data":[{"x":355.6965876777252,"y":214.05150078988953},{"x":335.6965876777252,"y":276.23396524486583}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"da9065314309047453","data":[{"x":355.6965876777252,"y":214.05150078988953},{"x":380.1965876777252,"y":276.23396524486583}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"da545359090681841","data":[{"x":454.6965876777252,"y":214.05150078988953},{"x":445.5,"y":280.6666660308838}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"da4733405428538744","data":[{"x":454.6965876777252,"y":214.05150078988953},{"x":475,"y":280.6666660308838}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"da3110369266443366","data":[{"x":504.1965876777252,"y":214.05150078988953},{"x":496.1965876777252,"y":276.23396524486583}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"da6657434869061204","data":[{"x":504.1965876777252,"y":214.05150078988953},{"x":542.6965876777252,"y":276.23396524486583}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"dp48302591128291916","type":"circle","data":{"p1":{"x":404.25860979462885,"y":49.916666666666664},"p2":{"x":421.57614533965256,"y":67.23420221169036},"flipX":true},"style":{"thickness":2}},{"id":"da14878287553720237","data":[{"x":235.3333282470703,"y":63.5},{"x":121.69658767772518,"y":195.73396524486583}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"da7906866558921558","data":[{"x":248.3333282470703,"y":64},{"x":355.6965876777252,"y":196.73396524486583}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"da6368537989812343","data":[{"x":404.25860979462885,"y":58.57543443917851},{"x":217.69658767772518,"y":196.73396524486583}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"da9126076638936663","data":[{"x":407.5,"y":66.16666603088379},{"x":267.1965876777252,"y":196.73396524486583}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"da6220502617301947","data":[{"x":421.57614533965256,"y":58.57543443917851},{"x":504.1965876777252,"y":196.73396524486583}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"dp8234168664097423","type":"circle","data":{"p1":{"x":162.53781990521333,"y":195.73396524486583},"p2":{"x":179.85535545023703,"y":213.05150078988953},"flipX":true},"style":{"thickness":2}},{"id":"da17004928345515014","data":[{"p1":{"x":241.9173775671407,"y":66.23420221169036},"p2":{"x":171.19658767772518,"y":195.73396524486583},"cp":{"dx":-1.4173775671407043,"dy":46.43246381919343},"cp2":{"dx":34.30341232227482,"dy":-19.06729921398204}}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"type":"cubic","headScale":0.6},{"id":"dp5369251712276115","type":"doc-rounded-rect","data":{"p1":{"x":200.41353258370987,"y":189.8319115323856},"p2":{"x":286,"y":220.28688783570314},"cornerRadiusPercentage":1,"flipX":true},"style":{"fillColor":[74,144,226,0.3],"strokeColor":"none","strokeType":"."}},{"id":"dp06493937665149474","type":"circle","data":{"p1":{"x":209.03781990521333,"y":196.73396524486583},"p2":{"x":226.35535545023703,"y":214.05150078988953},"flipX":true},"style":{"thickness":2}},{"id":"da45527648058580383","data":[{"x":250.55924170616123,"y":205.39273301737768},{"x":233.16666666666666,"y":205.39273301737768}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"dp690031985153834","type":"circle","data":{"p1":{"x":258.5378199052133,"y":196.73396524486583},"p2":{"x":275.855355450237,"y":214.05150078988953},"flipX":true},"style":{"thickness":2}},{"id":"dp8393337054062688","type":"doc-rounded-rect","data":{"p1":{"x":338.41353258370987,"y":189.8319115323856},"p2":{"x":424,"y":220.28688783570314},"cornerRadiusPercentage":1,"flipX":true},"style":{"fillColor":[74,144,226,0.3],"strokeColor":"none","strokeType":"."}},{"id":"dp9224300882863654","type":"circle","data":{"p1":{"x":347.0378199052133,"y":196.73396524486583},"p2":{"x":364.355355450237,"y":214.05150078988953},"flipX":true},"style":{"thickness":2}},{"id":"da7128271518762995","data":[{"x":388.55924170616123,"y":205.39273301737768},{"x":371.16666666666663,"y":205.39273301737768}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"dp5365417986274068","type":"circle","data":{"p1":{"x":396.5378199052133,"y":196.73396524486583},"p2":{"x":413.855355450237,"y":214.05150078988953},"flipX":true},"style":{"thickness":2}},{"id":"dp21946810260001304","type":"doc-rounded-rect","data":{"p1":{"x":437.41353258370987,"y":189.8319115323856},"p2":{"x":523,"y":220.28688783570314},"cornerRadiusPercentage":1,"flipX":true},"style":{"fillColor":[74,144,226,0.3],"strokeColor":"none","strokeType":"."}},{"id":"dp8731592575303555","type":"circle","data":{"p1":{"x":446.0378199052133,"y":196.73396524486583},"p2":{"x":463.355355450237,"y":214.05150078988953},"flipX":true},"style":{"thickness":2}},{"id":"da4142606917973545","data":[{"x":487.55924170616123,"y":205.39273301737768},{"x":470.16666666666663,"y":205.39273301737768}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"dp8345091790717905","type":"circle","data":{"p1":{"x":495.5378199052133,"y":196.73396524486583},"p2":{"x":512.8553554502371,"y":214.05150078988953},"flipX":true},"style":{"thickness":2}},{"id":"da5894623497346217","data":[{"x":250.57614533965256,"y":57.57543443917851},{"x":405.1965876777252,"y":196.73396524486583}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"da1166823519908724","data":[{"p1":{"x":412.9173775671407,"y":67.23420221169036},"p2":{"x":454.6965876777252,"y":196.73396524486583},"cp":{"dx":-9.417377567140704,"dy":33.43246381919343},"cp2":{"dx":-50.69658767772518,"dy":-22.06729921398204}}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"type":"cubic","headScale":0.6},{"id":"da250919371920449","data":[{"x":171.19658767772518,"y":213.05150078988953},{"x":157,"y":280.1666660308838}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"da09791477577972052","data":[{"x":171.19658767772518,"y":213.05150078988953},{"x":183.5,"y":279.6666660308838}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"da03785701415761067","data":[{"x":177.55924170616123,"y":285.8927330173777},{"x":160.16666666666666,"y":285.8927330173777}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"da01872063778972244","data":[{"x":320.55924170616123,"y":207.89273301737768},{"x":303.16666666666663,"y":207.89273301737768}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"da3613204734227895","data":[{"x":421.55924170616123,"y":286.3927330173777},{"x":404.16666666666663,"y":286.3927330173777}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"da9980440694221578","data":[{"x":405.1965876777252,"y":214.05150078988953},{"x":401,"y":279.6666660308838}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"da7709243774219362","data":[{"x":405.1965876777252,"y":214.05150078988953},{"x":427.5,"y":278.6666660308838}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6}],"settings":{"grid":true,"diagramHeight":336}}]},{"id":"n0.4927878538015349","blocks":[],"style":null}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":2121,"delayRenderCache":{"av":2121,"map":{}}}

==> figs/docs/2f20ee60-5db7-4b2c-bf8b-b1613c00d6f0 <==
{"id":"r0.9363525302207351","lines":[{"blocks":[{"text":"\\diagram","type":"composite","elements":{},"connections":[],"intersections":{"id":"di018738070182718003","items":[],"style":{}},"shapes":[{"id":"dp7678180359824416","type":"ellipse","data":{"p1":{"x":49.620695321905416,"y":47.57472397714416},"p2":{"x":83.04597134476127,"y":81}},"style":{"fillColor":"none"}},{"id":"dp30943822528415454","type":"ellipse","data":{"p1":{"x":49.96670401123383,"y":165.40727418009203},"p2":{"x":83.39198003408957,"y":198.83255020294786},"rotation":12.59},"style":{"fillColor":"none"}},{"id":"dp25365469387754036","type":"ellipse","data":{"p1":{"x":87.7964198266168,"y":103.4782423779815},"p2":{"x":121.22169584947291,"y":136.9035184008373},"rotation":11.34},"style":{"fillColor":[255,255,255,1]}},{"id":"dp7921073162567045","type":"ellipse","data":{"p1":{"x":225.2590272620554,"y":189.6627528888692},"p2":{"x":258.68430328491115,"y":223.08802891172502},"rotation":1.24},"style":{"fillColor":"none"}},{"id":"dp7164384411895472","type":"ellipse","data":{"p1":{"x":161.72685914559003,"y":159.00372577019766},"p2":{"x":195.15213516844568,"y":192.42900179305337},"rotation":312.14},"style":{"fillColor":"none"}},{"id":"dp1575690908235119","type":"ellipse","data":{"p1":{"x":154.80345741092947,"y":44.630031391797814},"p2":{"x":188.22873343378535,"y":78.05530741465364}},"style":{"fillColor":"none"}},{"id":"dp876913725987533","type":"ellipse","data":{"p1":{"x":218.349497886343,"y":99.14772407837313},"p2":{"x":251.77477390919876,"y":132.57300010122896}},"style":{"fillColor":"none"}},{"id":"da30066865907408724","data":[{"x":62.33333333333333,"y":165.66666666666669},{"x":62.33333333333333,"y":80.33333333333334}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da20089240367824313","data":[{"x":95.00000000000001,"y":133.66666666666669},{"x":77.6666666666667,"y":169.66666666666669}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da5200525497623829","data":[{"x":75.00000000000001,"y":79},{"x":94.33333333333333,"y":107.66666666666667}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da008777702432074541","data":[{"x":239.00000000000003,"y":132.33333333333334},{"x":242.33333333333331,"y":189.66666666666666}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da22708496323155036","data":[{"x":112.33333333333333,"y":105.66666666666667},{"x":155,"y":65.66666666666667}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da8303552775456196","data":[{"x":188.33333333333331,"y":65},{"x":231,"y":99.66666666666667}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da5450445884933472","data":[{"x":194,"y":168.66666666666669},{"x":228,"y":130.66666666666669}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da35701763839380396","data":[{"x":118.00000000000001,"y":130.66666666666669},{"x":163,"y":168.66666666666669}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}}],"settings":{"grid":true},"id":"n0.1790561663137804"}],"id":"n0.1350696478635458"}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":4,"delayRenderCache":{"av":4,"map":{}}}

==> figs/docs/32b90faa-abeb-44c1-a319-cf41603b11b1 <==
{"id":"r0.8446259560934545","lines":[{"blocks":[{"text":"\\diagram","type":"composite","elements":{"de025248099529535217":{"id":"de025248099529535217","lines":[{"blocks":[{"id":"n0.24409373399099676","text":"5"}],"id":"n0.6717827961417553"}],"shape":{"data":{"p":{"x":128.8643076797487,"y":153.30550394860256},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de39477509033102254":{"id":"de39477509033102254","lines":[{"blocks":[{"text":"2","id":"n0.6184375838931457"}],"id":"n0.3367382751830077"}],"shape":{"data":{"p":{"x":65.72367457392377,"y":60.256149897913346},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de6882383615175067":{"id":"de6882383615175067","lines":[{"blocks":[{"id":"n0.8655310222352957","text":"4"}],"id":"n0.023172031153918526"}],"shape":{"data":{"p":{"x":66.83140497928915,"y":256.32443164757996},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de5433981856983177":{"id":"de5433981856983177","lines":[{"blocks":[{"id":"n0.7923455347763033","text":"1"}],"id":"n0.20383520791531162"}],"shape":{"data":{"p":{"x":240.7450786216489,"y":54.71749787108662},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de36633508228345857":{"id":"de36633508228345857","lines":[{"blocks":[{"id":"n0.4883945651770736","text":"6"}],"id":"n0.3972610725454533"}],"shape":{"data":{"p":{"x":347.0871975367224,"y":145.55139111104518},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de48197968942878555":{"id":"de48197968942878555","lines":[{"blocks":[{"id":"n0.40896109414724213","text":"3"}],"id":"n0.08222314278848875"}],"shape":{"data":{"p":{"x":251.82238267530238,"y":245.24712759392654},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de73180313314566":{"id":"de73180313314566","lines":[{"blocks":[{"text":"7","id":"n0.4646242437363426"}],"id":"n0.09532159362380233"}],"shape":{"data":{"p":{"x":357.0567711850105,"y":296.2027262407325},"rotation":0},"anchor":"left-top"},"isTextMode":true}},"connections":[],"intersections":{"id":"di018738070182718003","items":[],"style":{}},"shapes":[{"id":"dp003952293913724869","type":"circle","data":{"p1":{"x":315.18166268553887,"y":118.41832019208528},"p2":{"x":390.98376104685144,"y":194.22041855339785}},"style":{"strokeType":{"type":"dash","pattern":[6,6]},"strokeColor":[70,114,191,0.5],"thickness":2,"fillColor":"none"}},{"id":"dp5328103640683022","type":"ellipse","data":{"p1":{"x":44.95402865523873,"y":42.85625299199422},"p2":{"x":100.49332049260892,"y":98.39554482936434}},"style":{"fillColor":[247,31,31,1]}},{"id":"dp7250437190184513","type":"ellipse","data":{"p1":{"x":45.52895517377332,"y":238.64630089431083},"p2":{"x":101.06824701114326,"y":294.1855927316803},"rotation":12.59},"style":{"fillColor":[247,31,31,1]}},{"id":"dp8522947932757496","type":"ellipse","data":{"p1":{"x":108.38664482631847,"y":135.74529364125738},"p2":{"x":163.92593666368901,"y":191.28458547862738},"rotation":11.34},"style":{"fillColor":[247,31,31,1]}},{"id":"dp36773303037713356","type":"ellipse","data":{"p1":{"x":336.79390961187244,"y":278.949097787917},"p2":{"x":392.33320144924306,"y":334.4883896252872},"rotation":1.24},"style":{"fillColor":[70,114,191,1]}},{"id":"dp06833667561838697","type":"ellipse","data":{"p1":{"x":231.22913809978522,"y":228.00619298050708},"p2":{"x":286.7684299371551,"y":283.5454848178769},"rotation":312.14},"style":{"fillColor":[70,114,191,1]}},{"id":"dp5227364052833068","type":"ellipse","data":{"p1":{"x":219.72524418472122,"y":37.96336472513116},"p2":{"x":275.26453602209136,"y":93.50265656250127}},"style":{"fillColor":[70,114,191,1]}},{"id":"dp7842656804303263","type":"ellipse","data":{"p1":{"x":325.31306594751015,"y":128.5497234540565},"p2":{"x":380.85235778488016,"y":184.0890152914266}},"style":{"fillColor":[70,114,191,1]}},{"id":"da6433920756150986","data":[{"x":66.0772921417317,"y":239.0773063107636},{"x":66.0772921417317,"y":97.28781442399901}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da9257172944690841","data":[{"x":120.3560820046338,"y":185.9062468532269},{"x":91.55509146513478,"y":245.7236887429557}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da02918461673488304","data":[{"x":87.12416984367336,"y":95.07235361326829},{"x":119.24835159926843,"y":142.7047610439783}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da4896970497790636","data":[{"x":359.62584956354925,"y":183.69078604249617},{"x":365.16450159037583,"y":278.9556009039161}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da9504762335968284","data":[{"x":149.15707254413283,"y":139.38156982788226},{"x":220.05181848751522,"y":72.91774550596136}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da42445026461452606","data":[{"x":275.4383387557826,"y":71.81001510059599},{"x":346.33308469916494,"y":129.4119961795941}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da8236720921246363","data":[{"x":284.854047201388,"y":244.06209313490763},{"x":341.3482978750208,"y":180.92146002908285}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da8422667281310829","data":[{"x":158.57278098973836,"y":180.92146002908285},{"x":233.34458335189936,"y":244.06209313490763}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"dp7974759228827735","type":"circle","data":{"p1":{"x":34.82262539326754,"y":32.724849730022996},"p2":{"x":110.62472375458012,"y":108.52694809133557}},"style":{"strokeType":{"type":"dash","pattern":[6,6]},"strokeColor":[247,31,31,0.5],"thickness":2}}],"settings":{"grid":true,"diagramHeight":358.6640625},"id":"n0.2692365095875584"}],"id":"n0.6972094735025989"}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":38,"delayRenderCache":{"av":38,"map":{}}}

==> figs/docs/5e157a28-d82d-4a92-ba31-8f05b6859148 <==
{"id":"r0.776406658125812","lines":[{"blocks":[{"text":"\\diagram","type":"composite","elements":{"de3544795981582072":{"id":"de3544795981582072","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"i","id":"n0.08514454852001418"}],"id":"n0.43426065844567674"}],"id":"n0.6901971308271797"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.5866127357428037"}],"id":"n0.5193810027171173"}],"shape":{"data":{"p":{"x":260.66666666666663,"y":39.000000000000014}},"anchor":"left-top"},"isTextMode":true},"de8484510341321756":{"id":"de8484510341321756","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"j","id":"n0.8312475411636133"}],"id":"n0.9478795093356753"}],"id":"n0.8290467198692975"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.6385239986157161"}],"id":"n0.09983342083567748"}],"shape":{"data":{"p":{"x":447,"y":89.33333333333331}},"anchor":"left-top"},"isTextMode":true},"de9666708060481679":{"id":"de9666708060481679","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"e","id":"n0.11498992169876598"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"1","id":"n0.22706598082780016"}],"id":"n0.41482356638812634"}],"id":"n0.09311345581863173"}},"id":"n0.11586559892914194"}],"id":"n0.3079095250387529"}],"id":"n0.3156600015741382"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.9570765398071353"}],"id":"n0.6356762682372832"}],"shape":{"data":{"p":{"x":192,"y":68.66666666666667}},"anchor":"left-top","style":{"textColor":[247,31,31,0.7],"strokeColor":[247,31,31,0.7]}},"isTextMode":true},"de737126538049655":{"id":"de737126538049655","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"e","id":"n0.8358301542319027"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"0","id":"n0.563588593151775"}],"id":"n0.10178818225206876"}],"id":"n0.2939749662912836"}},"id":"n0.7617971141524673"}],"id":"n0.3729864701196306"}],"id":"n0.8022284885660058"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.6103695698033464"}],"id":"n0.6343721093033703"}],"shape":{"data":{"p":{"x":466.00000000000006,"y":202.00000000000003}},"anchor":"left-top","style":{"textColor":[70,114,191,0.7]}},"isTextMode":true}},"connections":[],"intersections":{"id":"di018738070182718003","items":[],"style":{}},"shapes":[{"id":"dp6354509486975801","type":"ellipse","data":{"p1":{"x":154.29440727711722,"y":200.3236383304401},"p2":{"x":187.71968329997304,"y":233.74891435329593}},"style":{"fillColor":"none"}},{"id":"dp7001276822468621","type":"ellipse","data":{"p1":{"x":193.25037935120338,"y":103.75910268422604},"p2":{"x":226.6756553740592,"y":137.18437870708186}},"style":{"fillColor":[70,114,191,1]}},{"id":"dp3861827195136025","type":"ellipse","data":{"p1":{"x":204.96670401123384,"y":202.74060751342537},"p2":{"x":238.3919800340896,"y":236.16588353628117},"rotation":12.59},"style":{"fillColor":"none"}},{"id":"dp4169065632691238","type":"ellipse","data":{"p1":{"x":284.7964198266168,"y":118.14490904464816},"p2":{"x":318.2216958494729,"y":151.57018506750393},"rotation":11.34},"style":{"fillColor":[255,255,255,1]}},{"id":"dp5470533987627895","type":"ellipse","data":{"p1":{"x":279.5652175137361,"y":198.57464460518992},"p2":{"x":312.9904935365919,"y":231.99992062804577},"rotation":1.24},"style":{"fillColor":[70,114,191,1]}},{"id":"dp5414864328622275","type":"ellipse","data":{"p1":{"x":373.7268591455899,"y":193.67039243686418},"p2":{"x":407.15213516844557,"y":227.0956684597199},"rotation":312.14},"style":{"fillColor":[70,114,191,1]}},{"id":"dp3273686568045808","type":"ellipse","data":{"p1":{"x":369.80345741092947,"y":93.29669805846447},"p2":{"x":403.22873343378535,"y":126.7219740813203}},"style":{"fillColor":[70,114,191,1]}},{"id":"dp4913079312946387","type":"ellipse","data":{"p1":{"x":451.349497886343,"y":128.8143907450398},"p2":{"x":484.77477390919876,"y":162.2396667678956}},"style":{"fillColor":[70,114,191,1]}},{"id":"da19980729985161894","data":[{"x":175.33333333333334,"y":201.33333333333334},{"x":198,"y":132}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da19342881412810398","data":[{"x":209.96301736263126,"y":137.18437870708186},{"x":220.66666666666666,"y":202.66666666666666}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da1524998124953485","data":[{"x":226.6756553740592,"y":120.47174069565395},{"x":285.1226902403077,"y":131.57132943503288}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da7458612511372753","data":[{"x":298.2228402170017,"y":151.2439146538132},{"x":296.639523585014,"y":198.57855838298735}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da8660509904424405","data":[{"x":314.29829411481217,"y":124.5923043139567},{"x":369.80345741092947,"y":110.00933606989238}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da3070656274770447","data":[{"x":386.51609542235735,"y":126.7219740813203},{"x":390.8046279406934,"y":194.23268510418194}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da7790663635222754","data":[{"x":406.49823487933577,"y":204.0411894408334},{"x":457.3333333333333,"y":158}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da9392144903901656","data":[{"x":315.25,"y":144.5},{"x":378.04694881946455,"y":199.16977868966148}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"dg09882176398384401","entities":[{"id":"dp017924181030872344","type":"doc-arc","data":{"p1":{"x":285.271848370746,"y":118.08470058053712},"p2":{"x":318.6971243936021,"y":151.5099766033929},"rotation":68.87,"angle2":180,"angle1":0},"style":{"fillColor":[247,31,31,1]}},{"id":"da2248946597254886","data":[{"x":295.9598268557248,"y":119.20837625025047},{"x":308.0091459086233,"y":150.38630093367954}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"fillColor":[247,31,31,1]}}]},{"id":"dg2978327801588845","entities":[{"id":"dp7456470482556339","type":"doc-arc","data":{"p1":{"x":284.4385150374126,"y":118.25136724720372},"p2":{"x":317.8637910602687,"y":151.67664327005943},"rotation":248.87,"angle2":180,"angle1":0},"style":{"fillColor":[70,114,191,1]}},{"id":"da8477314914797089","data":[{"x":307.1758125752898,"y":150.55296760034608},{"x":295.12649352239146,"y":119.37504291691701}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"fillColor":[70,114,191,1]}}],"data":{"rotation":180}},{"id":"ds17463094214994124","type":"polygon-curve","data":[{"p1":{"x":281.75,"y":117.25},"p2":{"x":416.6666666666667,"y":96},"cp":{"dx":31.5,"dy":-25},"cp2":{"dx":3.3333333333333144,"dy":-30}},{"p1":{"x":416.6666666666667,"y":96},"p2":{"x":416.6666666666667,"y":160.66666666666666},"cp":{"dx":-3.3333333333333144,"dy":30},"cp2":{"dx":-9.333333333333371,"dy":-11.333333333333343}},{"p1":{"x":416.6666666666667,"y":160.66666666666666},"p2":{"x":493.33333333333337,"y":126},"cp":{"dx":9.333333333333371,"dy":11.333333333333343},"cp2":{"dx":-21.999999999999943,"dy":-52}},{"p1":{"x":493.33333333333337,"y":126},"p2":{"x":381.25,"y":237.75},"cp":{"dx":21.999999999999886,"dy":52},"cp2":{"dx":43,"dy":10}},{"p1":{"x":381.25,"y":237.75},"p2":{"x":281.75,"y":117.25},"cp":{"dx":-43,"dy":-10},"cp2":{"dx":-31.5,"dy":25}}],"style":{"strokeType":"--","strokeColor":[70,114,191,0.5],"thickness":2}},{"id":"ds014139747602392116","type":"polygon-curve","data":[{"p1":{"x":252,"y":176},"p2":{"x":180.66666666666666,"y":114},"cp":{"dx":-3.3333333333333712,"dy":-29.333333333333343},"cp2":{"dx":-18.666666666666686,"dy":50}},{"p1":{"x":180.66666666666666,"y":114},"p2":{"x":420.6666666666667,"y":79.33333333333333},"cp":{"dx":18.666666666666686,"dy":-50},"cp2":{"dx":-12.666666666666686,"dy":-12.666666666666671}},{"p1":{"x":420.6666666666667,"y":79.33333333333333},"p2":{"x":424,"y":220.66666666666669},"cp":{"dx":12.666666666666686,"dy":12.666666666666671},"cp2":{"dx":10,"dy":-29.333333333333314}},{"p1":{"x":424,"y":220.66666666666669},"p2":{"x":293.41704601787,"y":243.63840736232063},"cp":{"dx":-10,"dy":29.333333333333314},"cp2":{"dx":43,"dy":10}},{"p1":{"x":293.41704601787,"y":243.63840736232063},"p2":{"x":252,"y":176},"cp":{"dx":-43,"dy":-10},"cp2":{"dx":3.3333333333333712,"dy":29.333333333333343}}],"style":{"strokeType":"--","strokeColor":[247,31,31,0.5],"thickness":2}},{"id":"da27354519496507956","data":[{"x":269.3333333333333,"y":62},{"x":294.6666666666667,"y":114.66666666666666}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"style":{"thickness":1,"strokeColor":[0,0,0,1]},"headScale":0.7},{"id":"da12692253565998146","data":[{"x":443,"y":111},{"x":402,"y":188}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"style":{"thickness":1,"strokeColor":[0,0,0,1]},"headScale":0.7}],"settings":{"grid":true},"id":"n0.7664433281450045"}],"id":"n0.9297965813003339"}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":17,"delayRenderCache":{"av":17,"map":{}}}

==> figs/docs/68c4af46-de00-4bb9-9e6b-421cee80a55d <==
{"id":"r0.9600904132466492","lines":[{"id":"n0.23592352158215357","blocks":[]},{"id":"n0.8610334732055211","blocks":[{"id":"n0.6361712915578899","text":"\t"},{"id":"n0.8636753557032222","text":"\\diagram","type":"composite","elements":{"de5477084784861312":{"id":"de5477084784861312","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"k","id":"n0.23700857182319268"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"type":"single","text":"(","id":"n0.6328252767377811"},{"text":"c","id":"n0.11243101382583687"},{"type":"single","text":")","id":"n0.9680921179754931"}],"id":"n0.8925725293292028"}],"id":"n0.04406341491858434"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.7501828463877214"}],"id":"n0.4855857306303264"}],"id":"n0.2168910804010895"}},"id":"n0.8668709801312438"}],"id":"n0.7655701799008161"}],"id":"n0.3977918009086929"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.8246616670886859"}],"id":"n0.42189953978488126"}],"shape":{"data":{"p":{"x":586.2965379192827,"y":70.79321004139163},"rotation":0},"anchor":"center","settings":{"fontSize":"\\footnotesize"}},"isTextMode":true,"isInGroup":false},"de4210769100892233":{"id":"de4210769100892233","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"k","id":"n0.44693986522870155"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.4684634563968568"}],"id":"n0.34823176184676186"}],"id":"n0.49793712128364254"}},"id":"n0.7708019950681051"}],"id":"n0.5485278644299063"}],"id":"n0.37769200352952503"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.5103400268015756"}],"id":"n0.052502982037228696"}],"shape":{"data":{"p":{"x":491.2346588510114,"y":87.55454646995399},"rotation":0},"anchor":"center","settings":{"fontSize":"\\normalsize"}},"isTextMode":true,"isInGroup":false},"de15188357285758025":{"id":"de15188357285758025","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"N","id":"n0.8316999347420186"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.1403580635089423"}],"id":"n0.6785837251656066"}],"id":"n0.253179407928106"}},"id":"n0.33026605475791526"},{"type":"single","text":"(","id":"n0.04003996129602205"},{"text":"k","id":"n0.6963159947439646"},{"id":"n0.2977893335070556","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.5045214043585184","lines":[{"id":"n0.21168863546862005","blocks":[{"id":"n0.30152797339726156","text":"i"}]}]}}},{"type":"single","text":")","id":"n0.12827236617140025"},{"text":"∩A","id":"n0.24737628445281912"},{"text":"\\power","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"type":"single","text":"(","id":"n0.29984732048849416"},{"text":"1","id":"n0.9208986646600794"},{"type":"single","text":")","id":"n0.5491912567910573"}],"id":"n0.5839809114845163"}],"id":"n0.9705054618444722"}},"id":"n0.06509447803636959"}],"id":"n0.5422087484915035"}],"id":"n0.11226648411146756"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.6686761664993313"}],"id":"n0.5646860781639365"}],"shape":{"data":{"p":{"x":471.7870914014861,"y":168.11028603512287},"rotation":0},"anchor":"top","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":false},"de5719517316923577":{"id":"de5719517316923577","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"N","id":"n0.019314248964243053"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.8956744628589475"}],"id":"n0.8027334803913964"}],"id":"n0.012390040409531844"}},"id":"n0.9891788185080737"},{"type":"single","text":"(","id":"n0.0680719505294356"},{"text":"k","id":"n0.515660692162524"},{"id":"n0.2122513082439761","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.927114572331522","lines":[{"id":"n0.6785880880031825","blocks":[{"id":"n0.14482303680466302","text":"i"}]}]}}},{"type":"single","text":")","id":"n0.40336238694354476"},{"text":"∩B","id":"n0.9014617230401747"},{"text":"\\power","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"type":"single","text":"(","id":"n0.8471877617577834"},{"text":"1","id":"n0.8596261776304577"},{"type":"single","text":")","id":"n0.9351702833490201"}],"id":"n0.052147059786393335"}],"id":"n0.6268755506103516"}},"id":"n0.7739229535716532"}],"id":"n0.8861967036577549"}],"id":"n0.15300738993657115"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.7124085964583"}],"id":"n0.32736978052321253"}],"shape":{"data":{"p":{"x":590.166548177304,"y":170.70141050717115},"rotation":0},"anchor":"top","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":false},"de9991240930255139":{"id":"de9991240930255139","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"A","id":"n0.20495779668741365"},{"text":"\\power","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"type":"single","text":"(","id":"n0.3924763154482942"},{"text":"1","id":"n0.05602620015331161"},{"type":"single","text":")","id":"n0.43882943432616184"}],"id":"n0.2892041448684275"}],"id":"n0.8851865347348906"}},"id":"n0.28800447254851336"}],"id":"n0.1887891653877205"}],"id":"n0.5714615488643953"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.8405038664134461"}],"id":"n0.6643971127737158"}],"shape":{"data":{"p":{"x":472.64361697033655,"y":82.97948964593837},"rotation":0},"anchor":"right-bottom"},"isTextMode":true,"isInGroup":false},"de7669520425369756":{"id":"de7669520425369756","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"B","id":"n0.047751094122099325"},{"text":"\\power","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"type":"single","text":"(","id":"n0.346505702670697"},{"text":"1","id":"n0.6788469733493288"},{"type":"single","text":")","id":"n0.6768262797130931"}],"id":"n0.26357034033172555"}],"id":"n0.4787147737522308"}},"id":"n0.24304643671364468"}],"id":"n0.024943852978151382"}],"id":"n0.9749924846764011"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.18458185378970549"}],"id":"n0.7446108349966036"}],"shape":{"data":{"p":{"x":603.5727078160104,"y":105.32793821735486},"rotation":0},"anchor":"bottom-left"},"isTextMode":true,"isInGroup":false},"de6441237021236035":{"id":"de6441237021236035","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.8746424096578092","text":"k"},{"id":"n0.4815754781753583","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.45123662152723565","lines":[{"id":"n0.5767943390609875","blocks":[{"id":"n0.6755137529603965","text":"i"}]}]}}}],"id":"n0.9678571623523362"}],"id":"n0.29185377900883"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.5474884739887464"}],"id":"n0.6902955128635853"}],"shape":{"data":{"p":{"x":60.62216065248679,"y":89.4978898239902},"rotation":0},"anchor":"center","settings":{"fontSize":"\\normalsize"}},"isTextMode":true,"isInGroup":false},"de9759068321357365":{"id":"de9759068321357365","lines":[{"id":"n0.8770593429435007","blocks":[{"id":"n0.8715480407690004","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.1684391717522702","lines":[{"id":"n0.6018364942040022","blocks":[{"text":"N","id":"n0.1409936700351031"},{"id":"n0.9155227077982511","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.14294861783894097","lines":[{"id":"n0.15884970427905842","blocks":[{"id":"n0.24580252217718823","text":"a"}]}]}}},{"id":"n0.9656217788172532","type":"single","text":"("},{"text":"k","id":"n0.3795650513369737"},{"id":"n0.6863200106758056","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.6030402429563784","lines":[{"id":"n0.4935626143277938","blocks":[{"id":"n0.05536407180467351","text":"i"}]}]}}},{"id":"n0.19638210815462442","type":"single","text":")"},{"text":"∩A","id":"n0.12697150035931992"},{"text":"\\power","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"type":"single","text":"(","id":"n0.6861361818381249"},{"text":"1","id":"n0.5489947509152571"},{"type":"single","text":")","id":"n0.2973181527075752"}],"id":"n0.724771913659708"}],"id":"n0.23947105223885035"}},"id":"n0.2645854181282825"}]}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"}}]}],"shape":{"data":{"p":{"x":41.1745932029616,"y":170.05362938915908},"rotation":0},"anchor":"top","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":false},"de3435133745663099":{"id":"de3435133745663099","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"N","id":"n0.5312586502712173"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.7656929635932135"}],"id":"n0.17614173430517632"}],"id":"n0.9409397961334305"}},"id":"n0.6810913838974417"},{"type":"single","text":"(","id":"n0.15558779310976956"},{"text":"k","id":"n0.8484508175111867"},{"id":"n0.907348943004104","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.5007525116806473","lines":[{"id":"n0.35121657772143244","blocks":[{"id":"n0.41802603250147663","text":"i"}]}]}}},{"type":"single","text":")","id":"n0.5389571744489035"},{"text":"∩B","id":"n0.7349415928620417"},{"text":"\\power","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"type":"single","text":"(","id":"n0.11364480894062434"},{"text":"1","id":"n0.3072413966612262"},{"type":"single","text":")","id":"n0.9769147232431148"}],"id":"n0.623936315551604"}],"id":"n0.5309173922421322"}},"id":"n0.37642041850123564"}],"id":"n0.5284858174609459"}],"id":"n0.016086564882261012"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.7422192382340613"}],"id":"n0.4842970082073996"}],"shape":{"data":{"p":{"x":159.5540499787795,"y":172.64475386120736},"rotation":0},"anchor":"top","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":false},"de36992110778251":{"id":"de36992110778251","lines":[{"id":"n0.2512013615748012","blocks":[{"id":"n0.9813331364547291","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.9907098925721369","lines":[{"id":"n0.11330343580445024","blocks":[{"id":"n0.09654383412962031","text":"A"},{"id":"n0.5783030344981395","text":"\\power","type":"composite","elements":{"powerValue":{"id":"n0.3520271110025892","lines":[{"id":"n0.48662611214644214","blocks":[{"id":"n0.46520014894962847","type":"single","text":"("},{"id":"n0.983467071875809","text":"1"},{"id":"n0.15125811609945217","type":"single","text":")"}]}]}}}]}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"}}]}],"shape":{"data":{"p":{"x":43.03111877181209,"y":84.92283299997459},"rotation":0},"anchor":"right-bottom"},"isTextMode":true,"isInGroup":false},"de548357599214798":{"id":"de548357599214798","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.991140521516749","text":"B"},{"text":"\\power","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"type":"single","text":"(","id":"n0.9874165666398829"},{"text":"1","id":"n0.9798570128245527"},{"type":"single","text":")","id":"n0.327298919600042"}],"id":"n0.8746030884715033"}],"id":"n0.6335867858121575"}},"id":"n0.9946117036578648"}],"id":"n0.652792657072601"}],"id":"n0.4034112984198728"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.19497179318812208"}],"id":"n0.19517581507440718"}],"shape":{"data":{"p":{"x":172.9602096174859,"y":107.27128157139109},"rotation":0},"anchor":"bottom-left"},"isTextMode":true,"isInGroup":false},"de170641066039654":{"id":"de170641066039654","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"k","id":"n0.37227140567375283"},{"id":"n0.27813696902377094","text":"\\power-index","type":"composite","elements":{"powerValue":{"id":"n0.6106935622054173","lines":[{"id":"n0.6245959124071079","blocks":[{"id":"n0.6568369394401146","type":"single","text":"("},{"id":"n0.3242943436436809","text":"c"},{"id":"n0.29055120272312007","type":"single","text":")"}]}]},"indexValue":{"id":"n0.4084884940870481","lines":[{"id":"n0.3975757266381903","blocks":[{"id":"n0.8956300959364483","text":"i"}]}]}}}],"id":"n0.400924480113249"}],"id":"n0.14418901364546954"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.83722741348861"}],"id":"n0.9352409978575214"}],"shape":{"data":{"p":{"x":370.909316180269,"y":70.79321004139163},"rotation":0},"anchor":"center","settings":{"fontSize":"\\footnotesize"}},"isTextMode":true,"isInGroup":false},"de5035886710934834":{"id":"de5035886710934834","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"k","id":"n0.07349920584348935"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.9635027420369875"}],"id":"n0.45329487839465377"}],"id":"n0.3766391141254317"}},"id":"n0.9414364712910239"}],"id":"n0.8253889310251645"}],"id":"n0.05068220882975649"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.9826916624532747"}],"id":"n0.8888653614066704"}],"shape":{"data":{"p":{"x":275.8474371119975,"y":87.55454646995399},"rotation":0},"anchor":"center","settings":{"fontSize":"\\normalsize"}},"isTextMode":true,"isInGroup":false},"de8365054714402089":{"id":"de8365054714402089","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"N","id":"n0.9878718955402157"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.1251071952757039"}],"id":"n0.1460418584342047"}],"id":"n0.5546279589650713"}},"id":"n0.36282641362640233"},{"type":"single","text":"(","id":"n0.6968568649071685"},{"text":"k","id":"n0.313206165405455"},{"id":"n0.7628856556627162","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.08448884780830013","lines":[{"id":"n0.029549338617628207","blocks":[{"id":"n0.4885551241312418","text":"i"}]}]}}},{"type":"single","text":")","id":"n0.7059992956771932"},{"text":"∩A","id":"n0.7155363949697109"},{"text":"\\power","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"type":"single","text":"(","id":"n0.36837064792640706"},{"text":"1","id":"n0.05796991167679644"},{"type":"single","text":")","id":"n0.36651266239910285"}],"id":"n0.7785163616211654"}],"id":"n0.18097373321342847"}},"id":"n0.6789816237297166"}],"id":"n0.5788346001979057"}],"id":"n0.5710795725706659"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.7757172289013914"}],"id":"n0.4570319809263661"}],"shape":{"data":{"p":{"x":256.3998696624723,"y":168.11028603512287},"rotation":0},"anchor":"top","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":false},"de7244290037671248":{"id":"de7244290037671248","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"N","id":"n0.33711535314125696"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.7772456954346649"}],"id":"n0.7395841627618198"}],"id":"n0.7646614243636753"}},"id":"n0.6816867947190057"},{"type":"single","text":"(","id":"n0.35980446861218596"},{"text":"k","id":"n0.8424167806369578"},{"id":"n0.361057636687643","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.5522038300973591","lines":[{"id":"n0.38633867531462407","blocks":[{"id":"n0.735457298920881","text":"i"}]}]}}},{"type":"single","text":")","id":"n0.32178471695211885"},{"text":"∩B","id":"n0.33904776862491315"},{"text":"\\power","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"type":"single","text":"(","id":"n0.19944313802114677"},{"text":"1","id":"n0.3148761542209706"},{"type":"single","text":")","id":"n0.9014601136207931"}],"id":"n0.43127677971974454"}],"id":"n0.7049744412493093"}},"id":"n0.2078583471549691"}],"id":"n0.6307344150447967"}],"id":"n0.5497238752341633"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.8096197706441948"}],"id":"n0.28926206098682994"}],"shape":{"data":{"p":{"x":374.77932643829024,"y":170.70141050717115},"rotation":0},"anchor":"top","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":false},"de8635436804851921":{"id":"de8635436804851921","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"A","id":"n0.911122658712662"},{"text":"\\power","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"type":"single","text":"(","id":"n0.5756122103057777"},{"text":"1","id":"n0.43036123774079105"},{"type":"single","text":")","id":"n0.7480991198470348"}],"id":"n0.0791685310746324"}],"id":"n0.18584126435611292"}},"id":"n0.8054555694655776"}],"id":"n0.9398242046977547"}],"id":"n0.5904548957516162"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.11502045148806372"}],"id":"n0.9841908745772543"}],"shape":{"data":{"p":{"x":257.2563952313228,"y":82.97948964593837},"rotation":0},"anchor":"right-bottom"},"isTextMode":true,"isInGroup":false},"de5383743483289485":{"id":"de5383743483289485","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"B","id":"n0.993247697153768"},{"text":"\\power","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"type":"single","text":"(","id":"n0.32085474796245705"},{"text":"1","id":"n0.3897465216402827"},{"type":"single","text":")","id":"n0.4939196480344814"}],"id":"n0.4217607333837714"}],"id":"n0.006605753780423385"}},"id":"n0.6582060267498833"}],"id":"n0.6504009888845783"}],"id":"n0.691135733822869"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.3571563125596746"}],"id":"n0.3278972769362216"}],"shape":{"data":{"p":{"x":388.18548607699665,"y":105.32793821735486},"rotation":0},"anchor":"bottom-left"},"isTextMode":true,"isInGroup":false},"de4701755302559858":{"id":"de4701755302559858","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"G","id":"n0.6917363963992815"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"type":"single","text":"(","id":"n0.3262365864545045"},{"text":"1","id":"n0.7771389332987639"},{"type":"single","text":")","id":"n0.8476171854628376"}],"id":"n0.9439986868056407"}],"id":"n0.21585585087966241"},"indexValue":{"id":"n0.7076156488818364","lines":[{"id":"n0.5872389328203143","blocks":[{"id":"n0.38059894257468896","text":"i"}]}]}},"id":"n0.024083197345851293"}],"id":"n0.893137613127712"}],"id":"n0.06813144124957105"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.9057093942707122"}],"id":"n0.27244707340095276"}],"shape":{"data":{"p":{"x":315.5583333333334,"y":220.5048872180451},"rotation":0},"anchor":"center"},"isTextMode":true,"isInGroup":true},"de528190398203549":{"id":"de528190398203549","lines":[{"id":"n0.9056319969674991","blocks":[{"id":"n0.42280523304044926","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.6235698046106921","lines":[{"id":"n0.2634887327098274","blocks":[{"id":"n0.2419702575711884","text":"G"},{"id":"n0.39077384155815165","text":"\\power-index","type":"composite","elements":{"powerValue":{"id":"n0.4346659947387168","lines":[{"id":"n0.5537877709330761","blocks":[{"id":"n0.5046050840217706","type":"single","text":"("},{"id":"n0.720070616563901","text":"1"},{"id":"n0.9027493563983588","type":"single","text":")"}]}]},"indexValue":{"id":"n0.4536969038167262","lines":[{"id":"n0.9246437663929514","blocks":[{"id":"n0.06996750529780016","text":"i-1"}]}]}}}]}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"}}]}],"shape":{"data":{"p":{"x":96.49166666666667,"y":220.5048872180451},"rotation":0},"anchor":"center"},"isTextMode":true,"isInGroup":true},"de18319978451090724":{"id":"de18319978451090724","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"(G","id":"n0.10057520804296516"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"type":"single","text":"(","id":"n0.5012725885732676"},{"text":"1","id":"n0.6234263358946366"},{"type":"single","text":")","id":"n0.6472053203697818"}],"id":"n0.8528772445312554"}],"id":"n0.24036995429300645"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.22879305734210176"}],"id":"n0.3331666838168863"}],"id":"n0.8539623852702274"}},"id":"n0.5615445733475295"},{"type":"single","text":")","id":"n0.5106507636453466"},{"text":"'","id":"n0.43928164106845324"}],"id":"n0.6456629570665271"}],"id":"n0.3998820809210015"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.2705640226327577"}],"id":"n0.33940094243718333"}],"shape":{"data":{"p":{"x":531.8333333333334,"y":220.5048872180451},"rotation":0},"anchor":"center"},"isTextMode":true,"isInGroup":true}},"connections":[],"intersections":{"id":"di9833419058199953","items":[],"style":{}},"shapes":[{"id":"dp7439272634554253","type":"circle","data":{"p1":{"x":105.72392099407732,"y":97.83807171839557},"p2":{"x":207.58750180147555,"y":199.7016525257938}},"style":{"strokeColor":"none","fillColor":[208,2,27,0.3]}},{"id":"dp10297461440893652","type":"ellipse","data":{"p1":{"x":-24.96421929405972,"y":91.79378724807975},"p2":{"x":124.67396871802137,"y":179.67511523503515},"rotation":288.4},"style":{"fillColor":[74,144,226,0.3],"strokeColor":"none"}},{"id":"dp5058737271039968","type":"ellipse","data":{"p1":{"x":49.81657294377052,"y":78.69230211527398},"p2":{"x":71.42774836120307,"y":100.30347753270644},"flipX":true},"style":{"thickness":2}},{"id":"dp965310266595484","type":"ellipse","data":{"p1":{"x":132.5258647518268,"y":124.64001547614505},"p2":{"x":180.78555804372613,"y":172.89970876804435},"rotation":302.75},"style":{"strokeColor":[0,0,0,1],"fillColor":[208,2,27,0.7]}},{"id":"da4275499712342943","data":[{"x":71.42774836120307,"y":89.4978898239902},{"x":144.5,"y":128}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da2613172347348214","data":[{"x":70.3388774226679,"y":94.03235765007472},{"x":133.5,"y":147.5}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"dp7602249295601631","type":"ellipse","data":{"p1":{"x":26.550330604581415,"y":133.3887890928006},"p2":{"x":62.95962864927965,"y":169.7980871374989},"rotation":280.96},"style":{"strokeColor":[0,0,0,1],"fillColor":[74,144,226,0.7]}},{"id":"da12389357378659827","data":[{"x":54.14434947236613,"y":98.24293491715315},{"x":35.358697050016055,"y":135.8952124016048}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da5265498589195854","data":[{"x":60.62216065248679,"y":100.30347753270644},{"x":60.62216065248683,"y":141.72524246371344}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"dp6845487302950799","type":"ellipse","data":{"p1":{"x":360.1037284715527,"y":59.9876223326754},"p2":{"x":381.71490388898525,"y":81.59879775010785},"flipX":true},"style":{"thickness":2}},{"id":"dp15280769790455428","type":"ellipse","data":{"p1":{"x":320.9491974535881,"y":95.89472836435935},"p2":{"x":422.8127782609863,"y":197.7583091717576}},"style":{"strokeColor":"none","fillColor":[208,2,27,0.3]}},{"id":"dp6971124682263525","type":"ellipse","data":{"p1":{"x":190.2610571654509,"y":89.85044389404345},"p2":{"x":339.89924517753207,"y":177.73177188099896},"rotation":288.4},"style":{"fillColor":[74,144,226,0.3],"strokeColor":"none"}},{"id":"dp5182294928261728","type":"ellipse","data":{"p1":{"x":265.0418494032812,"y":76.74895876123776},"p2":{"x":286.65302482071377,"y":98.36013417867021},"flipX":true},"style":{"thickness":2}},{"id":"dp15859450319654744","type":"circle","data":{"p1":{"x":347.75114121133754,"y":122.69667212210881},"p2":{"x":396.0108345032369,"y":170.95636541400816},"rotation":302.75},"style":{"strokeColor":[0,0,0,1],"fillColor":[208,2,27,0.7]}},{"id":"dp5216472331201056","type":"ellipse","data":{"p1":{"x":241.77560706409207,"y":131.4454457387643},"p2":{"x":278.1849051087905,"y":167.8547437834627},"rotation":280.96},"style":{"strokeColor":[0,0,0,1],"fillColor":[74,144,226,0.7]}},{"id":"da4625491934508261","data":[{"x":375.3142277827512,"y":81.22248604138599},{"x":384.9346188907706,"y":126.5323763619668}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da3719778997489085","data":[{"x":368.31819170822075,"y":81.61115471219324},{"x":362.74727409331695,"y":125.14204584260443}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da11818921215391565","data":[{"x":211.87905170830552,"y":40.83333333333334},{"x":211.87905170830552,"y":239.0543554450272}],"head":"no","tail":"no","shaft":"--","mVer":1,"style":{"thickness":2,"strokeColor":[155,155,155,1]}},{"id":"da6171872740924502","data":[{"x":427.5901640063253,"y":40.83333333333334},{"x":427.5901640063253,"y":239.0543554450272}],"head":"no","tail":"no","shaft":"--","mVer":1,"style":{"thickness":2,"strokeColor":[155,155,155,1]}},{"id":"dp9150254716943744","type":"ellipse","data":{"p1":{"x":575.4909502105664,"y":59.9876223326754},"p2":{"x":597.102125627999,"y":81.59879775010785},"flipX":true},"style":{"thickness":2}},{"id":"dp0006011602728090981","type":"ellipse","data":{"p1":{"x":536.336419192602,"y":95.89472836435935},"p2":{"x":638.2,"y":197.7583091717576}},"style":{"strokeColor":"none","fillColor":[208,2,27,0.3]}},{"id":"dp44283206540690423","type":"ellipse","data":{"p1":{"x":405.6482789044648,"y":89.85044389404356},"p2":{"x":555.2864669165458,"y":177.73177188099916},"rotation":288.4},"style":{"fillColor":[74,144,226,0.3],"strokeColor":"none"}},{"id":"dp8262005611246444","type":"ellipse","data":{"p1":{"x":480.429071142295,"y":76.74895876123776},"p2":{"x":502.0402465597277,"y":98.36013417867021},"flipX":true},"style":{"thickness":2}},{"id":"dp5797081248511038","type":"ellipse","data":{"p1":{"x":563.1383629503513,"y":122.69667212210878},"p2":{"x":611.3980562422506,"y":170.95636541400827},"rotation":302.75},"style":{"strokeColor":[0,0,0,1],"fillColor":[208,2,27,0.7]}},{"id":"dp3041916380646521","type":"ellipse","data":{"p1":{"x":457.16282880310587,"y":131.4454457387644},"p2":{"x":493.57212684780427,"y":167.85474378346268},"rotation":280.96},"style":{"strokeColor":[0,0,0,1],"fillColor":[74,144,226,0.7]}},{"id":"da09078445625578802","data":[{"x":269.165552777054,"y":96.68826023392418},{"x":250.37990035470392,"y":134.34053771837586}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da6575094037045488","data":[{"x":275.64336395717464,"y":98.74880284947747},{"x":275.6433639571747,"y":140.17056778048448}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da887960745624137","data":[{"x":484.8766650750739,"y":96.68826023392418},{"x":466.0910126527238,"y":134.34053771837586}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da3864456176443334","data":[{"x":491.3544762551946,"y":98.74880284947747},{"x":491.3544762551946,"y":140.17056778048448}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da8254390891756558","data":[{"x":589.8593340683492,"y":81.22248604138599},{"x":599.4797251763686,"y":126.5323763619668}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da8641322126271846","data":[{"x":582.8632979938187,"y":81.61115471219324},{"x":577.2923803789149,"y":125.14204584260443}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da9143318761014485","data":[{"x":44.95596102516692,"y":127.17849563142369},{"x":55,"y":129.25}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":1}},{"id":"da7048525481313153","data":[{"x":124.5,"y":134.25},{"x":131.37808363381473,"y":124.73515227738751}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":1}},{"id":"da7274283541797011","data":[{"x":368.34652003120254,"y":114.51843550720642},{"x":381.6260329504501,"y":114.51843550720648}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":1}},{"id":"da5819060643924989","data":[{"x":582.6142889751862,"y":114.51843550720639},{"x":595.8938018944338,"y":114.51843550720645}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":1}},{"id":"da3039190956512947","data":[{"x":259.9559610251669,"y":125.67849563142369},{"x":270,"y":127.75}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":1}},{"id":"da6498923870702062","data":[{"x":475.9559610251669,"y":125.67849563142369},{"x":486,"y":127.75}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":1}},{"id":"da4879143249039055","data":[{"x":339,"y":132.75},{"x":345.87808363381475,"y":123.2351522773875}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":1}},{"id":"da41016519570898313","data":[{"x":286.42774836120304,"y":87.9978898239902},{"x":359.5,"y":126.5}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da001905187312601031","data":[{"x":285.3388774226679,"y":92.53235765007472},{"x":348.5,"y":146}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"dg39045868041654397","entities":[{"id":"dp9032223267392154","type":"doc-rounded-rect","data":{"p1":{"x":77.36666666666667,"y":205.54999999999998},"p2":{"x":115.61666666666667,"y":235.45977443609024}},"style":{"fillColor":[155,155,155,0.5]}},{"id":"dl5733728347228726","linkedId":"de528190398203549"}]},{"id":"dg3416030564471595","entities":[{"id":"dp5122081605074942","type":"doc-rounded-rect","data":{"p1":{"x":296.4333333333334,"y":205.54999999999998},"p2":{"x":334.6833333333334,"y":235.4597744360902}},"style":{"fillColor":[155,155,155,0.5]}},{"id":"dl05855798232486231","linkedId":"de4701755302559858"}]},{"id":"dg5036373141853545","entities":[{"id":"dp685368320348354","type":"doc-rounded-rect","data":{"p1":{"x":508.66666666666663,"y":205.54999999999998},"p2":{"x":555,"y":235.4597744360902}},"style":{"fillColor":[155,155,155,0.5]}},{"id":"dl6824393491960634","linkedId":"de18319978451090724"}]}],"settings":{"grid":true}}]},{"id":"n0.4366202696179722","blocks":[],"style":null}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":1013,"delayRenderCache":{"av":1013,"map":{}}}

==> figs/docs/6c3ee879-723a-45da-becd-12608393d3db <==
{"id":"r0.06735421054204804","lines":[{"blocks":[{"text":"\\diagram","type":"composite","elements":{"de345569061800336":{"id":"de345569061800336","lines":[{"blocks":[{"text":"1","id":"n0.29251927413831424"}],"id":"n0.049943145334872874"}],"shape":{"data":{"p":{"x":128.8643076797487,"y":153.30550394860256},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de9609572224981677":{"id":"de9609572224981677","lines":[{"blocks":[{"text":"2","id":"n0.8620186571624497"}],"id":"n0.6379535734683317"}],"shape":{"data":{"p":{"x":65.72367457392377,"y":60.256149897913346},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de37168216021499334":{"id":"de37168216021499334","lines":[{"blocks":[{"text":"3","id":"n0.38764013199022584"}],"id":"n0.2017170134046684"}],"shape":{"data":{"p":{"x":66.83140497928915,"y":256.32443164757996},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de3371895549164241":{"id":"de3371895549164241","lines":[{"blocks":[{"text":"4","id":"n0.2068903913772666"}],"id":"n0.21851565719017363"}],"shape":{"data":{"p":{"x":240.7450786216489,"y":54.71749787108662},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de65488930736744":{"id":"de65488930736744","lines":[{"blocks":[{"text":"5","id":"n0.8836909389355077"}],"id":"n0.5722976062884864"}],"shape":{"data":{"p":{"x":347.0871975367224,"y":145.55139111104518},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de15796909924404012":{"id":"de15796909924404012","lines":[{"blocks":[{"text":"6","id":"n0.3549924094031196"}],"id":"n0.7650859410607105"}],"shape":{"data":{"p":{"x":251.82238267530238,"y":245.24712759392654},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de43775475014727006":{"id":"de43775475014727006","lines":[{"blocks":[{"text":"7","id":"n0.3051781463947183"}],"id":"n0.11249227132161677"}],"shape":{"data":{"p":{"x":357.0567711850105,"y":296.2027262407325},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de9896426970245582":{"id":"de9896426970245582","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"*","id":"n0.17817658159901129"}],"id":"n0.42834572353008404"}],"id":"n0.7879123135941577"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.03805204370492832"}],"id":"n0.5333726743740843"}],"shape":{"data":{"p":{"x":127.33333333333331,"y":111.66666666666667}},"anchor":"left-top"},"isTextMode":true},"de16564388907577676":{"id":"de16564388907577676","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.39600668305400877","text":"e"},{"id":"n0.594477899446666","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.39777562947591916","lines":[{"id":"n0.4161833037827043","blocks":[{"id":"n0.15857280009555685","text":"1"}]}]}}}],"id":"n0.14205851465202368"}],"id":"n0.8651404849746063"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.6809308936156713"}],"id":"n0.1889993265701786"}],"shape":{"data":{"p":{"x":66,"y":19.00000000000003}},"anchor":"left-top","style":{"textColor":[247,31,31,1]}},"isTextMode":true},"de217727765680936":{"id":"de217727765680936","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.4998949332761944","text":"e"},{"id":"n0.7712090544856323","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.1938053597840339","lines":[{"id":"n0.7895322139056342","blocks":[{"id":"n0.5118338695865323","text":"0"}]}]}}}],"id":"n0.6233749437168543"}],"id":"n0.39154144287226944"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.8211708262419024"}],"id":"n0.8502731843320026"}],"shape":{"data":{"p":{"x":61.245570604444836,"y":296.5178666040418}},"anchor":"left-top","style":{"textColor":[70,114,191,1]}},"isTextMode":true},"de320786155654154":{"id":"de320786155654154","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"e","id":"n0.08347060050772992"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.16046876852384484","text":"1"}],"id":"n0.5790916181442054"}],"id":"n0.6437500611936995"}},"id":"n0.2969281662112355"}],"id":"n0.970585659679829"}],"id":"n0.08292384504071015"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.01683043364888759"}],"id":"n0.7786172433552387"}],"shape":{"data":{"p":{"x":238.33333333333334,"y":13.333333333333329}},"anchor":"left-top","style":{"textColor":[247,31,31,1]}},"isTextMode":true},"de20101408233961982":{"id":"de20101408233961982","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"*","id":"n0.9735430907654603"}],"id":"n0.526650490226767"}],"id":"n0.6783346917071056"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.765784494345332"}],"id":"n0.2138594831675258"}],"shape":{"data":{"p":{"x":252.33333333333334,"y":282.66666666666663}},"anchor":"left-top"},"isTextMode":true},"de23060147202727577":{"id":"de23060147202727577","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.2330556974058262","text":"*"}],"id":"n0.9535237492543718"}],"id":"n0.3911255050149658"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.9264758215706481"}],"id":"n0.7721568702856969"}],"shape":{"data":{"p":{"x":385.33333333333337,"y":143}},"anchor":"left-top","style":{"textColor":[0,0,0,1]}},"isTextMode":true},"de592032626246557":{"id":"de592032626246557","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"e","id":"n0.988357328449528"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"0","id":"n0.7004849444264858"}],"id":"n0.4052250465647862"}],"id":"n0.6699485180142482"}},"id":"n0.798992467141352"}],"id":"n0.842770445251378"}],"id":"n0.8280817013149768"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.8858576894371559"}],"id":"n0.8741488377319735"}],"shape":{"data":{"p":{"x":399.3333333333333,"y":294.99999999999994}},"anchor":"left-top","style":{"textColor":[70,114,191,1]}},"isTextMode":true}},"connections":[],"intersections":{"id":"di018738070182718003","items":[],"style":{}},"shapes":[{"id":"dp36011981252403324","type":"ellipse","data":{"p1":{"x":44.95402865523873,"y":42.85625299199422},"p2":{"x":100.49332049260892,"y":98.39554482936434}},"style":{"fillColor":"none"}},{"id":"dp9944525012609338","type":"ellipse","data":{"p1":{"x":45.52895517377332,"y":238.64630089431083},"p2":{"x":101.06824701114326,"y":294.1855927316803},"rotation":12.59},"style":{"fillColor":"none"}},{"id":"dp6959252434549423","type":"ellipse","data":{"p1":{"x":108.38664482631847,"y":135.74529364125738},"p2":{"x":163.92593666368901,"y":191.28458547862738},"rotation":11.34},"style":{"fillColor":[255,255,255,1]}},{"id":"dp19065636230997107","type":"ellipse","data":{"p1":{"x":336.79390961187244,"y":278.949097787917},"p2":{"x":392.33320144924306,"y":334.4883896252872},"rotation":1.24},"style":{"fillColor":"none"}},{"id":"dp18557568518611567","type":"ellipse","data":{"p1":{"x":231.22913809978522,"y":228.00619298050708},"p2":{"x":286.7684299371551,"y":283.5454848178769},"rotation":312.14},"style":{"fillColor":"none"}},{"id":"dp9745215057428975","type":"ellipse","data":{"p1":{"x":219.72524418472122,"y":37.96336472513116},"p2":{"x":275.26453602209136,"y":93.50265656250127}},"style":{"fillColor":"none"}},{"id":"dp8575189176443259","type":"ellipse","data":{"p1":{"x":325.31306594751015,"y":128.5497234540565},"p2":{"x":380.85235778488016,"y":184.0890152914266}},"style":{"fillColor":"none"}},{"id":"da3887442655264841","data":[{"x":66.0772921417317,"y":239.0773063107636},{"x":66.0772921417317,"y":97.28781442399901}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"da811568196747092","data":[{"x":120.3560820046338,"y":185.9062468532269},{"x":91.55509146513478,"y":245.7236887429557}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"da9587227521276189","data":[{"x":87.12416984367336,"y":95.07235361326829},{"x":119.24835159926843,"y":142.7047610439783}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"da538871014198508","data":[{"x":359.62584956354925,"y":183.69078604249617},{"x":365.16450159037583,"y":278.9556009039161}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"da8208323338758907","data":[{"x":149.15707254413283,"y":139.38156982788226},{"x":220.05181848751522,"y":72.91774550596136}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"da10418561169836504","data":[{"x":275.4383387557826,"y":71.81001510059599},{"x":346.33308469916494,"y":129.4119961795941}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"da9511932409531874","data":[{"x":284.854047201388,"y":244.06209313490763},{"x":341.3482978750208,"y":180.92146002908285}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"da28413184061019403","data":[{"x":158.57278098973836,"y":180.92146002908285},{"x":233.34458335189936,"y":244.06209313490763}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}}],"settings":{"grid":true,"diagramHeight":358.6640625},"id":"n0.45728395049338477"}],"id":"n0.31644194418568916"}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":45,"delayRenderCache":{"av":45,"map":{}}}

==> figs/docs/7e77001c-f3e4-48ad-87a1-ea2c986bc5e6 <==
{"id":"r0.5827846549346337","lines":[{"blocks":[{"text":"\\diagram","type":"composite","elements":{},"connections":[],"intersections":{"id":"di018738070182718003","items":[],"style":{}},"shapes":[{"id":"dp038687753522042456","type":"ellipse","data":{"p1":{"x":49.620695321905416,"y":47.57472397714416},"p2":{"x":83.04597134476127,"y":81}},"style":{"fillColor":"none"}},{"id":"dp9056051655118029","type":"ellipse","data":{"p1":{"x":49.96670401123383,"y":165.40727418009203},"p2":{"x":83.39198003408957,"y":198.83255020294786},"rotation":12.59},"style":{"fillColor":"none"}},{"id":"dp9920647236382272","type":"ellipse","data":{"p1":{"x":87.7964198266168,"y":103.4782423779815},"p2":{"x":121.22169584947291,"y":136.9035184008373},"rotation":11.34},"style":{"fillColor":[255,255,255,1]}},{"id":"dp2486947949659155","type":"ellipse","data":{"p1":{"x":225.2590272620554,"y":189.6627528888692},"p2":{"x":258.68430328491115,"y":223.08802891172502},"rotation":1.24},"style":{"fillColor":"none"}},{"id":"dp9568864361706426","type":"ellipse","data":{"p1":{"x":161.72685914559003,"y":159.00372577019766},"p2":{"x":195.15213516844568,"y":192.42900179305337},"rotation":312.14},"style":{"fillColor":"none"}},{"id":"dp10976789485208438","type":"ellipse","data":{"p1":{"x":154.80345741092947,"y":44.630031391797814},"p2":{"x":188.22873343378535,"y":78.05530741465364}},"style":{"fillColor":"none"}},{"id":"dp2257479211072284","type":"ellipse","data":{"p1":{"x":218.349497886343,"y":99.14772407837313},"p2":{"x":251.77477390919876,"y":132.57300010122896}},"style":{"fillColor":"none"}},{"id":"da9150526298104995","data":[{"x":62.33333333333333,"y":165.66666666666669},{"x":62.33333333333333,"y":80.33333333333334}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"da9038999327165957","data":[{"x":95.00000000000001,"y":133.66666666666669},{"x":77.6666666666667,"y":169.66666666666669}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"da7471967574334728","data":[{"x":75.00000000000001,"y":79},{"x":94.33333333333333,"y":107.66666666666667}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"da1181282131296919","data":[{"x":239.00000000000003,"y":132.33333333333334},{"x":242.33333333333331,"y":189.66666666666666}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"da08800419790132863","data":[{"x":112.33333333333333,"y":105.66666666666667},{"x":155,"y":65.66666666666667}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"da3877584245036687","data":[{"x":188.33333333333331,"y":65},{"x":231,"y":99.66666666666667}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"da48790371843673563","data":[{"x":194,"y":168.66666666666669},{"x":228,"y":130.66666666666669}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"da7637462449050694","data":[{"x":118.00000000000001,"y":130.66666666666669},{"x":163,"y":168.66666666666669}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}}],"settings":{"grid":true},"id":"n0.7564473742482591"}],"id":"n0.11586596050473719"}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":60,"delayRenderCache":{"av":60,"map":{}}}

==> figs/docs/805b23af-dfca-4b4d-924b-216c40cac3f1 <==
{"id":"r0.06447784081131613","lines":[{"id":"n0.6958009661950187","blocks":[]},{"id":"n0.5802418297710987","blocks":[{"id":"n0.7824124239150971","text":"\\diagram","type":"composite","elements":{"de7539823193538859":{"id":"de7539823193538859","lines":[{"id":"n0.08014479918717932","blocks":[{"id":"n0.9985200338754372","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.6952138247091006","lines":[{"id":"n0.9130539483654345","blocks":[{"id":"n0.6315630854692653","text":"e"},{"id":"n0.5782267926995655","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.6356188371790841","lines":[{"id":"n0.10621084901862599","blocks":[{"id":"n0.40996684915721393","text":"0"}]}]}}}]}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"}}]}],"shape":{"data":{"p":{"x":259.6,"y":124.80000000000007}},"anchor":"left-top"},"isTextMode":true},"de16515664730593693":{"id":"de16515664730593693","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"e","id":"n0.3966912367426785","style":{"mathModeType":"\\displaystyle"}},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.9600081056242173","text":"1"}],"id":"n0.7485215301854227"}],"id":"n0.5709108356939625"}},"id":"n0.4272596364792207","style":{"mathModeType":"\\displaystyle"}}],"id":"n0.43550984913778024"}],"id":"n0.12565817041890637"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.15944771819164227"}],"id":"n0.36677066475039277"}],"shape":{"data":{"p":{"x":132.00000000000006,"y":124.87343750000002}},"anchor":"left-top"},"isTextMode":true},"de465268162439717":{"id":"de465268162439717","lines":[{"id":"n0.09594209007453736","blocks":[{"id":"n0.7012580866856746","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.12044731579497725","lines":[{"id":"n0.7633771217606173","blocks":[{"id":"n0.1474459203244698","text":"-"}]}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"}}]}],"shape":{"data":{"p":{"x":197,"y":64}},"anchor":"left-top"},"isTextMode":true},"de4569815697933115":{"id":"de4569815697933115","lines":[{"id":"n0.3802376108478056","blocks":[{"id":"n0.5347419692074553","text":"GATE"},{"id":"n0.8034087534891119","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.8435814039907137","lines":[{"id":"n0.6731924666357483","blocks":[{"id":"n0.9276801159889791","text":"="}]}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"}}]}],"shape":{"data":{"p":{"x":17,"y":63}},"anchor":"left-top"},"isTextMode":true}},"connections":[],"intersections":{"id":"di007212778813125098","items":[],"style":{}},"shapes":[{"id":"dp5515081758440936","type":"ellipse","data":{"p1":{"x":96.10206044514979,"y":28.902060445149743},"p2":{"x":186.20000000000005,"y":119.00000000000006}}},{"id":"dp14139987799020592","type":"circle","data":{"p1":{"x":154.68580451798374,"y":39.51448038176201},"p2":{"x":164.28006934522807,"y":49.108745209006344}},"style":{"fillColor":[247,31,31,1]}},{"id":"dp21801246682419317","type":"circle","data":{"p1":{"x":112.11125434708697,"y":44.31161279538418},"p2":{"x":121.7055191743313,"y":53.90587762262852},"rotation":318.91},"style":{"fillColor":[247,31,31,1]}},{"id":"dp4817496353253219","type":"ellipse","data":{"p1":{"x":169.0772017588502,"y":75.13318855290663},"p2":{"x":178.67146658609454,"y":84.72745338015093}},"style":{"fillColor":[247,31,31,1]}},{"id":"dp29955759079511446","type":"circle","data":{"p1":{"x":136.35389780895275,"y":69.15389780895273},"p2":{"x":145.94816263619708,"y":78.74816263619707}},"style":{"fillColor":[247,31,31,1]}},{"id":"dp32099155351946096","type":"ellipse","data":{"p1":{"x":140.29440727711722,"y":106.07469262076955},"p2":{"x":149.88867210436155,"y":115.66895744801391}},"style":{"fillColor":[247,31,31,1]}},{"id":"dp6119022969400278","type":"ellipse","data":{"p1":{"x":104.91555572665375,"y":78.49118124244208},"p2":{"x":114.50982055389807,"y":88.0854460696865},"rotation":346.98},"style":{"fillColor":[247,31,31,1]}},{"id":"dg16696458363259992","entities":[{"id":"da8432750619144531","data":[{"x":156.8445141041137,"y":48.38917534696303},{"x":144.37196982869608,"y":69.97627120826277}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da8305595034520126","data":[{"x":120.0612718855516,"y":52.72423892126359},{"x":137.65598444962504,"y":70.93569769098721}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da5181339419709687","data":[{"x":169.0772017588502,"y":78.49118124244211},{"x":145.5712529321016,"y":75.13318855290663}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da6160864595078592","data":[{"x":114.38649339222201,"y":82.20756213017796},{"x":136.9364145875817,"y":76.33247165631215}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da7741186466284198","data":[{"x":141.15103022257495,"y":78.74816263619707},{"x":145.09153969073938,"y":106.07469262076955}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}}],"data":{"rotation":0}},{"id":"dp08168290511338117","type":"ellipse","data":{"p1":{"x":279.64544786854583,"y":40.42602022404401},"p2":{"x":289.06933339744626,"y":49.84990575294438}},"style":{"fillColor":[70,114,191,1]}},{"id":"dp584819553767451","type":"ellipse","data":{"p1":{"x":237.8269558340503,"y":45.137962988494195},"p2":{"x":247.25084136295072,"y":54.561848517394594},"rotation":318.91},"style":{"fillColor":[70,114,191,1]}},{"id":"dp41258489003116305","type":"ellipse","data":{"p1":{"x":293.78127616189647,"y":75.41219525008674},"p2":{"x":303.2051616907968,"y":84.83608077898714}},"style":{"fillColor":[70,114,191,1]}},{"id":"dp31569977708636165","type":"ellipse","data":{"p1":{"x":261.63908745812466,"y":69.53908745812478},"p2":{"x":271.06297298702503,"y":78.96297298702518}},"style":{"fillColor":[70,114,191,1]}},{"id":"dp2516189185637272","type":"ellipse","data":{"p1":{"x":265.50961957519525,"y":105.8042260807905},"p2":{"x":274.9335051040957,"y":115.2281116096909}},"style":{"fillColor":[70,114,191,1]}},{"id":"dp47485880980817674","type":"ellipse","data":{"p1":{"x":230.75904168737497,"y":78.71055518520183},"p2":{"x":240.1829272162754,"y":88.13444071410225},"rotation":346.98},"style":{"fillColor":[70,114,191,1]}},{"id":"da25524538414468756","data":[{"x":281.76582211254845,"y":49.14311433827686},{"x":269.51477092497794,"y":70.34685677830277}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da6866464126206429","data":[{"x":245.63579336191327,"y":53.40119389104319},{"x":262.9180510547477,"y":71.2892453311928}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da5424882641513622","data":[{"x":293.78127616189647,"y":78.71055518520186},{"x":270.6927566160905,"y":75.41219525008674}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da14833700695082053","data":[{"x":240.0617901541694,"y":82.36093889864318},{"x":262.21125964008013,"y":76.59018094119926}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da6557815116701942","data":[{"x":266.3510302225749,"y":78.96297298702518},{"x":270.22156233964546,"y":105.8042260807905}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"dp4428607604787118","type":"ellipse","data":{"p1":{"x":222.10206044514968,"y":30.002060445149766},"p2":{"x":310.6,"y":118.5000000000002}}}],"settings":{"grid":true,"diagramHeight":170.265625,"gridBold":false,"gridSize":10}}]},{"id":"n0.8281830687032437","blocks":[],"style":null}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":236,"delayRenderCache":{"av":236,"map":{}}}

==> figs/docs/859e6e39-50f6-43ab-9fe4-767623f6f1e7 <==
{"id":"r0.050871064024779145","lines":[{"id":"n0.952291796451851","blocks":[]},{"id":"n0.6536761371441988","blocks":[{"id":"n0.4664334835344386","text":"\\diagram","type":"composite","elements":{"de8037801504579731":{"id":"de8037801504579731","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"i","id":"n0.25555225797153747"}],"id":"n0.7597639830703928"}],"id":"n0.4490628176749656"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.2328516892563417"}],"id":"n0.9367820800857416"}],"shape":{"data":{"p":{"x":217.16666666666663,"y":22.166666666666686}},"anchor":"left-top"},"isTextMode":true},"de35506470128654444":{"id":"de35506470128654444","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"j","id":"n0.9495862905544359"}],"id":"n0.2418041383753795"}],"id":"n0.3926618893090972"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.007073801323990603"}],"id":"n0.1699476608981303"}],"shape":{"data":{"p":{"x":427,"y":62}},"anchor":"left-top"},"isTextMode":true},"de7048065826810717":{"id":"de7048065826810717","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"e","id":"n0.6657652082706871"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.5758874241013405","text":"0"}],"id":"n0.7107270297259194"}],"id":"n0.27232266808303485"}},"id":"n0.592380102955145"}],"id":"n0.7006161876818566"}],"id":"n0.25417225338754745"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.9062547844620807"}],"id":"n0.20608115605915733"}],"shape":{"data":{"p":{"x":173,"y":55.33333333333334}},"anchor":"left-top","style":{"textColor":[70,114,191,0.7],"strokeColor":[247,31,31,0.7]}},"isTextMode":true},"de9969575487545663":{"id":"de9969575487545663","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"e","id":"n0.06965983447743018"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.9587253483153813","text":"1"}],"id":"n0.24066866141078003"}],"id":"n0.15330792825568906"}},"id":"n0.4968586311882872"}],"id":"n0.8755504557689089"}],"id":"n0.5516280020256239"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.33071019953462066"}],"id":"n0.003414493639377403"}],"shape":{"data":{"p":{"x":447.00000000000006,"y":188.66666666666669}},"anchor":"left-top","style":{"textColor":[247,31,31,0.7]}},"isTextMode":true}},"connections":[],"intersections":{"id":"di018738070182718003","items":[],"style":{}},"shapes":[{"id":"dp6278273965868246","type":"ellipse","data":{"p1":{"x":135.29440727711722,"y":186.99030499710676},"p2":{"x":168.71968329997304,"y":220.4155810199626}},"style":{"fillColor":[70,114,191,1]}},{"id":"dp3888594191770549","type":"ellipse","data":{"p1":{"x":174.25037935120338,"y":90.42576935089271},"p2":{"x":207.6756553740592,"y":123.85104537374855}},"style":{"fillColor":[70,114,191,1]}},{"id":"dp8825239105362244","type":"ellipse","data":{"p1":{"x":185.96670401123384,"y":189.40727418009203},"p2":{"x":219.3919800340896,"y":222.83255020294786},"rotation":12.59},"style":{"fillColor":[70,114,191,1]}},{"id":"dp8181833415681834","type":"ellipse","data":{"p1":{"x":265.7964198266168,"y":104.81157571131483},"p2":{"x":299.2216958494729,"y":138.2368517341706},"rotation":11.34},"style":{"fillColor":[255,255,255,1]}},{"id":"dp5215271362607576","type":"ellipse","data":{"p1":{"x":260.5652175137361,"y":185.2413112718566},"p2":{"x":293.9904935365919,"y":218.66658729471243},"rotation":1.24},"style":{"fillColor":"none"}},{"id":"dp7457878487719132","type":"ellipse","data":{"p1":{"x":354.72685914559,"y":180.33705910353098},"p2":{"x":388.1521351684457,"y":213.7623351263867},"rotation":312.14},"style":{"fillColor":[247,31,31,1]}},{"id":"dp9130899695035204","type":"ellipse","data":{"p1":{"x":350.80345741092947,"y":79.96336472513114},"p2":{"x":384.22873343378535,"y":113.38864074798697}},"style":{"fillColor":[247,31,31,1]}},{"id":"dp22495501429737175","type":"ellipse","data":{"p1":{"x":432.349497886343,"y":115.48105741170646},"p2":{"x":465.77477390919876,"y":148.90633343456227}},"style":{"fillColor":[247,31,31,1]}},{"id":"da45163841721681375","data":[{"x":156.33333333333334,"y":188},{"x":179,"y":118.66666666666667}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da950645533080333","data":[{"x":190.96301736263126,"y":123.85104537374855},{"x":201.66666666666666,"y":189.33333333333331}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da36902950645143884","data":[{"x":207.6756553740592,"y":107.13840736232062},{"x":266.1226902403077,"y":118.23799610169955}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da746479996589531","data":[{"x":279.2228402170017,"y":137.91058132047988},{"x":277.639523585014,"y":185.24522504965404}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da4910379186426199","data":[{"x":295.29829411481217,"y":111.25897098062337},{"x":350.80345741092947,"y":96.67600273655906}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da8671316054275053","data":[{"x":367.51609542235735,"y":113.38864074798697},{"x":371.8046279406934,"y":180.89935177084863}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da9028559063613073","data":[{"x":386.75,"y":190.5},{"x":438.3333333333333,"y":144.66666666666669}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da9178761275900345","data":[{"x":296.25,"y":131.16666666666669},{"x":359.04694881946455,"y":185.83644535632817}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"dg04640974050720881","entities":[{"id":"dp776908654711185","type":"doc-arc","data":{"p1":{"x":266.271848370746,"y":104.75136724720379},"p2":{"x":299.6971243936021,"y":138.17664327005957},"rotation":68.87,"angle2":180,"angle1":0},"style":{"fillColor":[70,114,191,1]}},{"id":"da7834277178847115","data":[{"x":276.9598268557248,"y":105.87504291691714},{"x":289.0091459086233,"y":137.05296760034622}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"fillColor":[70,114,191,1]}}]},{"id":"dg21565273094307136","entities":[{"id":"dp6304082120071617","type":"doc-arc","data":{"p1":{"x":265.4385150374126,"y":104.91803391387039},"p2":{"x":298.8637910602687,"y":138.3433099367261},"rotation":248.87,"angle2":180,"angle1":0},"style":{"fillColor":[247,31,31,1]}},{"id":"da06997615459628115","data":[{"x":288.1758125752898,"y":137.21963426701274},{"x":276.12649352239146,"y":106.04170958358368}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"fillColor":[247,31,31,1]}}],"data":{"rotation":180}},{"id":"ds7898546975082403","type":"polygon-curve","data":[{"p1":{"x":262.75,"y":103.91666666666667},"p2":{"x":397.6666666666667,"y":82.66666666666667},"cp":{"dx":31.5,"dy":-25},"cp2":{"dx":3.3333333333333144,"dy":-30}},{"p1":{"x":397.6666666666667,"y":82.66666666666667},"p2":{"x":397.6666666666667,"y":147.33333333333331},"cp":{"dx":-3.3333333333333144,"dy":30},"cp2":{"dx":-9.333333333333371,"dy":-11.333333333333343}},{"p1":{"x":397.6666666666667,"y":147.33333333333331},"p2":{"x":474.33333333333337,"y":112.66666666666667},"cp":{"dx":9.333333333333371,"dy":11.333333333333343},"cp2":{"dx":-21.999999999999943,"dy":-52}},{"p1":{"x":474.33333333333337,"y":112.66666666666667},"p2":{"x":362.25,"y":224.41666666666669},"cp":{"dx":21.999999999999886,"dy":52},"cp2":{"dx":43,"dy":10}},{"p1":{"x":362.25,"y":224.41666666666669},"p2":{"x":262.75,"y":103.91666666666667},"cp":{"dx":-43,"dy":-10},"cp2":{"dx":-31.5,"dy":25}}],"style":{"strokeType":"--","strokeColor":[247,31,31,0.5],"thickness":2}},{"id":"ds16719263025699926","type":"polygon-curve","data":[{"p1":{"x":126.25,"y":217},"p2":{"x":161.66666666666666,"y":100.66666666666667},"cp":{"dx":-3.3333333333333712,"dy":-29.333333333333343},"cp2":{"dx":-18.666666666666686,"dy":50.000000000000014}},{"p1":{"x":161.66666666666666,"y":100.66666666666667},"p2":{"x":306.25,"y":97},"cp":{"dx":18.666666666666686,"dy":-50.000000000000014},"cp2":{"dx":-15.5,"dy":-14}},{"p1":{"x":306.25,"y":97},"p2":{"x":275.25,"y":151.5},"cp":{"dx":15.5,"dy":14},"cp2":{"dx":52,"dy":28}},{"p1":{"x":275.25,"y":151.5},"p2":{"x":233.25,"y":185},"cp":{"dx":-52,"dy":-28},"cp2":{"dx":-29,"dy":-70}},{"p1":{"x":233.25,"y":185},"p2":{"x":126.25,"y":217},"cp":{"dx":29,"dy":70},"cp2":{"dx":3.3333333333333712,"dy":29.333333333333343}}],"style":{"strokeType":"--","strokeColor":[70,114,191,0.5],"thickness":2}},{"id":"da40553886032987996","data":[{"x":219.75,"y":47.5},{"x":202.75,"y":89.5}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"style":{"thickness":1,"strokeColor":[0,0,0,1]},"headScale":0.7},{"id":"da3726540889950014","data":[{"x":421.5,"y":86},{"x":383.5,"y":173}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"style":{"thickness":1,"strokeColor":[0,0,0,1]},"headScale":0.7}],"settings":{"grid":true}}]},{"id":"n0.48440111412063036","blocks":[],"style":null}],"pageSettings":{"pageSize":{"width":677,"sizeUnit":"px"}},"___version":2,"version":2,"av":163,"delayRenderCache":{"av":163,"map":{}}}

==> figs/docs/87ba44e8-3c05-4fd7-8b4b-d046ea991c28 <==
{"id":"r0.28521863390524915","lines":[{"id":"n0.06518260433361944","blocks":[]},{"id":"n0.6194212053376131","blocks":[{"id":"n0.07332230663346939","text":"\\diagram","type":"composite","elements":{"de27015728856363497":{"id":"de27015728856363497","lines":[{"id":"n0.5789419106206919","blocks":[{"id":"n0.14053065499663497","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.7783555987421398","lines":[{"id":"n0.8124787856003206","blocks":[{"id":"n0.8029616716976593","text":"1"}]}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"}}]}],"shape":{"data":{"p":{"x":270.250710900474,"y":25.325434439178522}},"anchor":"center","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true},"de15039028513302677":{"id":"de15039028513302677","lines":[{"id":"n0.5107313851872686","blocks":[{"id":"n0.42843794643142674","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.9060529032807887","lines":[{"id":"n0.19573768613661602","blocks":[{"id":"n0.7675130730368354","text":"K"},{"id":"n0.0832967800500739","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.05545852423710129","lines":[{"id":"n0.7429118926211464","blocks":[{"id":"n0.4385704272700135","text":"n"}]}]}}}]}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"}}]}],"shape":{"data":{"p":{"x":343.4505166666666,"y":131.16666666666666}},"anchor":"top","settings":{"fontSize":"\\footnotesize"},"style":{"textColor":[0,0,0,1]}},"isTextMode":true},"de2056536707556802":{"id":"de2056536707556802","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.5939194986973031","text":"R"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"n","id":"n0.3939647741472545"}],"id":"n0.04922346118876497"}],"id":"n0.8476042378455018"}},"id":"n0.5160389805441985"}],"id":"n0.848091092695114"}],"id":"n0.03968552834638284"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.028048137251828864"}],"id":"n0.20536520778145428"}],"shape":{"data":{"p":{"x":338.1171833333333,"y":219.16666666666663}},"anchor":"top","settings":{"fontSize":"\\footnotesize"},"style":{"textColor":[0,0,0,1]}},"isTextMode":true},"de0067964242732707625":{"id":"de0067964242732707625","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.753640532500151","text":"t"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"n","id":"n0.8381313780692095"}],"id":"n0.6076886538188415"}],"id":"n0.37209380528486524"}},"id":"n0.48919320239616626"}],"id":"n0.3209465815232093"}],"id":"n0.4180808384353798"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.9001540985749843"}],"id":"n0.43043063733752573"}],"shape":{"data":{"p":{"x":84.84373333333335,"y":223.5}},"anchor":"top","settings":{"fontSize":"\\footnotesize"}},"isTextMode":true},"de8507121270116855":{"id":"de8507121270116855","lines":[{"id":"n0.08652612109775304","blocks":[{"id":"n0.3749822100905851","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.6752865795068277","lines":[{"id":"n0.6856995060429103","blocks":[{"id":"n0.6509987067803147","text":"\\bigr","type":"composite","elements":{},"bracketName":"brace","size":"Big","isClose":true},{"id":"n0.11857832842928673","text":"n"}]}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"}},{"id":"n0.32522147741758056","text":" nodes"}]}],"shape":{"data":{"p":{"x":486.33333333333337,"y":183.33333333333334}},"anchor":"left-top"},"isTextMode":true},"de27788409947776493":{"id":"de27788409947776493","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"\\bigr","type":"composite","elements":{},"bracketName":"brace","size":"Big","isClose":true,"id":"n0.7344591634201596"},{"id":"n0.21680986402429903","text":"m"},{"id":"n0.07616773770299168","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.14586786714133626","lines":[{"id":"n0.5351187879381474","blocks":[{"id":"n0.10818886797984995","text":"n"}]}]}}}],"id":"n0.7557516266998732"}],"id":"n0.8610858042888305"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.7161347467271861"},{"text":" nodes","id":"n0.8145059028898136"}],"id":"n0.3126632235315552"}],"shape":{"data":{"p":{"x":486.33333333333337,"y":88}},"anchor":"left-top"},"isTextMode":true}},"connections":[],"intersections":{"id":"di30119318020760555","items":[],"style":{}},"shapes":[{"id":"dp6775323334711851","type":"doc-rounded-rect","data":{"p1":{"x":20.5,"y":188.64581358609792},"p2":{"x":486.2819905213271,"y":219.10078988941547},"cornerRadiusPercentage":1,"flipX":true},"style":{"fillColor":[74,144,226,0.3],"strokeColor":"none","strokeType":"."}},{"id":"dp6273853992007636","type":"doc-rounded-rect","data":{"p1":{"x":66.87914691943132,"y":91.11216429699843},"p2":{"x":442.6895734597157,"y":129.33017377567143},"flipX":true,"cornerRadiusPercentage":1},"style":{"fillColor":[74,144,226,0.3],"strokeType":".","strokeColor":"none"}},{"id":"dp05832111500862136","type":"circle","data":{"p1":{"x":261.59194312796217,"y":16.66666666666667},"p2":{"x":278.90947867298587,"y":33.98420221169037},"flipX":true},"style":{"thickness":2}},{"id":"dp8579067391001112","type":"ellipse","data":{"p1":{"x":414.1454976303319,"y":102.97567140600319},"p2":{"x":431.46303317535546,"y":120.29320695102686},"flipX":true},"style":{"thickness":2}},{"id":"dp7210264341356638","type":"circle","data":{"p1":{"x":458.5739336492891,"y":195.73396524486583},"p2":{"x":475.8914691943128,"y":213.05150078988953},"flipX":true},"style":{"thickness":2}},{"id":"dp6725517433680526","type":"circle","data":{"p1":{"x":428.2383886255925,"y":195.73396524486583},"p2":{"x":445.5559241706162,"y":213.05150078988953},"flipX":true},"style":{"thickness":2}},{"id":"dp6374152753703906","type":"circle","data":{"p1":{"x":363.8529857819906,"y":195.73396524486583},"p2":{"x":381.1705213270143,"y":213.05150078988953},"flipX":true},"style":{"thickness":2}},{"id":"da7671201549013111","data":[{"x":411,"y":204.39273301737768},{"x":394.2004739336494,"y":204.39273301737768}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"da441223531627952","data":[{"x":327.6666666666667,"y":111.63443917851504},{"x":311.6666666666667,"y":111.63443917851504}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"da1106915686367067","data":[{"x":428.3578199052133,"y":118.58135860979462},{"x":465,"y":195.60000000000002}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"da2646109971355177","data":[{"x":424.7748815165878,"y":120.67140600315957},{"x":436.89715639810436,"y":195.73396524486583}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"da09711609278280009","data":[{"x":415.9369668246446,"y":117.62590837282781},{"x":375.79999999999995,"y":195.2}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"da9055635253679755","data":[{"x":419.69905213270147,"y":120.5221169036335},{"x":407.4,"y":196.39999999999998}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"dp15935464131712362","type":"ellipse","data":{"p1":{"x":235.79478672985783,"y":99.79083728278043},"p2":{"x":253.11232227488154,"y":117.10837282780415},"flipX":true},"style":{"thickness":2}},{"id":"dp7422525143293746","type":"circle","data":{"p1":{"x":280.22322274881526,"y":195.73396524486583},"p2":{"x":297.54075829383896,"y":213.05150078988953},"flipX":true},"style":{"thickness":2}},{"id":"dp5215752214617919","type":"circle","data":{"p1":{"x":249.88767772511858,"y":195.73396524486583},"p2":{"x":267.2052132701423,"y":213.05150078988953},"flipX":true},"style":{"thickness":2}},{"id":"dp7445383691733272","type":"ellipse","data":{"p1":{"x":185.50227488151654,"y":195.73396524486583},"p2":{"x":202.8198104265404,"y":213.05150078988953},"flipX":true},"style":{"thickness":2}},{"id":"da7401796013065329","data":[{"x":236.8696682464456,"y":204.39273301737768},{"x":220.33333333333331,"y":204.39273301737768}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"da9207597860669241","data":[{"x":250.0071090047394,"y":115.3965244865719},{"x":285.8,"y":195.60000000000002}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"da7066359381073841","data":[{"x":246.42417061611377,"y":117.48657187993683},{"x":256.6,"y":195.2}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"da9696290080488186","data":[{"x":237.58625592417064,"y":114.44107424960504},{"x":197,"y":195.39999999999998}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"da7030082937125366","data":[{"x":241.34834123222765,"y":117.33728278041076},{"x":228.50947867298584,"y":195.0173775671406}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"dp5603243908746471","type":"circle","data":{"p1":{"x":81.3303317535545,"y":100.58704581358612},"p2":{"x":98.6478672985782,"y":117.90458135860982},"flipX":true},"style":{"thickness":2}},{"id":"dp032378341087528906","type":"circle","data":{"p1":{"x":125.75876777251193,"y":195.73396524486583},"p2":{"x":143.07630331753563,"y":213.05150078988953},"flipX":true},"style":{"thickness":2}},{"id":"dp056330744794505616","type":"circle","data":{"p1":{"x":65.38625592417065,"y":195.73396524486583},"p2":{"x":82.70379146919436,"y":213.05150078988953},"flipX":true},"style":{"thickness":2}},{"id":"dp01320910698982214","type":"circle","data":{"p1":{"x":31.037819905213325,"y":195.73396524486583},"p2":{"x":48.35535545023703,"y":213.05150078988953},"flipX":true},"style":{"thickness":2}},{"id":"da32847301341249957","data":[{"x":113.05924170616123,"y":204.39273301737768},{"x":95.66666666666666,"y":204.39273301737768}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"da3127696548597576","data":[{"x":95.54265402843606,"y":116.19273301737758},{"x":134.41753554502378,"y":194.93775671406013}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"da8859796406630904","data":[{"x":91.9597156398105,"y":118.2827804107425},{"x":104.0819905213271,"y":194.93775671406013}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"da6297628972213167","data":[{"x":83.12180094786737,"y":115.23728278041074},{"x":39.69658767772518,"y":194.93775671406013}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"da8019018837930725","data":[{"x":86.88388625592421,"y":118.13349131121646},{"x":74.0450236966825,"y":195.8135860979463}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6},{"id":"da8265471433565201","data":[{"p1":{"x":278.90947867298587,"y":25.325434439178522},"p2":{"x":467.2327014218009,"y":195.73396524486583},"cp":{"dx":148.6521327014218,"dy":-1.492890995260666},"cp2":{"dx":30.56729857819903,"dy":-63.73396524486583}}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"type":"cubic","headScale":0.6},{"id":"da3012795567225317","data":[{"p1":{"x":278.90947867298587,"y":25.325434439178522},"p2":{"x":442.6,"y":197.2},"cp":{"dx":147.85592417061605,"dy":12.838862559241704},"cp2":{"dx":42.19905213270147,"dy":-58.12322274881515}}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"type":"cubic","headScale":0.6},{"id":"da8187967735753341","data":[{"p1":{"x":277.87440758293843,"y":30.20221169036335},"p2":{"x":369.79999999999995,"y":195.2},"cp":{"dx":107.48815165876778,"dy":61.30805687203793},"cp2":{"dx":7.2000000000000455,"dy":-51.19999999999999}}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"type":"cubic","headScale":0.6},{"id":"da5688795005286167","data":[{"p1":{"x":261.59194312796217,"y":25.325434439178522},"p2":{"x":35.5,"y":196},"cp":{"dx":-201.87867298578203,"dy":-3.0853080568720515},"cp2":{"dx":-7.962085308056828,"dy":-63.69668246445502}}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"type":"cubic","headScale":0.6},{"id":"da6836923570044471","data":[{"p1":{"x":261.59194312796217,"y":25.325434439178522},"p2":{"x":69.5,"y":197},"cp":{"dx":-187.54691943127966,"dy":13.635071090047383},"cp2":{"dx":-31.848341232227455,"dy":-66.88151658767777}}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"type":"cubic","headScale":0.6},{"id":"da5743850482413462","data":[{"p1":{"x":261.9502369668247,"y":30.20221169036335},"p2":{"x":138.53791469194312,"y":195.8135860979463},"cp":{"dx":-110.55023696682471,"dy":47.397788309636645},"cp2":{"dx":-5.537914691943115,"dy":-65.41358609794631}}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"type":"cubic","headScale":0.6},{"id":"dg302120896633882","entities":[{"id":"dp5892295935836898","type":"doc-right-angle","data":{"p1":{"x":80.11611374407573,"y":172.0268562401263},"p2":{"x":90.46682464454977,"y":270.955766192733},"rotation":270,"flipX":true}},{"id":"da6584187404998083","data":[{"x":134.75592417061608,"y":216.3669444898403},{"x":134.75592417061608,"y":226.66666666666669}],"head":"no","tail":"no","shaft":"-","mVer":1}],"data":{"rotation":90}},{"id":"da0591061009352043","data":[{"p1":{"x":261.9502369668247,"y":30.20221169036335},"p2":{"x":187.4251184834124,"y":194.77851500789893},"cp":{"dx":-63.350236966824724,"dy":81.79778830963664},"cp2":{"dx":3.974881516587601,"dy":-63.57851500789894}}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"type":"cubic","headScale":0.6},{"id":"da2107190541064632","data":[{"p1":{"x":270.25071090047396,"y":33.98420221169037},"p2":{"x":264.2592417061612,"y":196.45055292259082},"cp":{"dx":6.907109004739311,"dy":43.03507109004737},"cp2":{"dx":22.45308056872028,"dy":-50.63886255924166}}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"type":"cubic","headScale":0.6},{"id":"da14159707321992498","data":[{"p1":{"x":272.85829383886266,"y":34.50173775671405},"p2":{"x":292.2,"y":196},"cp":{"dx":23.88625592417054,"dy":44.42843601895737},"cp2":{"dx":12.898578199052167,"dy":-54.93838862559241}}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"type":"cubic","headScale":0.6}],"settings":{"grid":true,"diagramHeight":336}}]},{"id":"n0.4927878538015349","blocks":[],"style":null}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":957,"delayRenderCache":{"av":957,"map":{}}}

==> figs/docs/a25fc49a-1e59-41ac-a56d-e448b64018db <==
{"id":"r0.9985913243451319","lines":[{"blocks":[{"text":"\\diagram","type":"composite","elements":{"de9044116868092833":{"id":"de9044116868092833","lines":[{"blocks":[{"text":"5","id":"n0.03365061643301637"}],"id":"n0.10460424301501758"}],"shape":{"data":{"p":{"x":128.8643076797487,"y":153.30550394860256},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de3497163068976279":{"id":"de3497163068976279","lines":[{"blocks":[{"text":"2","id":"n0.5201733817522745"}],"id":"n0.8761146662946115"}],"shape":{"data":{"p":{"x":65.72367457392377,"y":60.256149897913346},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de8863745168376593":{"id":"de8863745168376593","lines":[{"blocks":[{"text":"4","id":"n0.8375628828247146"}],"id":"n0.4945718388768239"}],"shape":{"data":{"p":{"x":66.83140497928915,"y":256.32443164757996},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de07588287070962263":{"id":"de07588287070962263","lines":[{"blocks":[{"text":"1","id":"n0.19239814286915635"}],"id":"n0.1426290773637402"}],"shape":{"data":{"p":{"x":240.7450786216489,"y":54.71749787108662},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de5393471101244944":{"id":"de5393471101244944","lines":[{"blocks":[{"text":"6","id":"n0.36994293865934647"}],"id":"n0.5763095513666101"}],"shape":{"data":{"p":{"x":347.0871975367224,"y":145.55139111104518},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de9889106025636631":{"id":"de9889106025636631","lines":[{"blocks":[{"text":"3","id":"n0.11259243727394863"}],"id":"n0.9477826943520649"}],"shape":{"data":{"p":{"x":251.82238267530238,"y":245.24712759392654},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de887609073895836":{"id":"de887609073895836","lines":[{"blocks":[{"text":"7","id":"n0.9574843772843196"}],"id":"n0.8677888929873532"}],"shape":{"data":{"p":{"x":357.0567711850105,"y":296.2027262407325},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de4886888726793903":{"id":"de4886888726793903","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"*","id":"n0.23596085205849704"}],"id":"n0.29067595683099423"}],"id":"n0.062380728294148424"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.6913549850816203"}],"id":"n0.23227304427369488"}],"shape":{"data":{"p":{"x":240,"y":17.00000000000003}},"anchor":"left-top"},"isTextMode":true},"de9511667999305062":{"id":"de9511667999305062","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"e","id":"n0.6093485921089938"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"1","id":"n0.253855442378059"}],"id":"n0.544688337006112"}],"id":"n0.41386266168883035"}},"id":"n0.7861488141604047"}],"id":"n0.6529169034237015"}],"id":"n0.3954789691391096"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.0946549000814183"}],"id":"n0.10238032377850392"}],"shape":{"data":{"p":{"x":62,"y":19}},"anchor":"left-top","style":{"textColor":[247,31,31,1]}},"isTextMode":true},"de9039305937524613":{"id":"de9039305937524613","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"*","id":"n0.5678663939786854"}],"id":"n0.7936300338501139"}],"id":"n0.40231445270705146"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.6718969353612751"}],"id":"n0.9575900136762763"}],"shape":{"data":{"p":{"x":254.33333333333334,"y":284.66666666666663}},"anchor":"left-top"},"isTextMode":true},"de7015381639364437":{"id":"de7015381639364437","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"e","id":"n0.6827189651059127"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"0","id":"n0.0535029566810612"}],"id":"n0.11529277501801483"}],"id":"n0.6713159981348888"}},"id":"n0.3195757068792915"}],"id":"n0.942621714564287"}],"id":"n0.22835166517518224"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.48330780142080587"}],"id":"n0.26895952461545836"}],"shape":{"data":{"p":{"x":385.33333333333337,"y":143}},"anchor":"left-top","style":{"textColor":[70,114,191,1]}},"isTextMode":true},"de24760227446137928":{"id":"de24760227446137928","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"e","id":"n0.6494284147712419"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"1","id":"n0.18350017890275372"}],"id":"n0.32890632658443963"}],"id":"n0.5906855976172447"}},"id":"n0.5123719807544154"}],"id":"n0.14745664635408118"}],"id":"n0.025856211802699924"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.25362377045591744"}],"id":"n0.6818338525471679"}],"shape":{"data":{"p":{"x":61.333333333333314,"y":293.99999999999994}},"anchor":"left-top","style":{"textColor":[247,31,31,1]}},"isTextMode":true},"de830508034863153":{"id":"de830508034863153","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"*","id":"n0.3872084083299474"}],"id":"n0.19435667825294423"}],"id":"n0.5164470480899168"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.17661662062597627"}],"id":"n0.2830771065574269"}],"shape":{"data":{"p":{"x":94.33333333333337,"y":149.66666666666663}},"anchor":"left-top"},"isTextMode":true},"de3975804514362884":{"id":"de3975804514362884","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"*","id":"n0.5678062383568634"}],"id":"n0.2603030929155328"}],"id":"n0.6438081819368608"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.27924461712113335"}],"id":"n0.7363396134110105"}],"shape":{"data":{"p":{"x":395.33333333333337,"y":296.66666666666663}},"anchor":"left-top"},"isTextMode":true}},"connections":[],"intersections":{"id":"di018738070182718003","items":[],"style":{}},"shapes":[{"id":"dp6035839523535407","type":"ellipse","data":{"p1":{"x":44.95402865523873,"y":42.85625299199422},"p2":{"x":100.49332049260892,"y":98.39554482936434}},"style":{"fillColor":"none"}},{"id":"dp32750554968646073","type":"ellipse","data":{"p1":{"x":45.52895517377332,"y":238.64630089431083},"p2":{"x":101.06824701114326,"y":294.1855927316803},"rotation":12.59},"style":{"fillColor":"none"}},{"id":"dp4524396334316858","type":"ellipse","data":{"p1":{"x":108.38664482631847,"y":135.74529364125738},"p2":{"x":163.92593666368901,"y":191.28458547862738},"rotation":11.34},"style":{"fillColor":[255,255,255,1]}},{"id":"dp6018995913081344","type":"ellipse","data":{"p1":{"x":336.79390961187244,"y":278.949097787917},"p2":{"x":392.33320144924306,"y":334.4883896252872},"rotation":1.24},"style":{"fillColor":"none"}},{"id":"dp6224840239709277","type":"ellipse","data":{"p1":{"x":231.22913809978522,"y":228.00619298050708},"p2":{"x":286.7684299371551,"y":283.5454848178769},"rotation":312.14},"style":{"fillColor":"none"}},{"id":"dp9746429905339573","type":"ellipse","data":{"p1":{"x":219.72524418472122,"y":37.96336472513116},"p2":{"x":275.26453602209136,"y":93.50265656250127}},"style":{"fillColor":"none"}},{"id":"dp8403031461767165","type":"ellipse","data":{"p1":{"x":325.31306594751015,"y":128.5497234540565},"p2":{"x":380.85235778488016,"y":184.0890152914266}},"style":{"fillColor":"none"}},{"id":"da7003551264465873","data":[{"x":66.0772921417317,"y":239.0773063107636},{"x":66.0772921417317,"y":97.28781442399901}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"da9857106916676444","data":[{"x":120.3560820046338,"y":185.9062468532269},{"x":91.55509146513478,"y":245.7236887429557}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"da5694975698556846","data":[{"x":87.12416984367336,"y":95.07235361326829},{"x":119.24835159926843,"y":142.7047610439783}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"da47080577402734236","data":[{"x":359.62584956354925,"y":183.69078604249617},{"x":365.16450159037583,"y":278.9556009039161}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"da04674290247759605","data":[{"x":149.15707254413283,"y":139.38156982788226},{"x":220.05181848751522,"y":72.91774550596136}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"da8616976365044808","data":[{"x":275.4383387557826,"y":71.81001510059599},{"x":346.33308469916494,"y":129.4119961795941}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"da6227058507623549","data":[{"x":284.854047201388,"y":244.06209313490763},{"x":341.3482978750208,"y":180.92146002908285}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"da47374811522284954","data":[{"x":158.57278098973836,"y":180.92146002908285},{"x":233.34458335189936,"y":244.06209313490763}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2}},{"id":"da5119249099586307","data":[{"x":99,"y":61},{"x":219.72524418472125,"y":65.73301064381621}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2,"strokeColor":[0,0,0,1]}},{"id":"da9394116449243033","data":[{"x":100.49332049260892,"y":70.62589891067928},{"x":247,"y":230}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2,"strokeColor":[0,0,0,1]}},{"id":"da3223292985728612","data":[{"x":102,"y":267},{"x":233,"y":265}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2,"strokeColor":[0,0,0,1]}},{"id":"da33250200371535366","data":[{"x":100,"y":260},{"x":240,"y":92}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2,"strokeColor":[0,0,0,1]}},{"id":"da7689897731296891","data":[{"x":161,"y":152},{"x":325.31306594751015,"y":156.31936937274156}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2,"strokeColor":[0,0,0,1]}},{"id":"da296134335013271","data":[{"x":253,"y":93},{"x":259,"y":228}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2,"strokeColor":[0,0,0,1]}},{"id":"da2844528890024529","data":[{"x":263,"y":87},{"x":348,"y":285}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2,"strokeColor":[0,0,0,1]}},{"id":"da8799013953533033","data":[{"x":284,"y":267},{"x":336.80041272787156,"y":306.1177976467841}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":2,"strokeColor":[0,0,0,1]}}],"settings":{"grid":true,"diagramHeight":358.6640625},"id":"n0.8096274616313681"}],"id":"n0.6049316660578776"}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":2,"delayRenderCache":{"av":2,"map":{}}}

==> figs/docs/a8943bc4-3273-4bf3-b662-74fa4fa220bc <==
{"id":"r0.4375928235107577","lines":[{"blocks":[{"text":"\\diagram","type":"composite","elements":{"de7765045494426801":{"id":"de7765045494426801","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"G","id":"n0.11766022769822526"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i-1","id":"n0.14264849205016117"}],"id":"n0.6742645133176386"}],"id":"n0.8986815463326481"}},"id":"n0.22722980483879174"}],"id":"n0.4386747276761169"}],"id":"n0.537369819340622"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.7467931839351494"}],"id":"n0.39012984437306963"}],"shape":{"data":{"p":{"x":45.77467834199227,"y":148.8048872180451},"rotation":0},"anchor":"center"},"isTextMode":true,"isInGroup":true},"de2746680852491752":{"id":"de2746680852491752","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"G","id":"n0.03337358914233457"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.7567024163245031","text":"i"}],"id":"n0.7177625658529534"}],"id":"n0.2959186169782604"}},"id":"n0.7111242959624999"}],"id":"n0.5146826790977959"}],"id":"n0.5940414284650617"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.5012858638173145"}],"id":"n0.46673469954973745"}],"shape":{"data":{"p":{"x":353.0413450086589,"y":148.8048872180451},"rotation":0},"anchor":"center"},"isTextMode":true,"isInGroup":true},"de693674574125986":{"id":"de693674574125986","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"G","id":"n0.628176764881075"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.2980035095923037"}],"id":"n0.9026833292180252"}],"id":"n0.8960690862643972"}},"id":"n0.8723301416718818"},{"id":"n0.9813310273349436","text":"'"}],"id":"n0.8122166024630024"}],"id":"n0.7388988349486807"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.357681293659291"}],"id":"n0.7149724482603586"}],"shape":{"data":{"p":{"x":45.774678341992264,"y":309.1485373590226},"rotation":0},"anchor":"center"},"isTextMode":true,"isInGroup":true},"de29918931349792754":{"id":"de29918931349792754","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"G","id":"n0.10183263126000441"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.3627316150331308"}],"id":"n0.09193054714972715"}],"id":"n0.04662775032679911"}},"id":"n0.6096319621112813"},{"text":"''","id":"n0.2505439250426613"}],"id":"n0.7902284965374995"}],"id":"n0.25347695245789614"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.16061921589725414"}],"id":"n0.5871362684760146"}],"shape":{"data":{"p":{"x":353.0413450086589,"y":309.1485373590226},"rotation":0},"anchor":"center"},"isTextMode":true,"isInGroup":true},"de8219032819322303":{"id":"de8219032819322303","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"k","id":"n0.3610102205448573"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.8038521397474703"}],"id":"n0.6516148941104005"}],"id":"n0.7650550197648431"}},"id":"n0.08475035895381189"}],"id":"n0.527800417863205"}],"id":"n0.6950296327756982"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.14917732065257394"}],"id":"n0.10579604505655449"}],"shape":{"data":{"p":{"x":164.74476957457608,"y":72.66455649065688},"rotation":0},"anchor":"center","settings":{"fontSize":"\\normalsize"}},"isTextMode":true,"isInGroup":false},"de04283524877908573":{"id":"de04283524877908573","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"N","id":"n0.8801300433579429"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.291379626699916"}],"id":"n0.13547962306674144"}],"id":"n0.15798535956240722"},"powerValue":{"id":"n0.4824145095044019","lines":[{"id":"n0.8077133127515737","blocks":[{"id":"n0.17169925138260034","text":"G"},{"id":"n0.35445006946713575","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.8934963371915996","lines":[{"id":"n0.9498324753539562","blocks":[{"id":"n0.36625465023745796","text":"i-1"}]}]}}}]}]}},"id":"n0.5274944417406209"},{"type":"single","text":"(","id":"n0.6472531277313562"},{"text":"k","id":"n0.9675588407744684"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.8824400805040313"}],"id":"n0.9602650684640242"}],"id":"n0.5215707503700362"}},"id":"n0.10213664553526414"},{"type":"single","text":")","id":"n0.6962438075155524"},{"text":"∩A","id":"n0.7418351275556754"},{"id":"n0.10579038250939443","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.676014547321123","lines":[{"id":"n0.359786619434068","blocks":[{"id":"n0.36446715593683066","text":"i"}]}]}}}],"id":"n0.5318731672690591"}],"id":"n0.14531112898633802"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.41102203919422364"}],"id":"n0.8728565664350789"}],"shape":{"data":{"p":{"x":251.63053545838423,"y":147.22029605582574},"rotation":0},"anchor":"top","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":false},"de17654966827324947":{"id":"de17654966827324947","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"N","id":"n0.7074566541931357"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.8690852412096277"}],"id":"n0.3959920873465246"}],"id":"n0.773990093278438"},"powerValue":{"id":"n0.08833300021885382","lines":[{"id":"n0.022858244320182353","blocks":[{"id":"n0.6283571647115973","text":"G"},{"id":"n0.24146177184364181","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.2192055513141129","lines":[{"id":"n0.1843382320319198","blocks":[{"id":"n0.8614330403210204","text":"i-1"}]}]}}}]}]}},"id":"n0.7626988817359919"},{"type":"single","text":"(","id":"n0.0355233546650815"},{"text":"k","id":"n0.9724778172896884"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.7221316227919881"}],"id":"n0.8294038375212891"}],"id":"n0.7172016925558227"}},"id":"n0.8988468758596786"},{"type":"single","text":")","id":"n0.2701375911877455"},{"text":"∩B","id":"n0.9421509886414561"},{"id":"n0.5075928957969955","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.9174963915565781","lines":[{"id":"n0.2684107048666349","blocks":[{"id":"n0.8331782614818077","text":"i"}]}]}}}],"id":"n0.1507134520313398"}],"id":"n0.13313886657236074"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.4511352144142009"}],"id":"n0.4654100119620319"}],"shape":{"data":{"p":{"x":255.1766589008688,"y":33.925953861207375},"rotation":0},"anchor":"bottom","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":false},"de4242152326557307":{"id":"de4242152326557307","lines":[{"id":"n0.12826432060281845","blocks":[{"id":"n0.5391823853110798","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.004285027630421379","lines":[{"id":"n0.32626627040988665","blocks":[{"id":"n0.7877988096803397","text":"N"},{"id":"n0.17260669483489965","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.24483296398164978","lines":[{"id":"n0.43610590563554275","blocks":[{"id":"n0.7862279545359894","text":"b"}]}]}}},{"id":"n0.757584323430389","type":"single","text":"("},{"id":"n0.5244811315960887","text":"k"},{"id":"n0.8067083566847186","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.5340846144526621","lines":[{"id":"n0.4925768636823298","blocks":[{"id":"n0.37732534898515024","text":"i"}]}]}}},{"id":"n0.9700720201362443","type":"single","text":")"}]}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"}}]}],"shape":{"data":{"p":{"x":53.103904509379056,"y":66.95514779785285}},"anchor":"center","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":false},"de13448811536801464":{"id":"de13448811536801464","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"k","id":"n0.658228377023353"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i,B","id":"n0.11376595364462183"}],"id":"n0.2136373231628088"}],"id":"n0.2910128095262037"}},"id":"n0.728438537809698"}],"id":"n0.2606889383312059"}],"id":"n0.5807980803822568"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.16815638408215716"}],"id":"n0.2522718902761838"}],"shape":{"data":{"p":{"x":480.77745959189406,"y":73.16455649065688},"rotation":0},"anchor":"center","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":false},"de003322659665177863":{"id":"de003322659665177863","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"N","id":"n0.5983859513352379"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"b","id":"n0.7894265861401861"}],"id":"n0.6078925435497855"}],"id":"n0.7245294940438491"}},"id":"n0.6425384169941681"},{"type":"single","text":"(","id":"n0.757612107613489"},{"text":"k","id":"n0.30815472240772523"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.31028502320052676"}],"id":"n0.43125171607776114"}],"id":"n0.8550792913560805"}},"id":"n0.57455147617371"},{"type":"single","text":")","id":"n0.0007334788216086796"}],"id":"n0.16971525193346348"}],"id":"n0.8805017220638471"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.17543267037348254"}],"id":"n0.7571415958623684"}],"shape":{"data":{"p":{"x":369.136594526697,"y":67.45514779785285}},"anchor":"center","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":false},"de30888920507420425":{"id":"de30888920507420425","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"k","id":"n0.9153328199507491"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i,A","id":"n0.35469042476705837"}],"id":"n0.5972113557201999"}],"id":"n0.2730038798433585"}},"id":"n0.615489506221329"}],"id":"n0.8941870421016553"}],"id":"n0.4552747076178878"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.929094730754499"}],"id":"n0.940881420640058"}],"shape":{"data":{"p":{"x":471.2774595918941,"y":121.66455649065688},"rotation":0},"anchor":"center","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":false},"de34186704701286486":{"id":"de34186704701286486","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"N","id":"n0.9587647500376018"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.5500960157843409"}],"id":"n0.5503875921545063"}],"id":"n0.6762784856456932"},"powerValue":{"lines":[{"blocks":[{"text":"G","id":"n0.7215779218337377"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i-1","id":"n0.2920602909022314"}],"id":"n0.29760355225443647"}],"id":"n0.6541108645470048"}},"id":"n0.8443661666878315"}],"id":"n0.4077715915386566"}],"id":"n0.638711738752707"}},"id":"n0.7640411088031489"},{"type":"single","text":"(","id":"n0.9107003061982724"},{"text":"k","id":"n0.5566147141031275"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.1597629963729883"}],"id":"n0.29792103503210887"}],"id":"n0.8358982435309548"}},"id":"n0.43754328385522934"},{"type":"single","text":")","id":"n0.18545422750510365"},{"text":"∩A","id":"n0.6148854205716086"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.8022464908893501"}],"id":"n0.32420018799108963"}],"id":"n0.9516089465508146"}},"id":"n0.14794249451206642"}],"id":"n0.17288135617243494"}],"id":"n0.8537641712458439"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.8675630282548157"}],"id":"n0.8324398778241886"}],"shape":{"data":{"p":{"x":568.297202125051,"y":146.2202960558257},"rotation":0},"anchor":"top","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":false},"de3793001073762772":{"id":"de3793001073762772","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"N","id":"n0.7029454692284811"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.49706719095968155"}],"id":"n0.88201507385877"}],"id":"n0.01424522013682994"},"powerValue":{"lines":[{"blocks":[{"text":"G","id":"n0.5942723221809305"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i-1","id":"n0.15923055550852094"}],"id":"n0.781179315854065"}],"id":"n0.8185862594812265"}},"id":"n0.42256070929614853"}],"id":"n0.9952313950230784"}],"id":"n0.4290710169389671"}},"id":"n0.3139978363828291"},{"type":"single","text":"(","id":"n0.07897078601136998"},{"text":"k","id":"n0.020929486051988633"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.09325176183010209"}],"id":"n0.3175744019762483"}],"id":"n0.9815033366034562"}},"id":"n0.8631257776160641"},{"type":"single","text":")","id":"n0.7350088830708841"},{"text":"∩B","id":"n0.863113610149344"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.9788227456651177"}],"id":"n0.43694143651471373"}],"id":"n0.12777599225753744"}},"id":"n0.28294934737624344"}],"id":"n0.41480893703297994"}],"id":"n0.8744403126887612"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.1801688205239942"}],"id":"n0.8627224178631074"}],"shape":{"data":{"p":{"x":571.8433255675354,"y":33.92595386120736},"rotation":0},"anchor":"bottom","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":false},"de9797546646233857":{"id":"de9797546646233857","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"k","id":"n0.9579878115814102"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i,B","id":"n0.8526376187708817"}],"id":"n0.3008171417023662"}],"id":"n0.5015595066985326"}},"id":"n0.9984123161108147"}],"id":"n0.43343822861158365"}],"id":"n0.7359059066623186"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.19751630723770708"}],"id":"n0.2275614387854823"}],"shape":{"data":{"p":{"x":164.74476957457608,"y":234.11852343927842},"rotation":0},"anchor":"center","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":false},"de1339697301946321":{"id":"de1339697301946321","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"N","id":"n0.34843446590275695"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"b","id":"n0.3387191378440102"}],"id":"n0.769197621460697"}],"id":"n0.08864897719027853"}},"id":"n0.9912990004962241"},{"type":"single","text":"(","id":"n0.05530317633893955"},{"text":"k","id":"n0.15169892703187648"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.24706923095088018"}],"id":"n0.38258269824787683"}],"id":"n0.11399546446407305"}},"id":"n0.5563728392944807"},{"type":"single","text":")","id":"n0.181959691543764"}],"id":"n0.9556833898484498"}],"id":"n0.7457604877873101"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.08468429738509409"}],"id":"n0.49596140798701405"}],"shape":{"data":{"p":{"x":53.10390450937902,"y":228.4091147464744}},"anchor":"center","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":false},"de9210151181692874":{"id":"de9210151181692874","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"k","id":"n0.2769549568142293"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i,A","id":"n0.11270445189537015"}],"id":"n0.7523837847136936"}],"id":"n0.08800408744907995"}},"id":"n0.5242770716263807"}],"id":"n0.614033623541548"}],"id":"n0.41582744636602564"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.8755197633882956"}],"id":"n0.20139941287759666"}],"shape":{"data":{"p":{"x":155.2447695745761,"y":282.6185234392784},"rotation":0},"anchor":"center","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":false},"de528501042986044":{"id":"de528501042986044","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"N","id":"n0.7739397759753415"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.9797293912676075"}],"id":"n0.2798499923420308"}],"id":"n0.978188653396328"},"powerValue":{"lines":[{"blocks":[{"text":"G","id":"n0.24162475863505595"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i-1","id":"n0.7099957506464059"}],"id":"n0.5085084961239243"}],"id":"n0.8668254511568061"}},"id":"n0.2457530344154344"}],"id":"n0.4273082531702115"}],"id":"n0.47935472973527515"}},"id":"n0.5120886394821964"},{"type":"single","text":"(","id":"n0.5202299058823616"},{"text":"k","id":"n0.12422395961916677"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.16680951901100105"}],"id":"n0.9038499255555612"}],"id":"n0.34447808096845556"}},"id":"n0.5466629346242007"},{"type":"single","text":")","id":"n0.369542454669739"},{"text":"∩A","id":"n0.19908057508079113"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.5904933402340449"}],"id":"n0.24201273310206672"}],"id":"n0.619715595843237"}},"id":"n0.8815518085647474"}],"id":"n0.6463712855241048"}],"id":"n0.6010181374912196"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.29859428891443773"}],"id":"n0.6579794277745616"}],"shape":{"data":{"p":{"x":251.63053545838426,"y":311.8869627224924},"rotation":0},"anchor":"top","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":false},"de3400684421249236":{"id":"de3400684421249236","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"N","id":"n0.5272920805110144"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.18548385844897353"}],"id":"n0.7706241577792372"}],"id":"n0.6370535612362647"},"powerValue":{"lines":[{"blocks":[{"text":"G","id":"n0.6772360654802183"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i-1","id":"n0.60270874968986"}],"id":"n0.09590760222960326"}],"id":"n0.33457122341551315"}},"id":"n0.7535412572638782"}],"id":"n0.9779401532964331"}],"id":"n0.8094980225229713"}},"id":"n0.12916017780625033"},{"type":"single","text":"(","id":"n0.389893146341616"},{"text":"k","id":"n0.7519276750951587"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.48456216609838587"}],"id":"n0.40311262943803516"}],"id":"n0.41229014969930877"}},"id":"n0.32904290760446386"},{"type":"single","text":")","id":"n0.926963385687942"},{"text":"∩B","id":"n0.43985566958760125"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.10680831499932797"}],"id":"n0.6572494332746435"}],"id":"n0.7427357496726623"}},"id":"n0.5932481335626925"}],"id":"n0.6978594038323627"}],"id":"n0.34594129367678605"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.6187708919437953"}],"id":"n0.042711591360969026"}],"shape":{"data":{"p":{"x":252.17665890086874,"y":197.25928719454072},"rotation":0},"anchor":"bottom","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":false},"de21800500629938413":{"id":"de21800500629938413","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"k","id":"n0.17606698363362905"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i,B","id":"n0.7450250604138229"}],"id":"n0.6648854051906821"}],"id":"n0.4352032523118565"}},"id":"n0.25666558919911653"}],"id":"n0.2782420234917695"}],"id":"n0.8781721881795741"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.49016402408240745"}],"id":"n0.1896416755490855"}],"shape":{"data":{"p":{"x":480.777459591894,"y":237.11852343927842},"rotation":0},"anchor":"center","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":false},"de7681755659983813":{"id":"de7681755659983813","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"N","id":"n0.8598266127241212"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"b","id":"n0.0017962748863062927"}],"id":"n0.08958073569298453"}],"id":"n0.2416067324857083"}},"id":"n0.5166151180248175"},{"type":"single","text":"(","id":"n0.39989104774228545"},{"text":"k","id":"n0.9061465290849926"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.90102264919242"}],"id":"n0.3318560791748504"}],"id":"n0.9300836754341688"}},"id":"n0.020088615133755372"},{"type":"single","text":")","id":"n0.7680826366356408"}],"id":"n0.0055939857473688015"}],"id":"n0.701828177270583"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.09326835216358664"}],"id":"n0.0966276810352793"}],"shape":{"data":{"p":{"x":369.1365945266969,"y":231.4091147464744}},"anchor":"center","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":false},"de25165279858336675":{"id":"de25165279858336675","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"k","id":"n0.9761957803160111"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i,A","id":"n0.0021789147616821936"}],"id":"n0.20171417834692673"}],"id":"n0.44235161043010374"}},"id":"n0.8058520884189104"}],"id":"n0.30771344594166483"}],"id":"n0.7184483070857812"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.5185976614754455"}],"id":"n0.5468196537452479"}],"shape":{"data":{"p":{"x":471.277459591894,"y":285.6185234392784},"rotation":0},"anchor":"center","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":false},"de3104405477853185":{"id":"de3104405477853185","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"N","id":"n0.7882697542491204"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.6222508061737915"}],"id":"n0.9593333117547711"}],"id":"n0.23646231571219412"},"powerValue":{"lines":[{"blocks":[{"text":"G","id":"n0.419655474048807"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i-1","id":"n0.48385454015962237"}],"id":"n0.5934034705318751"}],"id":"n0.7220396198741703"}},"id":"n0.06588740019414052"}],"id":"n0.5001420305689612"}],"id":"n0.7669871416157932"}},"id":"n0.7104807849144901"},{"type":"single","text":"(","id":"n0.8775864376359939"},{"text":"k","id":"n0.15307336412009542"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.7339064195707112"}],"id":"n0.5436763710284709"}],"id":"n0.5860268654266063"}},"id":"n0.9616700642330929"},{"type":"single","text":")","id":"n0.010023930836436268"},{"text":"∩A","id":"n0.5168692399477055"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.22621609492266503"}],"id":"n0.5362361849584452"}],"id":"n0.7186940942547471"}},"id":"n0.7186105480504379"}],"id":"n0.04244171373431427"}],"id":"n0.9226264866505092"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.789435049963366"}],"id":"n0.396772177765528"}],"shape":{"data":{"p":{"x":567.297202125051,"y":311.88696272249234},"rotation":0},"anchor":"top","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":false},"de6105605663633311":{"id":"de6105605663633311","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"N","id":"n0.1678997957387387"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.028389499838341825"}],"id":"n0.6924529938494692"}],"id":"n0.3723326584779221"},"powerValue":{"lines":[{"blocks":[{"text":"G","id":"n0.8016443170106096"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i-1","id":"n0.8685623893294425"}],"id":"n0.42760491483420604"}],"id":"n0.3047753559222217"}},"id":"n0.31011781672519634"}],"id":"n0.6543002304880985"}],"id":"n0.8691948830728156"}},"id":"n0.20750551091528635"},{"type":"single","text":"(","id":"n0.24226023344206982"},{"text":"k","id":"n0.4633495200064883"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.7570356429203675"}],"id":"n0.6087904593862725"}],"id":"n0.2337242820100327"}},"id":"n0.7634988482720642"},{"type":"single","text":")","id":"n0.6181813681828563"},{"text":"∩B","id":"n0.49765242744527227"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.7179502359489185"}],"id":"n0.7784711265767796"}],"id":"n0.4860113949939562"}},"id":"n0.35714098545375283"}],"id":"n0.725458710184433"}],"id":"n0.9141728701984033"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.7974626569015872"}],"id":"n0.5755029569654848"}],"shape":{"data":{"p":{"x":569.8433255675354,"y":198.25928719454072},"rotation":0},"anchor":"bottom","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":false}},"connections":[],"intersections":{"id":"di9833419058199953","items":[],"style":{}},"shapes":[{"id":"da22181436622310136","data":[{"x":307.33333333333337,"y":15.333333333333314},{"x":307.33333333333337,"y":332.66666666666663}],"head":"no","tail":"no","shaft":"--","mVer":1,"style":{"thickness":2,"strokeColor":[155,155,155,1]}},{"id":"da9873848746720166","data":[{"x":6.666666666666657,"y":174.6333333333333},{"x":615.2,"y":174.6333333333333}],"head":"no","tail":"no","shaft":"--","mVer":1,"style":{"thickness":2,"strokeColor":[155,155,155,1]}},{"id":"dp09678993385539036","type":"ellipse","data":{"p1":{"x":153.9391818658598,"y":61.858968781940646},"p2":{"x":175.55035728329239,"y":83.47014419937311},"flipX":true},"style":{"thickness":2}},{"id":"dp5928812031939772","type":"ellipse","data":{"p1":{"x":233.16256539190695,"y":35.40400885045725},"p2":{"x":272.3335395841563,"y":74.57498304270668},"rotation":302.75},"style":{"strokeColor":[0,0,0,1],"fillColor":[208,2,27,0.7]}},{"id":"da11452991623397057","data":[{"x":172.33333333333334,"y":64.83333333333333},{"x":234.33333333333334,"y":48}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da689336208129746","data":[{"x":175.55035728329239,"y":72.66455649065688},{"x":236.33333333333331,"y":65.33333333333333}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"dp5695653245327148","type":"ellipse","data":{"p1":{"x":217.58605902601934,"y":79.10189393114506},"p2":{"x":283.62512093081546,"y":145.14095583594124},"rotation":280.96},"style":{"strokeColor":[0,0,0,1],"fillColor":[74,144,226,0.7]}},{"id":"da3783278769939673","data":[{"x":171.16666666666666,"y":81.82767079399117},{"x":217.5,"y":109}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da562171637544584","data":[{"x":173.21432621061342,"y":77.83333333333333},{"x":224.5,"y":92}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da29153342804416504","data":[{"x":225.13258724472976,"y":63.9145816318279},{"x":223,"y":52.66666666666666}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":1}},{"id":"da5516034702269903","data":[{"x":209.63258724472976,"y":101.58124829849457},{"x":214.5,"y":90.5}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":1}},{"id":"da1727934981033732","data":[{"x":87.66666666666666,"y":78.82767079399116},{"x":153.5,"y":77}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da43069062348557674","data":[{"x":83.21432621061342,"y":47.333333333333314},{"x":155.5,"y":65}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"dp3929348173165659","type":"ellipse","data":{"p1":{"x":16.78028947153447,"y":30.631532760008284},"p2":{"x":89.42751954722364,"y":103.27876283569742},"rotation":302.75},"style":{"strokeColor":[0,0,0,1],"fillColor":[126,211,33,0.7]}},{"id":"da7688092952711771","data":[{"x":135.13258724472976,"y":74.58124829849459},{"x":135.04291412683736,"y":62.841047261451735}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":1}},{"id":"dp9000380581873562","type":"ellipse","data":{"p1":{"x":469.9718718831778,"y":62.358968781940646},"p2":{"x":491.58304730061036,"y":83.97014419937311},"flipX":true},"style":{"thickness":2}},{"id":"da739794883452136","data":[{"x":403.6993566839846,"y":79.32767079399116},{"x":469.532690017318,"y":77.5}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da7515891720701993","data":[{"x":399.2470162279314,"y":47.833333333333314},{"x":471.532690017318,"y":65.5}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"dp7624501875339336","type":"ellipse","data":{"p1":{"x":332.8129794888525,"y":31.131532760008284},"p2":{"x":405.46020956454163,"y":103.77876283569742},"rotation":302.75},"style":{"strokeColor":[0,0,0,1],"fillColor":[126,211,33,0.7]}},{"id":"da6686887333214908","data":[{"x":451.6652772620477,"y":75.08124829849459},{"x":451.5756041441553,"y":63.341047261451735}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":1}},{"id":"dp15244213446299137","type":"ellipse","data":{"p1":{"x":460.4718718831778,"y":110.85896878194065},"p2":{"x":482.0830473006104,"y":132.47014419937312},"flipX":true},"style":{"thickness":2}},{"id":"da36264059739022825","data":[{"x":390.032690017318,"y":97.5},{"x":461.032690017318,"y":125.5}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da2832242489406456","data":[{"x":403.6993566839846,"y":79.32767079399116},{"x":468.032690017318,"y":111.5}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da49400036508749534","data":[{"x":449.1652772620477,"y":117.58124829849459},{"x":454.532690017318,"y":107.5}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":1}},{"id":"dg23201667576173945","entities":[{"id":"dp16347791823417857","type":"doc-rounded-rect","data":{"p1":{"x":26.64967834199227,"y":133.85},"p2":{"x":64.89967834199227,"y":163.75977443609023}},"style":{"fillColor":[155,155,155,0.5]}},{"id":"dl05052088386975595","linkedId":"de7765045494426801"}]},{"id":"dg6883465087679539","entities":[{"id":"dp8967978467687951","type":"doc-rounded-rect","data":{"p1":{"x":333.9163450086589,"y":133.85},"p2":{"x":372.1663450086589,"y":163.75977443609023}},"style":{"fillColor":[155,155,155,0.5]}},{"id":"dl9447510624873678","linkedId":"de2746680852491752"}]},{"id":"dp35882862515062475","type":"ellipse","data":{"p1":{"x":153.9391818658598,"y":223.31293573056217},"p2":{"x":175.55035728329236,"y":244.92411114799467},"flipX":true},"style":{"thickness":2}},{"id":"da2493661512431733","data":[{"x":87.6666666666666,"y":240.2816377426127},{"x":153.49999999999997,"y":238.45396694862154}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da7865905618658735","data":[{"x":83.2143262106134,"y":208.78730028195486},{"x":155.49999999999997,"y":226.45396694862154}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"dp2171544735840525","type":"ellipse","data":{"p1":{"x":16.78028947153447,"y":192.0854997086298},"p2":{"x":89.42751954722362,"y":264.73272978431896},"rotation":302.75},"style":{"strokeColor":[0,0,0,1],"fillColor":[126,211,33,0.7]}},{"id":"da3011231067876585","data":[{"x":135.6325872447297,"y":236.03521524711613},{"x":135.5429141268373,"y":224.29501421007328}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":1}},{"id":"dp26688018386533785","type":"ellipse","data":{"p1":{"x":144.4391818658598,"y":271.8129357305622},"p2":{"x":166.0503572832924,"y":293.42411114799467},"flipX":true},"style":{"thickness":2}},{"id":"da10678459055291634","data":[{"x":73.99999999999997,"y":258.45396694862154},{"x":144.99999999999997,"y":286.45396694862154}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da9977461846576332","data":[{"x":87.6666666666666,"y":240.2816377426127},{"x":151.99999999999997,"y":272.45396694862154}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da7455765432171115","data":[{"x":133.1325872447297,"y":278.5352152471161},{"x":138.49999999999997,"y":268.45396694862154}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":1}},{"id":"da6831355017266592","data":[{"x":166.30064331601542,"y":287.12063361528817},{"x":223.33333333333334,"y":293.3333333333333}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da6936276711902571","data":[{"x":166.0503572832924,"y":282.6185234392784},{"x":217.80064331601542,"y":273.62063361528817}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da6018702412916781","data":[{"x":209.80064331601542,"y":289.12063361528817},{"x":207.30064331601542,"y":278.12063361528817}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":1}},{"id":"dg5128480278905694","entities":[{"id":"dp7829885325504706","type":"doc-rounded-rect","data":{"p1":{"x":26.649678341992264,"y":294.1936501409775},"p2":{"x":64.89967834199227,"y":324.10342457706776}},"style":{"fillColor":[155,155,155,0.5]}},{"id":"dl13701192800054662","linkedId":"de693674574125986"}]},{"id":"dp9067583577251619","type":"ellipse","data":{"p1":{"x":469.9718718831777,"y":226.31293573056217},"p2":{"x":491.58304730061025,"y":247.92411114799467},"flipX":true},"style":{"thickness":2}},{"id":"da021888354952419142","data":[{"x":403.6993566839845,"y":243.2816377426127},{"x":469.53269001731786,"y":241.45396694862154}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da16437665356894327","data":[{"x":399.2470162279313,"y":211.78730028195486},{"x":471.53269001731786,"y":229.45396694862154}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"dp6978210942663718","type":"ellipse","data":{"p1":{"x":332.81297948885236,"y":195.0854997086298},"p2":{"x":405.4602095645415,"y":267.73272978431896},"rotation":302.75},"style":{"strokeColor":[0,0,0,1],"fillColor":[126,211,33,0.7]}},{"id":"da6426945013065339","data":[{"x":451.6652772620476,"y":239.03521524711613},{"x":451.5756041441552,"y":227.29501421007328}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":1}},{"id":"dp279886522107353","type":"ellipse","data":{"p1":{"x":460.4718718831777,"y":274.8129357305622},"p2":{"x":482.0830473006103,"y":296.42411114799467},"flipX":true},"style":{"thickness":2}},{"id":"da9796792389483315","data":[{"x":390.03269001731786,"y":261.45396694862154},{"x":461.03269001731786,"y":289.45396694862154}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da17262894723502042","data":[{"x":403.6993566839845,"y":243.2816377426127},{"x":468.03269001731786,"y":275.45396694862154}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da7761317567452739","data":[{"x":449.1652772620476,"y":281.5352152471161},{"x":454.53269001731786,"y":271.45396694862154}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":1}},{"id":"da15285894909230469","data":[{"x":482.3333333333333,"y":290.12063361528817},{"x":539.3333333333333,"y":296.12063361528817}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da8875174534723091","data":[{"x":482.0830473006103,"y":285.6185234392784},{"x":533.8333333333333,"y":276.62063361528817}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da37034494935338524","data":[{"x":525.8333333333333,"y":292.12063361528817},{"x":523.3333333333333,"y":281.12063361528817}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":1}},{"id":"dg4905105471007787","entities":[{"id":"dp6453451362898857","type":"doc-rounded-rect","data":{"p1":{"x":333.9163450086589,"y":294.1936501409775},"p2":{"x":372.1663450086589,"y":324.10342457706776}},"style":{"fillColor":[155,155,155,0.5]}},{"id":"dl5081766153258873","linkedId":"de29918931349792754"}]},{"id":"dp20405948284397213","type":"ellipse","data":{"p1":{"x":549.8292320585737,"y":35.40400885045724},"p2":{"x":589.000206250823,"y":74.57498304270666},"rotation":302.75},"style":{"strokeColor":[0,0,0,1],"fillColor":[208,2,27,0.7]}},{"id":"da6178426496011642","data":[{"x":489,"y":64.83333333333331},{"x":551,"y":47.999999999999986}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da7194239910301174","data":[{"x":492.21702394995907,"y":72.66455649065686},{"x":553,"y":65.33333333333331}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"dp9737227549289602","type":"ellipse","data":{"p1":{"x":534.252725692686,"y":79.10189393114504},"p2":{"x":600.2917875974822,"y":145.1409558359412},"rotation":280.96},"style":{"strokeColor":[0,0,0,1],"fillColor":[74,144,226,0.7]}},{"id":"da704117769915457","data":[{"x":487.83333333333337,"y":81.82767079399116},{"x":534.1666666666667,"y":108.99999999999999}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da6233768251573941","data":[{"x":489.8809928772801,"y":77.83333333333331},{"x":541.1666666666667,"y":91.99999999999999}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da32316046647271035","data":[{"x":541.7992539113965,"y":63.914581631827886},{"x":539.6666666666667,"y":52.66666666666664}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":1}},{"id":"da2589539957217737","data":[{"x":526.2992539113965,"y":101.58124829849456},{"x":531.1666666666667,"y":90.49999999999999}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":1}},{"id":"dp7938896756904461","type":"ellipse","data":{"p1":{"x":233.16256539190698,"y":196.7373421837906},"p2":{"x":272.3335395841563,"y":235.90831637604},"rotation":302.75},"style":{"strokeColor":[0,0,0,1],"fillColor":[208,2,27,0.7]}},{"id":"da909479126527639","data":[{"x":172.33333333333331,"y":226.16666666666666},{"x":234.33333333333331,"y":209.33333333333331}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da12170615642383265","data":[{"x":175.55035728329239,"y":233.9978898239902},{"x":236.33333333333331,"y":226.66666666666666}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"dp3252790741366527","type":"ellipse","data":{"p1":{"x":217.5860590260193,"y":240.43522726447839},"p2":{"x":283.6251209308155,"y":306.4742891692746},"rotation":280.96},"style":{"strokeColor":[0,0,0,1],"fillColor":[74,144,226,0.7]}},{"id":"da7100467652360782","data":[{"x":171.16666666666669,"y":243.1610041273245},{"x":217.50000000000006,"y":270.33333333333337}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da8963781613740296","data":[{"x":173.21432621061342,"y":239.16666666666666},{"x":224.50000000000006,"y":253.33333333333331}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da8350947524676868","data":[{"x":225.1325872447298,"y":225.24791496516121},{"x":223.00000000000006,"y":214}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":1}},{"id":"da3935692703546734","data":[{"x":209.6325872447298,"y":262.9145816318279},{"x":214.50000000000006,"y":251.83333333333331}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":1}},{"id":"dp827870488566085","type":"ellipse","data":{"p1":{"x":549.8292320585737,"y":199.7373421837906},"p2":{"x":589.000206250823,"y":238.90831637604},"rotation":302.75},"style":{"strokeColor":[0,0,0,1],"fillColor":[208,2,27,0.7]}},{"id":"da16288046821193558","data":[{"x":489,"y":229.16666666666666},{"x":551,"y":212.33333333333331}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da9901124272248998","data":[{"x":492.21702394995907,"y":236.9978898239902},{"x":553,"y":229.66666666666666}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"dp5914523916499952","type":"ellipse","data":{"p1":{"x":533.252725692686,"y":243.43522726447839},"p2":{"x":599.2917875974822,"y":309.4742891692746},"rotation":280.96},"style":{"strokeColor":[0,0,0,1],"fillColor":[74,144,226,0.7]}},{"id":"da9519968744741594","data":[{"x":541.7992539113965,"y":228.24791496516121},{"x":539.6666666666667,"y":217}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":1}}],"settings":{"grid":true,"diagramHeight":339.1848958333333},"id":"n0.004300098539481656"}],"id":"n0.4052119529819904"}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":739,"delayRenderCache":{"av":739,"map":{}}}

==> figs/docs/ac48574b-5c4e-4f5c-a585-955f497d7928 <==
{"id":"r0.9088962749303412","lines":[{"blocks":[{"text":"\\diagram","type":"composite","elements":{"de17675806290195006":{"id":"de17675806290195006","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"e","id":"n0.7496548659649882"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"0","id":"n0.04896796976257578"}],"id":"n0.09838349716907646"}],"id":"n0.4083766328073408"}},"id":"n0.4141654658104379"}],"id":"n0.7799475278098964"}],"id":"n0.8300521941018906"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.8837430411515108"}],"id":"n0.4134203640701819"}],"shape":{"data":{"p":{"x":259.6,"y":124.80000000000007}},"anchor":"left-top"},"isTextMode":true},"de4182436857327321":{"id":"de4182436857327321","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"e","style":{"mathModeType":"\\displaystyle"},"id":"n0.3467736849283998"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"1","id":"n0.0769248718134854"}],"id":"n0.036373192057555626"}],"id":"n0.8143504609030374"}},"style":{"mathModeType":"\\displaystyle"},"id":"n0.43282006981169063"}],"id":"n0.6450390308932508"}],"id":"n0.4085970686095979"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.08104549023770646"}],"id":"n0.7050163486810095"}],"shape":{"data":{"p":{"x":132.00000000000006,"y":124.87343750000002}},"anchor":"left-top"},"isTextMode":true},"de11996678676955996":{"id":"de11996678676955996","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"-","id":"n0.14556974428848957"}],"id":"n0.7945217314890181"}],"id":"n0.5722176415681899"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.42183711514499933"}],"id":"n0.0529148522963514"}],"shape":{"data":{"p":{"x":197,"y":64}},"anchor":"left-top"},"isTextMode":true},"de28893533177995834":{"id":"de28893533177995834","lines":[{"blocks":[{"text":"DATE","id":"n0.6846621158484627"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"=","id":"n0.14382496599832129"}],"id":"n0.2523473993708698"}],"id":"n0.9606784068297944"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.13019448331988737"}],"id":"n0.08471102814235776"}],"shape":{"data":{"p":{"x":17,"y":63}},"anchor":"left-top"},"isTextMode":true}},"connections":[],"intersections":{"id":"di007212778813125098","items":[],"style":{}},"shapes":[{"id":"dp8906017191472704","type":"ellipse","data":{"p1":{"x":96.10206044514979,"y":28.902060445149743},"p2":{"x":186.20000000000005,"y":119.00000000000006}}},{"id":"dp7583607920285613","type":"circle","data":{"p1":{"x":154.68580451798374,"y":39.51448038176201},"p2":{"x":164.28006934522807,"y":49.108745209006344}},"style":{"fillColor":[70,114,191,1]}},{"id":"dp8942160332641216","type":"circle","data":{"p1":{"x":112.11125434708697,"y":44.31161279538418},"p2":{"x":121.7055191743313,"y":53.90587762262852},"rotation":318.91},"style":{"fillColor":[70,114,191,1]}},{"id":"dp7473064183865517","type":"ellipse","data":{"p1":{"x":169.0772017588502,"y":75.13318855290663},"p2":{"x":178.67146658609454,"y":84.72745338015093}},"style":{"fillColor":[70,114,191,1]}},{"id":"dp06411734773062827","type":"circle","data":{"p1":{"x":136.35389780895275,"y":69.15389780895273},"p2":{"x":145.94816263619708,"y":78.74816263619707}},"style":{"fillColor":[247,31,31,1]}},{"id":"dp3157089948447107","type":"ellipse","data":{"p1":{"x":140.29440727711722,"y":106.07469262076955},"p2":{"x":149.88867210436155,"y":115.66895744801391}},"style":{"fillColor":[70,114,191,1]}},{"id":"dp1949607661579318","type":"ellipse","data":{"p1":{"x":104.91555572665375,"y":78.49118124244208},"p2":{"x":114.50982055389807,"y":88.0854460696865},"rotation":346.98},"style":{"fillColor":[70,114,191,1]}},{"id":"dg0038232066435830436","entities":[{"id":"da7893714881617722","data":[{"x":156.8445141041137,"y":48.38917534696303},{"x":144.37196982869608,"y":69.97627120826277}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da035733552553224524","data":[{"x":120.0612718855516,"y":52.72423892126359},{"x":137.65598444962504,"y":70.93569769098721}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da34736354456500496","data":[{"x":169.0772017588502,"y":78.49118124244211},{"x":145.5712529321016,"y":75.13318855290663}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da650066252629711","data":[{"x":114.38649339222201,"y":82.20756213017796},{"x":136.9364145875817,"y":76.33247165631215}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da04754852627627537","data":[{"x":141.15103022257495,"y":78.74816263619707},{"x":145.09153969073938,"y":106.07469262076955}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}}],"data":{"rotation":0}},{"id":"dp7027685761830689","type":"ellipse","data":{"p1":{"x":279.64544786854583,"y":40.42602022404401},"p2":{"x":289.06933339744626,"y":49.84990575294438}},"style":{"fillColor":[70,114,191,1]}},{"id":"dp26710259711408857","type":"ellipse","data":{"p1":{"x":237.8269558340503,"y":45.137962988494195},"p2":{"x":247.25084136295072,"y":54.561848517394594},"rotation":318.91},"style":{"fillColor":[70,114,191,1]}},{"id":"dp97748888177145","type":"ellipse","data":{"p1":{"x":293.78127616189647,"y":75.41219525008674},"p2":{"x":303.2051616907968,"y":84.83608077898714}},"style":{"fillColor":[70,114,191,1]}},{"id":"dp42687810546100735","type":"ellipse","data":{"p1":{"x":261.63908745812466,"y":69.53908745812478},"p2":{"x":271.06297298702503,"y":78.96297298702518}},"style":{"fillColor":[70,114,191,1]}},{"id":"dp45816895459461615","type":"ellipse","data":{"p1":{"x":265.50961957519525,"y":105.8042260807905},"p2":{"x":274.9335051040957,"y":115.2281116096909}},"style":{"fillColor":[70,114,191,1]}},{"id":"dp7504780106577442","type":"ellipse","data":{"p1":{"x":230.75904168737497,"y":78.71055518520183},"p2":{"x":240.1829272162754,"y":88.13444071410225},"rotation":346.98},"style":{"fillColor":[70,114,191,1]}},{"id":"da28842294053824924","data":[{"x":281.76582211254845,"y":49.14311433827686},{"x":269.51477092497794,"y":70.34685677830277}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da8456391476553058","data":[{"x":245.63579336191327,"y":53.40119389104319},{"x":262.9180510547477,"y":71.2892453311928}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da33536693661705064","data":[{"x":293.78127616189647,"y":78.71055518520186},{"x":270.6927566160905,"y":75.41219525008674}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da10929102746636055","data":[{"x":240.0617901541694,"y":82.36093889864318},{"x":262.21125964008013,"y":76.59018094119926}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da27034402409759384","data":[{"x":266.3510302225749,"y":78.96297298702518},{"x":270.22156233964546,"y":105.8042260807905}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"dp0068896259409778615","type":"ellipse","data":{"p1":{"x":222.10206044514968,"y":30.002060445149766},"p2":{"x":310.6,"y":118.5000000000002}}}],"settings":{"grid":true,"diagramHeight":170.265625,"gridBold":false,"gridSize":10},"id":"n0.6706229370812695"}],"id":"n0.8604242159833757"}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":21,"delayRenderCache":{"av":21,"map":{}}}

==> figs/docs/aebaf945-d51f-491c-8b58-3cf3e54de587 <==
{"id":"r0.1520862138937733","lines":[{"blocks":[{"text":"\\diagram","type":"composite","elements":{},"connections":[],"intersections":{"id":"di018738070182718003","items":[],"style":{}},"shapes":[{"id":"dp48920669465345235","type":"ellipse","data":{"p1":{"x":153.29440727711722,"y":200.3236383304401},"p2":{"x":186.71968329997304,"y":233.74891435329593}},"style":{"fillColor":"none"}},{"id":"dp509957996555537","type":"ellipse","data":{"p1":{"x":192.25037935120338,"y":103.75910268422604},"p2":{"x":225.6756553740592,"y":137.18437870708186}},"style":{"fillColor":"none"}},{"id":"dp03406273901071444","type":"ellipse","data":{"p1":{"x":204.96670401123384,"y":202.74060751342537},"p2":{"x":238.3919800340896,"y":236.16588353628117},"rotation":12.59},"style":{"fillColor":"none"}},{"id":"dp29905531123660034","type":"ellipse","data":{"p1":{"x":284.7964198266168,"y":118.14490904464816},"p2":{"x":318.2216958494729,"y":151.57018506750393},"rotation":11.34},"style":{"fillColor":[255,255,255,1]}},{"id":"dp6846493386905885","type":"ellipse","data":{"p1":{"x":279.5652175137361,"y":198.57464460518992},"p2":{"x":312.9904935365919,"y":231.99992062804577},"rotation":1.24},"style":{"fillColor":"none"}},{"id":"dp6190289844290746","type":"ellipse","data":{"p1":{"x":373.72685914559,"y":193.6703924368643},"p2":{"x":407.1521351684457,"y":227.09566845972},"rotation":312.14},"style":{"fillColor":"none"}},{"id":"dp9032594962074556","type":"ellipse","data":{"p1":{"x":369.80345741092947,"y":93.29669805846447},"p2":{"x":403.22873343378535,"y":126.7219740813203}},"style":{"fillColor":"none"}},{"id":"dp5732142832034277","type":"ellipse","data":{"p1":{"x":452.349497886343,"y":128.8143907450398},"p2":{"x":485.77477390919876,"y":162.2396667678956}},"style":{"fillColor":"none"}},{"id":"da35995592625841355","data":[{"x":175.33333333333334,"y":201.33333333333334},{"x":198,"y":132}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da10970030098735228","data":[{"x":209.96301736263126,"y":137.18437870708186},{"x":220.66666666666666,"y":202.66666666666666}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da41032387745803844","data":[{"x":226.6756553740592,"y":120.47174069565395},{"x":285.1226902403077,"y":131.57132943503288}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da2393684724099212","data":[{"x":298.2228402170017,"y":151.2439146538132},{"x":296.639523585014,"y":198.57855838298735}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da4045112374071389","data":[{"x":314.29829411481217,"y":124.5923043139567},{"x":369.80345741092947,"y":110.00933606989238}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da6660013127665139","data":[{"x":386.51609542235735,"y":126.7219740813203},{"x":390.8046279406934,"y":194.23268510418194}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da44824060765404394","data":[{"x":406.49823487933577,"y":204.0411894408334},{"x":457.3333333333333,"y":158}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da8881215515149321","data":[{"x":315.25,"y":144.5},{"x":378.04694881946455,"y":199.16977868966148}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da37423110631872314","data":[{"x":183.5,"y":206.75},{"x":286,"y":140.75}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2,"strokeColor":[0,0,0,1]}},{"id":"da4798773022604228","data":[{"x":187.71968329997304,"y":217.03627634186802},{"x":205.5,"y":218.75}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2,"strokeColor":[0,0,0,1]}},{"id":"da5973583144126775","data":[{"x":236.5,"y":211.25},{"x":291.5,"y":148.25}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2,"strokeColor":[0,0,0,1]}},{"id":"da8890019687995259","data":[{"x":220,"y":107.25},{"x":374.5,"y":98.25}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2,"strokeColor":[0,0,0,1]}},{"id":"da3903429004805241","data":[{"x":222.5,"y":131.25},{"x":284,"y":204.25}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2,"strokeColor":[0,0,0,1]}},{"id":"da9330067255231866","data":[{"x":225.5,"y":126.25},{"x":373.5,"y":207.25}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2,"strokeColor":[0,0,0,1]}},{"id":"da9872380576646682","data":[{"x":312.9865797587944,"y":215.64895067646788},{"x":374.5,"y":213.25}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2,"strokeColor":[0,0,0,1]}},{"id":"da6858493343189613","data":[{"x":308,"y":202.5},{"x":375.5,"y":122.5}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2,"strokeColor":[0,0,0,1]}},{"id":"da028319408785988598","data":[{"x":317.89542543578216,"y":138.1437646771192},{"x":451.349497886343,"y":145.5270287564677}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2,"strokeColor":[0,0,0,1]}},{"id":"da9212769102748637","data":[{"x":403.22873343378535,"y":110.00933606989238},{"x":457,"y":132.75}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2,"strokeColor":[0,0,0,1]}}],"settings":{"grid":true},"id":"n0.23031347251131273"}],"id":"n0.6370818825687694"}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":106,"delayRenderCache":{"av":106,"map":{}}}

==> figs/docs/b5db53c3-ed79-42fd-bd24-8ffdbac8a8d6 <==
{"id":"r0.34336831155681624","lines":[{"blocks":[{"text":"\\diagram","type":"composite","elements":{"de836427235990252":{"id":"de836427235990252","lines":[{"blocks":[{"id":"n0.3426391635186823","text":"5"}],"id":"n0.5143212381753117"}],"shape":{"data":{"p":{"x":128.8643076797487,"y":153.30550394860256},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de14847325276395607":{"id":"de14847325276395607","lines":[{"blocks":[{"text":"2","id":"n0.38554956136334795"}],"id":"n0.21958814244035718"}],"shape":{"data":{"p":{"x":65.72367457392377,"y":60.256149897913346},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de047655461387096976":{"id":"de047655461387096976","lines":[{"blocks":[{"id":"n0.905644007753232","text":"4"}],"id":"n0.5033608559684208"}],"shape":{"data":{"p":{"x":66.83140497928915,"y":256.32443164757996},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de33823805891668557":{"id":"de33823805891668557","lines":[{"blocks":[{"id":"n0.05753358249009888","text":"1"}],"id":"n0.08811149330228929"}],"shape":{"data":{"p":{"x":240.7450786216489,"y":54.71749787108662},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de22964791973931042":{"id":"de22964791973931042","lines":[{"blocks":[{"id":"n0.18166790614302464","text":"6"}],"id":"n0.28036159175159003"}],"shape":{"data":{"p":{"x":347.0871975367224,"y":145.55139111104518},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de6279161930503641":{"id":"de6279161930503641","lines":[{"blocks":[{"id":"n0.14329687821185733","text":"3"}],"id":"n0.12773350966359276"}],"shape":{"data":{"p":{"x":251.82238267530238,"y":245.24712759392654},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de5845445468181816":{"id":"de5845445468181816","lines":[{"blocks":[{"text":"7","id":"n0.8921810337013605"}],"id":"n0.15058957150124863"}],"shape":{"data":{"p":{"x":357.0567711850105,"y":296.2027262407325},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de4688387060585977":{"id":"de4688387060585977","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"*","id":"n0.5692598508716165"}],"id":"n0.7763648378305781"}],"id":"n0.5928401620442478"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.9332433638967785"}],"id":"n0.01474219324028292"}],"shape":{"data":{"p":{"x":240,"y":17.00000000000003}},"anchor":"left-top"},"isTextMode":true},"de9795480303730029":{"id":"de9795480303730029","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"e","id":"n0.8366256680734776"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"1","id":"n0.8854487030292917"}],"id":"n0.37261786469813507"}],"id":"n0.30350195639258937"}},"id":"n0.9882368927270646"}],"id":"n0.7007059329186192"}],"id":"n0.24952047340926242"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.0409855798010621"}],"id":"n0.3720045924030888"}],"shape":{"data":{"p":{"x":62,"y":19}},"anchor":"left-top","style":{"textColor":[247,31,31,1]}},"isTextMode":true},"de012542281841566805":{"id":"de012542281841566805","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"*","id":"n0.8132672254296822"}],"id":"n0.4732932208503853"}],"id":"n0.8129480879016264"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.9699659726957692"}],"id":"n0.45403306019121903"}],"shape":{"data":{"p":{"x":254.33333333333334,"y":284.66666666666663}},"anchor":"left-top"},"isTextMode":true},"de9142213739989218":{"id":"de9142213739989218","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"e","id":"n0.588317368696863"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.420130062843697","text":"0"}],"id":"n0.6203986015621796"}],"id":"n0.26673400961970417"}},"id":"n0.7097175582645567"}],"id":"n0.17571138349715132"}],"id":"n0.849374801028796"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.055967090579388756"}],"id":"n0.0918075743313933"}],"shape":{"data":{"p":{"x":385.33333333333337,"y":143}},"anchor":"left-top","style":{"textColor":[70,114,191,1]}},"isTextMode":true},"de06258010549000437":{"id":"de06258010549000437","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"e","id":"n0.945366192915627"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.23421571098424487","text":"1"}],"id":"n0.9453198660745394"}],"id":"n0.2326935894069826"}},"id":"n0.50683558397918"}],"id":"n0.000165121029861659"}],"id":"n0.26206442836666377"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.9706488528175126"}],"id":"n0.10296542998089975"}],"shape":{"data":{"p":{"x":61.333333333333314,"y":293.99999999999994}},"anchor":"left-top","style":{"textColor":[247,31,31,1]}},"isTextMode":true},"de7796366757538453":{"id":"de7796366757538453","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"*","id":"n0.4500820839360742"}],"id":"n0.007479953940481288"}],"id":"n0.25348141147459247"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.7232115232225154"}],"id":"n0.04000114835381452"}],"shape":{"data":{"p":{"x":94.33333333333337,"y":149.66666666666663}},"anchor":"left-top"},"isTextMode":true},"de8239034622263439":{"id":"de8239034622263439","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"*","id":"n0.15627011725048767"}],"id":"n0.6334024554189228"}],"id":"n0.20607587643984027"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.6582372479128771"}],"id":"n0.3388743151506801"}],"shape":{"data":{"p":{"x":395.33333333333337,"y":296.66666666666663}},"anchor":"left-top"},"isTextMode":true}},"connections":[],"intersections":{"id":"di018738070182718003","items":[],"style":{}},"shapes":[{"id":"dp9125615449493809","type":"ellipse","data":{"p1":{"x":44.95402865523873,"y":42.85625299199422},"p2":{"x":100.49332049260892,"y":98.39554482936434}},"style":{"fillColor":"none"}},{"id":"dp6696137576130887","type":"ellipse","data":{"p1":{"x":45.52895517377332,"y":238.64630089431083},"p2":{"x":101.06824701114326,"y":294.1855927316803},"rotation":12.59},"style":{"fillColor":"none"}},{"id":"dp2099518139314911","type":"ellipse","data":{"p1":{"x":108.38664482631847,"y":135.74529364125738},"p2":{"x":163.92593666368901,"y":191.28458547862738},"rotation":11.34},"style":{"fillColor":[255,255,255,1]}},{"id":"dp7129976937210605","type":"ellipse","data":{"p1":{"x":336.79390961187244,"y":278.949097787917},"p2":{"x":392.33320144924306,"y":334.4883896252872},"rotation":1.24},"style":{"fillColor":"none"}},{"id":"dp5702366916287585","type":"ellipse","data":{"p1":{"x":231.22913809978522,"y":228.00619298050708},"p2":{"x":286.7684299371551,"y":283.5454848178769},"rotation":312.14},"style":{"fillColor":"none"}},{"id":"dp5781029111286848","type":"ellipse","data":{"p1":{"x":219.72524418472122,"y":37.96336472513116},"p2":{"x":275.26453602209136,"y":93.50265656250127}},"style":{"fillColor":"none"}},{"id":"dp37593405052156936","type":"ellipse","data":{"p1":{"x":325.31306594751015,"y":128.5497234540565},"p2":{"x":380.85235778488016,"y":184.0890152914266}},"style":{"fillColor":"none"}},{"id":"da19824323105390684","data":[{"x":66.0772921417317,"y":239.0773063107636},{"x":66.0772921417317,"y":97.28781442399901}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da39427378311335093","data":[{"x":120.3560820046338,"y":185.9062468532269},{"x":91.55509146513478,"y":245.7236887429557}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da958797173277401","data":[{"x":87.12416984367336,"y":95.07235361326829},{"x":119.24835159926843,"y":142.7047610439783}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da011781522350808649","data":[{"x":359.62584956354925,"y":183.69078604249617},{"x":365.16450159037583,"y":278.9556009039161}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da19438407183948536","data":[{"x":149.15707254413283,"y":139.38156982788226},{"x":220.05181848751522,"y":72.91774550596136}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da04075255648400633","data":[{"x":275.4383387557826,"y":71.81001510059599},{"x":346.33308469916494,"y":129.4119961795941}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da9520026185119386","data":[{"x":284.854047201388,"y":244.06209313490763},{"x":341.3482978750208,"y":180.92146002908285}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da2605956473538118","data":[{"x":158.57278098973836,"y":180.92146002908285},{"x":233.34458335189936,"y":244.06209313490763}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da9232359559871122","data":[{"x":99,"y":61},{"x":219.72524418472125,"y":65.73301064381621}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2,"strokeColor":[0,0,0,1]}},{"id":"da47121422749041764","data":[{"x":100.49332049260892,"y":70.62589891067928},{"x":247,"y":230}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2,"strokeColor":[0,0,0,1]}},{"id":"da6014248829557596","data":[{"x":102,"y":267},{"x":233,"y":265}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2,"strokeColor":[0,0,0,1]}},{"id":"da9826352489746542","data":[{"x":100,"y":260},{"x":240,"y":92}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2,"strokeColor":[0,0,0,1]}},{"id":"da13599011810051032","data":[{"x":161,"y":152},{"x":325.31306594751015,"y":156.31936937274156}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2,"strokeColor":[0,0,0,1]}},{"id":"da7166093305161052","data":[{"x":253,"y":93},{"x":259,"y":228}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2,"strokeColor":[0,0,0,1]}},{"id":"da656331592549618","data":[{"x":263,"y":87},{"x":348,"y":285}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2,"strokeColor":[0,0,0,1]}},{"id":"da724351495425859","data":[{"x":284,"y":267},{"x":336.80041272787156,"y":306.1177976467841}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2,"strokeColor":[0,0,0,1]}}],"settings":{"grid":true,"diagramHeight":358.6640625},"id":"n0.9367293560884689"}],"id":"n0.01597078583634537"}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":101,"delayRenderCache":{"av":101,"map":{}}}

==> figs/docs/b7c322b3-b690-4db0-b62b-bb4cc7c5fe38 <==
{"id":"r0.09751365378023824","lines":[{"blocks":[{"text":"\\diagram","type":"composite","elements":{"de3776378819029238":{"id":"de3776378819029238","lines":[{"blocks":[{"text":"1","id":"n0.27706544426750446"}],"id":"n0.838705474495796"}],"shape":{"data":{"p":{"x":128.8643076797487,"y":153.30550394860256},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de07996317660746421":{"id":"de07996317660746421","lines":[{"blocks":[{"text":"2","id":"n0.7376408784455493"}],"id":"n0.9869551168709203"}],"shape":{"data":{"p":{"x":65.72367457392377,"y":60.256149897913346},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de4288158533496289":{"id":"de4288158533496289","lines":[{"blocks":[{"text":"3","id":"n0.48723843543228207"}],"id":"n0.18392952485918168"}],"shape":{"data":{"p":{"x":66.83140497928915,"y":256.32443164757996},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de30289366292137654":{"id":"de30289366292137654","lines":[{"blocks":[{"text":"4","id":"n0.8879713644266161"}],"id":"n0.7812739630569621"}],"shape":{"data":{"p":{"x":240.7450786216489,"y":54.71749787108662},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de7082483270264905":{"id":"de7082483270264905","lines":[{"blocks":[{"text":"5","id":"n0.9938723841878196"}],"id":"n0.18923735903489547"}],"shape":{"data":{"p":{"x":347.0871975367224,"y":145.55139111104518},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de6419094039918298":{"id":"de6419094039918298","lines":[{"blocks":[{"text":"6","id":"n0.08301971637245531"}],"id":"n0.992098909241069"}],"shape":{"data":{"p":{"x":251.82238267530238,"y":245.24712759392654},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de7572450417813497":{"id":"de7572450417813497","lines":[{"blocks":[{"text":"7","id":"n0.6296798333208993"}],"id":"n0.13020950444801516"}],"shape":{"data":{"p":{"x":357.0567711850105,"y":296.2027262407325},"rotation":0},"anchor":"left-top"},"isTextMode":true}},"connections":[],"intersections":{"id":"di018738070182718003","items":[],"style":{}},"shapes":[{"id":"dp30563116406690516","type":"ellipse","data":{"p1":{"x":44.95402865523873,"y":42.856252991994204},"p2":{"x":100.49332049260892,"y":98.39554482936433}},"style":{"fillColor":[247,31,31,1]}},{"id":"dp3221896294664819","type":"ellipse","data":{"p1":{"x":45.52895517377332,"y":238.64630089431083},"p2":{"x":101.06824701114326,"y":294.1855927316803},"rotation":12.59},"style":{"fillColor":[70,114,191,1]}},{"id":"dp38265895108698333","type":"ellipse","data":{"p1":{"x":108.38664482631847,"y":135.74529364125738},"p2":{"x":163.92593666368901,"y":191.28458547862738},"rotation":11.34},"style":{"fillColor":[70,114,191,1]}},{"id":"dp6139758446433232","type":"ellipse","data":{"p1":{"x":336.79390961187244,"y":278.949097787917},"p2":{"x":392.33320144924306,"y":334.4883896252872},"rotation":1.24},"style":{"fillColor":[70,114,191,1]}},{"id":"dp002639172811321311","type":"ellipse","data":{"p1":{"x":231.22913809978522,"y":228.00619298050708},"p2":{"x":286.7684299371551,"y":283.5454848178769},"rotation":312.14},"style":{"fillColor":[70,114,191,1]}},{"id":"dp8960828151986147","type":"ellipse","data":{"p1":{"x":219.72524418472122,"y":37.96336472513116},"p2":{"x":275.26453602209136,"y":93.50265656250127}},"style":{"fillColor":[247,31,31,1]}},{"id":"dp6881270808520517","type":"ellipse","data":{"p1":{"x":325.31306594751015,"y":128.5497234540565},"p2":{"x":380.85235778488016,"y":184.0890152914266}},"style":{"fillColor":[70,114,191,1]}},{"id":"da2949854278862667","data":[{"x":66.0772921417317,"y":239.0773063107636},{"x":66.0772921417317,"y":97.28781442399901}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da4802642471037637","data":[{"x":120.3560820046338,"y":185.9062468532269},{"x":91.55509146513478,"y":245.7236887429557}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da4158019251323506","data":[{"x":87.12416984367336,"y":95.07235361326829},{"x":119.24835159926843,"y":142.7047610439783}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da25512174600731385","data":[{"x":359.62584956354925,"y":183.69078604249617},{"x":365.16450159037583,"y":278.9556009039161}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da002685686366488804","data":[{"x":149.15707254413283,"y":139.38156982788226},{"x":220.05181848751522,"y":72.91774550596136}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da29791343851596297","data":[{"x":275.4383387557826,"y":71.81001510059599},{"x":346.33308469916494,"y":129.4119961795941}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da9881386384414359","data":[{"x":284.854047201388,"y":244.06209313490763},{"x":341.3482978750208,"y":180.92146002908285}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da2674472279715796","data":[{"x":158.57278098973836,"y":180.92146002908285},{"x":233.34458335189936,"y":244.06209313490763}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"dp33469625825176075","type":"circle","data":{"p1":{"x":34.82262539326754,"y":32.72484973002298},"p2":{"x":110.62472375458012,"y":108.52694809133556}},"style":{"strokeType":{"type":"dash","pattern":[6,6]},"strokeColor":[247,31,31,0.5],"thickness":2}},{"id":"dp2545097050726708","type":"circle","data":{"p1":{"x":209.59384092275002,"y":27.831961463159928},"p2":{"x":285.3959392840626,"y":103.6340598244725}},"style":{"strokeType":{"type":"dash","pattern":[6,6]},"strokeColor":[247,31,31,0.5],"thickness":2}},{"id":"dp9718196664861285","type":"circle","data":{"p1":{"x":326.6625063499015,"y":268.81769452594585},"p2":{"x":402.46460471121406,"y":344.6197928872584}},"style":{"strokeType":{"type":"dash","pattern":[6,6]},"strokeColor":[70,114,191,0.5],"thickness":2}}],"settings":{"grid":true,"diagramHeight":358.6640625},"id":"n0.725290060590942"}],"id":"n0.6925701259602852"}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":94,"delayRenderCache":{"av":94,"map":{}}}

==> figs/docs/b883ad8f-2f35-480f-bb41-6ea6ceabe751 <==
{"id":"r0.9600904132466492","lines":[{"id":"n0.23592352158215357","blocks":[]},{"id":"n0.8610334732055211","blocks":[{"id":"n0.8636753557032222","text":"\\diagram","type":"composite","elements":{"de20266363427018663":{"id":"de20266363427018663","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"k","id":"n0.20485150670863095"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.31951088626023383"}],"id":"n0.37613534664111503"}],"id":"n0.659544896958147"}},"id":"n0.116114318893207"}],"id":"n0.9182901097766887"}],"id":"n0.6081122667562879"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.9511234181788533"}],"id":"n0.1356827367231055"}],"shape":{"data":{"p":{"x":66.07810290790941,"y":55.49788982399021},"rotation":0},"anchor":"center","settings":{"fontSize":"\\normalsize"}},"isTextMode":true,"isInGroup":false},"de826339790086142":{"id":"de826339790086142","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"N","id":"n0.33746310782508937"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.18439710091482553"}],"id":"n0.5970804194566492"}],"id":"n0.7804381177492692"}},"id":"n0.2791656544666814"},{"type":"single","text":"(","id":"n0.11207163969117695"},{"text":"k","id":"n0.5030823773958004"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.07844821131863622"}],"id":"n0.8960752742036528"}],"id":"n0.009630912462495145"}},"id":"n0.5043605702943774"},{"type":"single","text":")","id":"n0.9386700324747226"},{"text":"∩A","id":"n0.21407774445219552"},{"text":"\\power","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"type":"single","text":"(","id":"n0.20570741022554007"},{"text":"1","id":"n0.04397550114657167"},{"type":"single","text":")","id":"n0.18823209890602022"}],"id":"n0.7524458945841703"}],"id":"n0.18396435658996824"}},"id":"n0.5400852322382315"}],"id":"n0.2392227061557679"}],"id":"n0.17673404247147384"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.5136444063354666"}],"id":"n0.2596427110109174"}],"shape":{"data":{"p":{"x":52.74978767470243,"y":135.46603714337022},"rotation":0},"anchor":"top","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":false},"de18672678603594162":{"id":"de18672678603594162","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"N","id":"n0.9298232819894312"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.3526360519753762"}],"id":"n0.023819460607561238"}],"id":"n0.076122439997105"}},"id":"n0.3359036105188984"},{"type":"single","text":"(","id":"n0.6089671999511295"},{"text":"k","id":"n0.1750684840548029"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.002430687648571128"}],"id":"n0.23052289005143978"}],"id":"n0.8967021545733473"}},"id":"n0.19292718467472336"},{"type":"single","text":")","id":"n0.1723755828900584"},{"text":"∩B","id":"n0.05024863109876687"},{"text":"\\power","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"type":"single","text":"(","id":"n0.05979690782896219"},{"text":"1","id":"n0.8352743680959733"},{"type":"single","text":")","id":"n0.5582901632699591"}],"id":"n0.9004423309740877"}],"id":"n0.05105476337235659"}},"id":"n0.7857892410042802"}],"id":"n0.9823823266368183"}],"id":"n0.9426897480154197"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.9709926781861866"}],"id":"n0.03734290613225766"}],"shape":{"data":{"p":{"x":165.00999223420212,"y":138.64475386120736},"rotation":0},"anchor":"top","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":false},"de09695600186426634":{"id":"de09695600186426634","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"A","id":"n0.10105608605251493"},{"text":"\\power","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"type":"single","text":"(","id":"n0.3036782427808764"},{"text":"1","id":"n0.3824831423569124"},{"type":"single","text":")","id":"n0.7164747245792866"}],"id":"n0.4003507723055111"}],"id":"n0.6092520108797452"}},"id":"n0.917828489501862"}],"id":"n0.5923251381807864"}],"id":"n0.2679719002001155"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.1431052645670181"}],"id":"n0.013329790590214552"}],"shape":{"data":{"p":{"x":39.15372769390139,"y":80.25616633330793},"rotation":0},"anchor":"right-bottom"},"isTextMode":true,"isInGroup":false},"de6394186712270975":{"id":"de6394186712270975","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"B","id":"n0.23531803753795266"},{"text":"\\power","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"type":"single","text":"(","id":"n0.3725108469804057"},{"text":"1","id":"n0.2891351087921952"},{"type":"single","text":")","id":"n0.4182874552442726"}],"id":"n0.1868351766686256"}],"id":"n0.8372942891879067"}},"id":"n0.4472045414707724"}],"id":"n0.5927288355215281"}],"id":"n0.10668992930477628"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.9964143577823339"}],"id":"n0.05092810527441438"}],"shape":{"data":{"p":{"x":179.41615187290853,"y":72.27128157139109},"rotation":0},"anchor":"bottom-left"},"isTextMode":true,"isInGroup":false},"de9842397275307773":{"id":"de9842397275307773","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"k","id":"n0.004747082055949203"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i,B","id":"n0.5526406792984495"}],"id":"n0.9644148643314918"}],"id":"n0.5307596469129183"}},"id":"n0.02637523419982979"}],"id":"n0.8335422065949525"}],"id":"n0.09762594633122612"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.28113824613284"}],"id":"n0.5143579080076155"}],"shape":{"data":{"p":{"x":410.36525843569154,"y":36.793210041391625},"rotation":0},"anchor":"center","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":false},"de5118218489246686":{"id":"de5118218489246686","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"k","id":"n0.24871722379718642"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i,A","id":"n0.5095246164784026"}],"id":"n0.5379220882487268"}],"id":"n0.9884339528206545"}},"id":"n0.468500102546509"}],"id":"n0.5666590748965379"}],"id":"n0.852513937630931"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.27520156529034834"}],"id":"n0.24525041995584518"}],"shape":{"data":{"p":{"x":315.3033793674201,"y":53.55454646995398},"rotation":0},"anchor":"center","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":false},"de8486284771032058":{"id":"de8486284771032058","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"N","id":"n0.9123006420698565"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.2940758708638598"}],"id":"n0.3181421928780688"}],"id":"n0.4820657229610097"}},"id":"n0.5816105343820541"},{"type":"single","text":"(","id":"n0.648049336185667"},{"text":"k","id":"n0.7403768955476662"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.3777493586191485"}],"id":"n0.39219468819343706"}],"id":"n0.5257824073985311"}},"id":"n0.7774150219838634"},{"type":"single","text":")","id":"n0.4771491292262042"},{"text":"∩A","id":"n0.3889242255573786"},{"text":"\\power","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"type":"single","text":"(","id":"n0.9724094989084517"},{"text":"1","id":"n0.33402206560321"},{"type":"single","text":")","id":"n0.23213465046290982"}],"id":"n0.16437807911242808"}],"id":"n0.7089806366826277"}},"id":"n0.39999800911882843"}],"id":"n0.10899461715937941"}],"id":"n0.9191458927458396"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.556783973303336"}],"id":"n0.9987524274807678"}],"shape":{"data":{"p":{"x":299.97506413421314,"y":133.52269378933406},"rotation":0},"anchor":"top","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":false},"de16254883429353995":{"id":"de16254883429353995","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"N","id":"n0.8170636586706967"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.35345615975435285"}],"id":"n0.9916060380848049"}],"id":"n0.026713923294808817"}},"id":"n0.7366985288988837"},{"type":"single","text":"(","id":"n0.20335654622665356"},{"text":"k","id":"n0.9721878098614687"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.4912595184506434"}],"id":"n0.6468260132310801"}],"id":"n0.3445057274741976"}},"id":"n0.7988091709862892"},{"type":"single","text":")","id":"n0.8203171373458624"},{"text":"∩B","id":"n0.9975570296544802"},{"text":"\\power","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"type":"single","text":"(","id":"n0.35307856265854687"},{"text":"1","id":"n0.352413933908009"},{"type":"single","text":")","id":"n0.13210763108027024"}],"id":"n0.18197707340041536"}],"id":"n0.25738517131728034"}},"id":"n0.9790855459776195"}],"id":"n0.10369469199396919"}],"id":"n0.17313239559906957"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.33618621564809814"}],"id":"n0.1248085148086091"}],"shape":{"data":{"p":{"x":414.23526869371284,"y":136.70141050717115},"rotation":0},"anchor":"top","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":false},"de6767479617198635":{"id":"de6767479617198635","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"A","id":"n0.10897872569406752"},{"text":"\\power","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"type":"single","text":"(","id":"n0.37436275765068205"},{"text":"1","id":"n0.32287002471812487"},{"type":"single","text":")","id":"n0.6926141661798451"}],"id":"n0.7652852684286184"}],"id":"n0.09142653912038101"}},"id":"n0.4452897894647798"}],"id":"n0.6310987228482636"}],"id":"n0.1914030167073173"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.5646550664624987"}],"id":"n0.3267085495491402"}],"shape":{"data":{"p":{"x":290.0456708200787,"y":78.3128229792717},"rotation":0},"anchor":"right-bottom"},"isTextMode":true,"isInGroup":false},"de8474040461236185":{"id":"de8474040461236185","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"B","id":"n0.6701086853566185"},{"text":"\\power","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"type":"single","text":"(","id":"n0.8247541263942839"},{"text":"1","id":"n0.42597757910812395"},{"type":"single","text":")","id":"n0.9956313673431398"}],"id":"n0.5342856772109927"}],"id":"n0.21638813673471446"}},"id":"n0.7088635161368488"}],"id":"n0.7202431739242341"}],"id":"n0.6030035723374039"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.7257025968140056"}],"id":"n0.559233269043351"}],"shape":{"data":{"p":{"x":430.64142833241925,"y":70.32793821735486},"rotation":0},"anchor":"bottom-left"},"isTextMode":true,"isInGroup":false},"de37415865453131847":{"id":"de37415865453131847","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"G","id":"n0.5555080910977648"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"type":"single","text":"(","id":"n0.7667524428607375"},{"id":"n0.7249612225686213","text":"2"},{"type":"single","text":")","id":"n0.21558024603189296"}],"id":"n0.7104242279760211"}],"id":"n0.9867439405843204"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.5376545243450697"}],"id":"n0.4065317308696741"}],"id":"n0.9349420647215545"}},"id":"n0.5225329271799848"}],"id":"n0.8217034161395034"}],"id":"n0.7560492260741587"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.18015053765162192"}],"id":"n0.28196700277592757"}],"shape":{"data":{"p":{"x":355.014275588756,"y":185.8382205513784},"rotation":0},"anchor":"center"},"isTextMode":true,"isInGroup":true},"de4210610368618741":{"id":"de4210610368618741","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"G","id":"n0.5657315341996678"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"type":"single","text":"(","id":"n0.04020898625404978"},{"id":"n0.6749414735294959","text":"2"},{"type":"single","text":")","id":"n0.11232069553011903"}],"id":"n0.8419064978218589"}],"id":"n0.09421278655228216"},"indexValue":{"lines":[{"blocks":[{"text":"i-1","id":"n0.8418682947574898"}],"id":"n0.926137200128913"}],"id":"n0.6019262592866124"}},"id":"n0.812174650459768"}],"id":"n0.2678281197607375"}],"id":"n0.4866589952047484"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.3298376224479682"}],"id":"n0.4451890406534089"}],"shape":{"data":{"p":{"x":101.9476089220893,"y":186.5048872180451},"rotation":0},"anchor":"center"},"isTextMode":true,"isInGroup":true}},"connections":[],"intersections":{"id":"di9833419058199953","items":[],"style":{}},"shapes":[{"id":"dp020182146617273355","type":"circle","data":{"p1":{"x":251.95460119300895,"y":68.16849761225855},"p2":{"x":346.91779549071885,"y":163.13169190996848}},"style":{"strokeColor":"none","fillColor":[74,144,226,0.3]}},{"id":"dp7543482711246636","type":"circle","data":{"p1":{"x":3.0343297438496393,"y":70.41684597664623},"p2":{"x":97.38751402085666,"y":164.77003025365326}},"style":{"strokeColor":"none","fillColor":[74,144,226,0.3]}},{"id":"dp2200883684378665","type":"circle","data":{"p1":{"x":111.17986324949993,"y":63.83807171839557},"p2":{"x":213.04344405689818,"y":165.7016525257938}},"style":{"strokeColor":"none","fillColor":[208,2,27,0.3]}},{"id":"dp6094023916744253","type":"ellipse","data":{"p1":{"x":55.27251519919314,"y":44.692302115273975},"p2":{"x":76.8836906166257,"y":66.30347753270644},"flipX":true},"style":{"thickness":2}},{"id":"dp8083942167164371","type":"ellipse","data":{"p1":{"x":137.98180700724942,"y":90.64001547614504},"p2":{"x":186.24150029914875,"y":138.89970876804435},"rotation":302.75},"style":{"strokeColor":[0,0,0,1],"fillColor":[208,2,27,0.7]}},{"id":"da12106243337436395","data":[{"x":76.8836906166257,"y":55.49788982399021},{"x":149.95594225542263,"y":94}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da945236579494013","data":[{"x":75.79481967809053,"y":60.032357650074715},{"x":138.95594225542263,"y":113.5}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"dp8900102436622708","type":"ellipse","data":{"p1":{"x":32.00627286000403,"y":99.38878909280061},"p2":{"x":68.41557090470226,"y":135.7980871374989},"rotation":280.96},"style":{"strokeColor":[0,0,0,1],"fillColor":[74,144,226,0.7]}},{"id":"da716691451768712","data":[{"x":59.60029172778874,"y":64.24293491715315},{"x":40.814639305438675,"y":101.8952124016048}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da15237384461116066","data":[{"x":66.07810290790941,"y":66.30347753270644},{"x":66.07810290790945,"y":107.72524246371344}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"dp15132352280037464","type":"ellipse","data":{"p1":{"x":399.5596707269753,"y":25.9876223326754},"p2":{"x":421.17084614440785,"y":47.59879775010785},"flipX":true},"style":{"thickness":2}},{"id":"dp6508540693367029","type":"ellipse","data":{"p1":{"x":360.4051397090107,"y":61.89472836435935},"p2":{"x":462.2687205164089,"y":163.7583091717576}},"style":{"strokeColor":"none","fillColor":[208,2,27,0.3]}},{"id":"dp2749280428686842","type":"ellipse","data":{"p1":{"x":304.4977916587038,"y":42.74895876123776},"p2":{"x":326.10896707613637,"y":64.36013417867021},"flipX":true},"style":{"thickness":2}},{"id":"dp749858683454439","type":"circle","data":{"p1":{"x":387.20708346676014,"y":88.6966721221088},"p2":{"x":435.4667767586595,"y":136.95636541400816},"rotation":302.75},"style":{"strokeColor":[0,0,0,1],"fillColor":[208,2,27,0.7]}},{"id":"dp5141238542472601","type":"ellipse","data":{"p1":{"x":281.2315493195147,"y":97.4454457387643},"p2":{"x":317.64084736421313,"y":133.8547437834627},"rotation":280.96},"style":{"strokeColor":[0,0,0,1],"fillColor":[74,144,226,0.7]}},{"id":"da04266324197083948","data":[{"x":414.7701700381738,"y":47.22248604138599},{"x":424.3905611461932,"y":92.53237636196678}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da9467754937536541","data":[{"x":407.77413396364335,"y":47.61115471219324},{"x":402.20321634873955,"y":91.14204584260443}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da5927144806051112","data":[{"x":231.33499396372815,"y":6.833333333333343},{"x":231.33499396372815,"y":205.05435544502723}],"head":"no","tail":"no","shaft":"--","mVer":1,"style":{"thickness":2,"strokeColor":[155,155,155,1]}},{"id":"da546079785935311","data":[{"x":308.6214950324766,"y":62.68826023392418},{"x":289.8358426101265,"y":100.34053771837586}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da9384475105415515","data":[{"x":315.09930621259724,"y":64.74880284947747},{"x":315.0993062125973,"y":106.17056778048448}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da9607304531393006","data":[{"x":50.41190328058954,"y":93.17849563142369},{"x":60.45594225542263,"y":95.25}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":1}},{"id":"da5962364382388641","data":[{"x":129.95594225542263,"y":100.25},{"x":136.83402588923735,"y":90.7351522773875}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":1}},{"id":"da38607824571713856","data":[{"x":407.80246228662514,"y":80.51843550720642},{"x":421.0819752058727,"y":80.51843550720648}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":1}},{"id":"da8823690661281964","data":[{"x":299.4119032805895,"y":91.67849563142369},{"x":309.4559422554226,"y":93.75}],"head":"no","tail":"no","shaft":".","mVer":1,"style":{"thickness":1}},{"id":"dg17329104203843237","entities":[{"id":"dp5388657121115188","type":"doc-rounded-rect","data":{"p1":{"x":82.8226089220893,"y":171.54999999999998},"p2":{"x":121.0726089220893,"y":201.45977443609024}},"style":{"fillColor":[155,155,155,0.5]}},{"id":"dl2658525448653106","linkedId":"de4210610368618741"}]},{"id":"dg5901661342517579","entities":[{"id":"dp24485861403204945","type":"doc-rounded-rect","data":{"p1":{"x":335.889275588756,"y":170.8833333333333},"p2":{"x":374.139275588756,"y":200.79310776942353}},"style":{"fillColor":[155,155,155,0.5]}},{"id":"dl3461675574728129","linkedId":"de37415865453131847"}]}],"settings":{"grid":true,"diagramHeight":229.99479166666669}}]},{"id":"n0.4366202696179722","blocks":[],"style":null}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":717,"delayRenderCache":{"av":717,"map":{}}}

==> figs/docs/c7eb67ba-3996-4cd1-bd46-fb99aa4bdd90 <==
{"id":"r0.17747056039859443","lines":[{"blocks":[{"text":"\\diagram","type":"composite","elements":{"de3377854219142531":{"id":"de3377854219142531","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1","id":"n0.20952465146543853"}],"id":"n0.9162883025846424"}],"id":"n0.8322322416351335"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.04158868883930644"}],"id":"n0.775966655952385"}],"shape":{"data":{"p":{"x":461.439691943128,"y":156.09755134281215}},"anchor":"center"},"isTextMode":true,"isInGroup":true},"de9746836771703111":{"id":"de9746836771703111","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"2","id":"n0.6725943536422154"}],"id":"n0.5453296925648721"}],"id":"n0.9360481125987847"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.6675805816719198"}],"id":"n0.5888478550929215"}],"shape":{"data":{"p":{"x":536.439691943128,"y":40.59755134281215}},"anchor":"center"},"isTextMode":true,"isInGroup":true},"de7058376200954342":{"id":"de7058376200954342","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"3","id":"n0.3763561677202072"}],"id":"n0.915228141781457"}],"id":"n0.2759046315721758"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.4354812817585856"}],"id":"n0.2586901690293375"}],"shape":{"data":{"p":{"x":498.939691943128,"y":86.59755134281215}},"anchor":"center"},"isTextMode":true,"isInGroup":true},"de10690752715792029":{"id":"de10690752715792029","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"4","id":"n0.5064971060126788"}],"id":"n0.7947793048343104"}],"id":"n0.04101529746683186"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.7609053867699918"}],"id":"n0.25189572981811614"}],"shape":{"data":{"p":{"x":585.939691943128,"y":92.09755134281215}},"anchor":"center"},"isTextMode":true,"isInGroup":true},"de3042818168372794":{"id":"de3042818168372794","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"5","id":"n0.1505059768410395"}],"id":"n0.7605044414738868"}],"id":"n0.5594517491111686"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.24886184289993873"}],"id":"n0.8228918770983051"}],"shape":{"data":{"p":{"x":623.939691943128,"y":175.09755134281215}},"anchor":"center"},"isTextMode":true,"isInGroup":true},"de0849863605010528":{"id":"de0849863605010528","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"6","id":"n0.286815049606415"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"A","id":"n0.8104026477860262"}],"id":"n0.34286633604209826"}],"id":"n0.1081116810053373"}},"id":"n0.7597495991491978"}],"id":"n0.8433199361639947"}],"id":"n0.4207383981714343"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.9721161446261062"}],"id":"n0.55504990997464"}],"shape":{"data":{"p":{"x":520.439691943128,"y":182.4308846761455}},"anchor":"center","settings":{"fontSize":"\\small"}},"isTextMode":true,"isInGroup":true},"de061258972971343084":{"id":"de061258972971343084","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"7","style":{"mathModeType":null},"id":"n0.26217896376955374"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"A","id":"n0.6567327821772031"}],"id":"n0.6354559085544738"}],"id":"n0.42272965914634875"}},"style":{"mathModeType":null},"id":"n0.4229967908172001"}],"id":"n0.4983296770464174"}],"id":"n0.9803073299961937"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.334197022447017"}],"id":"n0.7675509951203241"}],"shape":{"data":{"p":{"x":520.9396919431281,"y":239.59755134281215}},"anchor":"center","settings":{"fontSize":"\\footnotesize"}},"isTextMode":true,"isInGroup":true},"de5679455674005585":{"id":"de5679455674005585","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"8","id":"n0.5459720018394416"}],"id":"n0.12275639960395579"}],"id":"n0.2653231431110712"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.08910921696079144"}],"id":"n0.8212658796068881"}],"shape":{"data":{"p":{"x":447.439691943128,"y":240.59755134281215}},"anchor":"center"},"isTextMode":true,"isInGroup":true},"de9216647693979059":{"id":"de9216647693979059","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"A","id":"n0.6968540353379695"},{"text":"\\power","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"type":"single","text":"(","id":"n0.9526208896117205"},{"text":"1","id":"n0.5256367509441366"},{"type":"single","text":")","id":"n0.822190243383168"}],"id":"n0.7151019442752578"}],"id":"n0.31487670072252505"}},"id":"n0.4075656582873286"}],"id":"n0.6080271311020071"}],"id":"n0.1843105391000388"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.7852421391520006"}],"id":"n0.29216369095973405"}],"shape":{"data":{"p":{"x":427.06030805687203,"y":83}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de5471652702069676":{"id":"de5471652702069676","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"B","id":"n0.3080626350980227"},{"text":"\\power","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"type":"single","text":"(","id":"n0.7670030927193696"},{"text":"1","id":"n0.8077326120523634"},{"type":"single","text":")","id":"n0.6052110867801184"}],"id":"n0.1468087964420124"}],"id":"n0.7662168123584401"}},"id":"n0.6753106294683315"}],"id":"n0.11511397327640682"}],"id":"n0.19431024796945784"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.5813443325835683"}],"id":"n0.7904664795805318"}],"shape":{"data":{"p":{"x":621.060308056872,"y":83}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de6254772879152124":{"id":"de6254772879152124","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"6","id":"n0.023711365578485077"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"B","id":"n0.5331817373012933"}],"id":"n0.46521008222348925"}],"id":"n0.1594258359232663"}},"id":"n0.39060775062372155"}],"id":"n0.2122393044306703"}],"id":"n0.7804586377015408"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.4577994964407881"}],"id":"n0.6487873890015221"}],"shape":{"data":{"p":{"x":565.1063586097947,"y":150.43088467614547}},"anchor":"center","settings":{"fontSize":"\\small"}},"isTextMode":true,"isInGroup":true},"de7724690333940571":{"id":"de7724690333940571","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"7","style":{"mathModeType":null},"id":"n0.9016222905760021"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"B","id":"n0.59938779954544"}],"id":"n0.6673321228914517"}],"id":"n0.725247685824693"}},"style":{"mathModeType":null},"id":"n0.3651709565939816"}],"id":"n0.013164248764108377"}],"id":"n0.2190150498428427"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.6605461325206448"}],"id":"n0.9544084544114038"}],"shape":{"data":{"p":{"x":574.939691943128,"y":245}},"anchor":"center","settings":{"fontSize":"\\footnotesize"}},"isTextMode":true,"isInGroup":true},"de5735043202187369":{"id":"de5735043202187369","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1","id":"n0.9179620968290698"}],"id":"n0.6261379759014449"}],"id":"n0.07519964592468176"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.21635526624147983"}],"id":"n0.14056766399775467"}],"shape":{"data":{"p":{"x":86.84340801102576,"y":155}},"anchor":"center"},"isTextMode":true,"isInGroup":true},"de5118042979405351":{"id":"de5118042979405351","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"2","id":"n0.5781562927244739"}],"id":"n0.43505106523282233"}],"id":"n0.3529414688376722"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.5191851490755326"}],"id":"n0.9313529957403774"}],"shape":{"data":{"p":{"x":161.34779189728175,"y":38.59755134281215}},"anchor":"center"},"isTextMode":true,"isInGroup":true},"de1323254760299537":{"id":"de1323254760299537","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"3","id":"n0.3302446892751618"}],"id":"n0.337554803377178"}],"id":"n0.8091219429653289"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.30788693931118494"}],"id":"n0.9518580969298129"}],"shape":{"data":{"p":{"x":124.84340801102576,"y":86}},"anchor":"center"},"isTextMode":true,"isInGroup":true},"de9019134361407426":{"id":"de9019134361407426","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"4","id":"n0.5313448055061378"}],"id":"n0.9541916804062807"}],"id":"n0.22170749516634136"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.42813058249456337"}],"id":"n0.8307947525590327"}],"shape":{"data":{"p":{"x":210.89340801102577,"y":90.5}},"anchor":"center"},"isTextMode":true,"isInGroup":true},"de31837363099354143":{"id":"de31837363099354143","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"5","id":"n0.3681396129708867"}],"id":"n0.9511641831771369"}],"id":"n0.5171143008062127"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.88264949196956"}],"id":"n0.9199815458106326"}],"shape":{"data":{"p":{"x":249.34340801102576,"y":174}},"anchor":"center"},"isTextMode":true,"isInGroup":true},"de03212568133696059":{"id":"de03212568133696059","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"6","id":"n0.32323567233322237"}],"id":"n0.41238615693513125"}],"id":"n0.26294928439353105"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.030666491532091333"}],"id":"n0.9324512082318657"}],"shape":{"data":{"p":{"x":163.34340801102576,"y":189.5}},"anchor":"center"},"isTextMode":true,"isInGroup":true},"de7463208319227395":{"id":"de7463208319227395","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"7","id":"n0.2966938775944694"}],"id":"n0.24413414078116746"}],"id":"n0.568144070440066"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.8433166113350101"}],"id":"n0.10304157293779048"}],"shape":{"data":{"p":{"x":163.84340801102576,"y":256.5}},"anchor":"center"},"isTextMode":true,"isInGroup":true},"de7875117653412074":{"id":"de7875117653412074","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"8","id":"n0.1729493000411202"}],"id":"n0.8954701214590113"}],"id":"n0.6324528942712546"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.4717552941606249"}],"id":"n0.09822019936112003"}],"shape":{"data":{"p":{"x":72.84340801102576,"y":239.5}},"anchor":"center"},"isTextMode":true,"isInGroup":true},"de8836686111401333":{"id":"de8836686111401333","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"A","id":"n0.018818902407259586"}],"id":"n0.7865648067852653"}],"id":"n0.9133234192903064"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.27617769228592226"}],"id":"n0.3699356251314241"}],"shape":{"data":{"p":{"x":48.96840801102576,"y":99}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de4944384494771481":{"id":"de4944384494771481","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"B","id":"n0.6532953675957476"}],"id":"n0.4625621511954805"}],"id":"n0.4991671660048349"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.09634006816969998"}],"id":"n0.366846827108551"}],"shape":{"data":{"p":{"x":256.96840801102576,"y":99}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de7522201713643537":{"id":"de7522201713643537","lines":[{"id":"n0.5552497745207199","blocks":[{"id":"n0.7125118688768921","text":"Phase I"}]}],"shape":{"data":{"p":{"x":306,"y":144}},"anchor":"left-top"},"isTextMode":true},"de7143053624396765":{"id":"de7143053624396765","lines":[{"id":"n0.6139156665990124","blocks":[{"id":"n0.9153069567198613","text":"Phase II"}]}],"shape":{"data":{"p":{"x":546,"y":302}},"anchor":"left-top"},"isTextMode":true},"de8638865150933372":{"id":"de8638865150933372","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1","id":"n0.2304478822188023"}],"id":"n0.04426400973609379"}],"id":"n0.41868035240072277"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.032404352070149356"}],"id":"n0.7272050200539182"}],"shape":{"data":{"p":{"x":461.4396919431281,"y":507.59755134281215}},"anchor":"center"},"isTextMode":true,"isInGroup":true},"de2908296551539664":{"id":"de2908296551539664","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"2","id":"n0.8436778975139834"}],"id":"n0.5062938118871998"}],"id":"n0.7902869713564857"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.3443772885466274"}],"id":"n0.6899500055478316"}],"shape":{"data":{"p":{"x":536.4396919431281,"y":392.09755134281215}},"anchor":"center"},"isTextMode":true,"isInGroup":true},"de04805762837656724":{"id":"de04805762837656724","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"3","id":"n0.01985509317603973"}],"id":"n0.47548030688261234"}],"id":"n0.7958066123936742"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.9788810352752293"}],"id":"n0.017514611284747295"}],"shape":{"data":{"p":{"x":498.9396919431281,"y":438.09755134281215}},"anchor":"center"},"isTextMode":true,"isInGroup":true},"de588362433308294":{"id":"de588362433308294","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"4","id":"n0.11521751789521595"}],"id":"n0.8068761824279547"}],"id":"n0.7943104620318107"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.03778374775118487"}],"id":"n0.6067744911091486"}],"shape":{"data":{"p":{"x":585.9396919431281,"y":443.59755134281215}},"anchor":"center"},"isTextMode":true,"isInGroup":true},"de45201336284664273":{"id":"de45201336284664273","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"5","id":"n0.3453444170073732"}],"id":"n0.9076220042944334"}],"id":"n0.2953112105174991"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.6506664777737994"}],"id":"n0.1729750341109395"}],"shape":{"data":{"p":{"x":623.9396919431281,"y":526.5975513428122}},"anchor":"center"},"isTextMode":true,"isInGroup":true},"de5435926234374486":{"id":"de5435926234374486","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"6","id":"n0.14478382581469118"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"A","id":"n0.8964087176649529"}],"id":"n0.2669599578850552"}],"id":"n0.6373453149666857"}},"id":"n0.6498574169323832"}],"id":"n0.24910661416778046"}],"id":"n0.901836454531697"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.175350899793705"}],"id":"n0.5194160112971289"}],"shape":{"data":{"p":{"x":520.4396919431281,"y":533.9308846761455}},"anchor":"center","settings":{"fontSize":"\\small"}},"isTextMode":true,"isInGroup":true},"de03143524405385634":{"id":"de03143524405385634","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"7","style":{"mathModeType":null},"id":"n0.18042388123230002"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"A","id":"n0.3864056626187198"}],"id":"n0.16591281925348822"}],"id":"n0.1989553545074667"}},"style":{"mathModeType":null},"id":"n0.47601072723982574"}],"id":"n0.9305954844753488"}],"id":"n0.9709535164010152"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.3884518695312391"}],"id":"n0.8167566410107219"}],"shape":{"data":{"p":{"x":520.9396919431281,"y":591.0975513428122}},"anchor":"center","settings":{"fontSize":"\\footnotesize"}},"isTextMode":true,"isInGroup":true},"de0859208809459453":{"id":"de0859208809459453","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"8","id":"n0.8425649489852385"}],"id":"n0.8747559896812491"}],"id":"n0.27982953930171917"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.06972879615768757"}],"id":"n0.823322715583769"}],"shape":{"data":{"p":{"x":447.4396919431281,"y":592.0975513428122}},"anchor":"center"},"isTextMode":true,"isInGroup":true},"de030069601839159077":{"id":"de030069601839159077","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"A","id":"n0.8937062985994373"},{"text":"\\power","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"type":"single","text":"(","id":"n0.1053796168847112"},{"text":"1","id":"n0.0570578454914481"},{"type":"single","text":")","id":"n0.18068638170373008"}],"id":"n0.5798065311755827"}],"id":"n0.7460415385786243"}},"id":"n0.968408069509237"}],"id":"n0.6937144560346564"}],"id":"n0.8001050402769898"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.8533703867336693"}],"id":"n0.12339294385208999"}],"shape":{"data":{"p":{"x":427.0603080568721,"y":434.5}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de32525387455748045":{"id":"de32525387455748045","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"B","id":"n0.9224096933433117"},{"text":"\\power","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"type":"single","text":"(","id":"n0.3638011590834298"},{"text":"1","id":"n0.12245256910558"},{"type":"single","text":")","id":"n0.859316052242213"}],"id":"n0.7064168976847944"}],"id":"n0.053753422066397105"}},"id":"n0.8574481282267556"}],"id":"n0.39256242842442357"}],"id":"n0.7085737039342996"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.6431041312061934"}],"id":"n0.9465305672651279"}],"shape":{"data":{"p":{"x":621.0603080568721,"y":434.5}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de3192619109950017":{"id":"de3192619109950017","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"6","id":"n0.10401890861885432"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"B","id":"n0.5511216871680724"}],"id":"n0.39755970457511314"}],"id":"n0.649194515721081"}},"id":"n0.37388418761820663"}],"id":"n0.39545430250740776"}],"id":"n0.9585816636375117"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.9717818985793591"}],"id":"n0.9595628939692227"}],"shape":{"data":{"p":{"x":565.1063586097948,"y":501.93088467614547}},"anchor":"center","settings":{"fontSize":"\\small"}},"isTextMode":true,"isInGroup":true},"de7184182056565798":{"id":"de7184182056565798","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"7","style":{"mathModeType":null},"id":"n0.3304181970856461"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"B","id":"n0.4991326505810545"}],"id":"n0.27780975112023243"}],"id":"n0.65903551151714"}},"style":{"mathModeType":null},"id":"n0.398577523493425"}],"id":"n0.5936004693672767"}],"id":"n0.5722055898576626"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.16472627950430185"}],"id":"n0.42379031524303246"}],"shape":{"data":{"p":{"x":574.9396919431281,"y":596.5}},"anchor":"center","settings":{"fontSize":"\\footnotesize"}},"isTextMode":true,"isInGroup":true},"de3411185373599821":{"id":"de3411185373599821","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"3","id":"n0.18552095712921757"},{"id":"n0.9744910181463171","text":"\\power","type":"composite","elements":{"powerValue":{"id":"n0.7370400504491526","lines":[{"id":"n0.8150196771377232","blocks":[{"id":"n0.8752841275717838","text":"c"}]}]}}}],"id":"n0.7056646451971527"}],"id":"n0.22194369278666315"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.6139354786675673"}],"id":"n0.771505996807871"}],"shape":{"data":{"p":{"x":610.4396919431281,"y":399.09755134281215}},"anchor":"center"},"isTextMode":true,"isInGroup":true},"de5839989731199371":{"id":"de5839989731199371","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.67654576287134","text":"4"},{"id":"n0.6772584695395591","text":"\\power","type":"composite","elements":{"powerValue":{"id":"n0.4158579561536837","lines":[{"id":"n0.7271822082067987","blocks":[{"id":"n0.9071898105169758","text":"c"}]}]}}}],"id":"n0.9639499277417489"}],"id":"n0.02385881263484646"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.8515393925498842"}],"id":"n0.16006409708002445"}],"shape":{"data":{"p":{"x":413.9396919431281,"y":524.5975513428122}},"anchor":"center"},"isTextMode":true,"isInGroup":true},"de6695614353438804":{"id":"de6695614353438804","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.47546496674493754","text":"5"},{"id":"n0.9262568774875144","text":"\\power","type":"composite","elements":{"powerValue":{"id":"n0.40661702488691254","lines":[{"id":"n0.4727123957214405","blocks":[{"id":"n0.8504935561973226","text":"c"}]}]}}}],"id":"n0.8456082728666208"}],"id":"n0.9133874302307556"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.7224550886762942"}],"id":"n0.07751689371806791"}],"shape":{"data":{"p":{"x":408.4396919431281,"y":558.5975513428122}},"anchor":"center"},"isTextMode":true,"isInGroup":true},"de17654312581252363":{"id":"de17654312581252363","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.9943674777831959","text":"1"},{"id":"n0.400070697068706","text":"\\power","type":"composite","elements":{"powerValue":{"id":"n0.2588392151411858","lines":[{"id":"n0.13881790993355803","blocks":[{"id":"n0.73681234662649","text":"c"}]}]}}}],"id":"n0.657266153003347"}],"id":"n0.3409870705879501"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.11785791867423145"}],"id":"n0.5108538622270611"}],"shape":{"data":{"p":{"x":635.9396919431281,"y":585.0975513428122}},"anchor":"center"},"isTextMode":true,"isInGroup":true},"de38975756146330953":{"id":"de38975756146330953","lines":[{"blocks":[{"text":"Phase III","id":"n0.5513101329743912"}],"id":"n0.5431031738799379"}],"shape":{"data":{"p":{"x":312.6666666666667,"y":473.3333333333333}},"anchor":"left-top"},"isTextMode":true},"de6144653206198403":{"id":"de6144653206198403","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1","id":"n0.13051148705082172"}],"id":"n0.8667253903161429"}],"id":"n0.3183356141499538"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.3178504545960952"}],"id":"n0.8681082567718714"}],"shape":{"data":{"p":{"x":81.49999999999997,"y":507.59755134281215}},"anchor":"center"},"isTextMode":true,"isInGroup":false},"de7801764873351877":{"id":"de7801764873351877","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"2","id":"n0.31206997145678983"},{"id":"n0.04270633935604384","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.0806826939122518","lines":[{"id":"n0.29980401087715336","blocks":[{"id":"n0.849508860708287","text":"A"}]}]}}}],"id":"n0.29589429103566567"}],"id":"n0.687877977391824"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.885530960318951"}],"id":"n0.4669500762262151"}],"shape":{"data":{"p":{"x":130.99999999999997,"y":383.59755134281215}},"anchor":"center","settings":{"fontSize":"\\footnotesize"}},"isTextMode":true,"isInGroup":false},"de005214853040938827":{"id":"de005214853040938827","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"3","id":"n0.29802927264439827"}],"id":"n0.5397107224918691"}],"id":"n0.4734682735662139"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.8302447980201604"}],"id":"n0.20247585997817108"}],"shape":{"data":{"p":{"x":118.99999999999997,"y":438.09755134281215}},"anchor":"center"},"isTextMode":true,"isInGroup":false},"de47239681985771953":{"id":"de47239681985771953","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"4","id":"n0.6946040210354658"}],"id":"n0.3260086719124393"}],"id":"n0.13916382240961833"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.5965667853266854"}],"id":"n0.41141257541798626"}],"shape":{"data":{"p":{"x":205.99999999999997,"y":443.59755134281215}},"anchor":"center"},"isTextMode":true,"isInGroup":false},"de004790600627458508":{"id":"de004790600627458508","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"5","id":"n0.3162488200357605"}],"id":"n0.5396609304907412"}],"id":"n0.9891443438434935"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.494122747974473"}],"id":"n0.08858175106307997"}],"shape":{"data":{"p":{"x":243.99999999999997,"y":526.5975513428122}},"anchor":"center"},"isTextMode":true,"isInGroup":false},"de2674578715507969":{"id":"de2674578715507969","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"6","id":"n0.8580587996489675"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"A","id":"n0.9180135160634177"}],"id":"n0.854838752073297"}],"id":"n0.9071630062236693"}},"id":"n0.3371001956370727"}],"id":"n0.6076653108070631"}],"id":"n0.8421387795056607"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.07885042960368027"}],"id":"n0.14605509063834576"}],"shape":{"data":{"p":{"x":140.49999999999991,"y":533.9308846761455}},"anchor":"center","settings":{"fontSize":"\\small"}},"isTextMode":true,"isInGroup":false},"de7232834084003468":{"id":"de7232834084003468","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"7","style":{"mathModeType":null},"id":"n0.5009250496842463"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"A","id":"n0.38871985661947983"}],"id":"n0.9825683703224966"}],"id":"n0.6041141760902848"}},"style":{"mathModeType":null},"id":"n0.2378705919231754"}],"id":"n0.6397283222121062"}],"id":"n0.3890022024093027"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.42755671457532185"}],"id":"n0.0003224680928881618"}],"shape":{"data":{"p":{"x":140.99999999999991,"y":591.0975513428122}},"anchor":"center","settings":{"fontSize":"\\footnotesize"}},"isTextMode":true,"isInGroup":false},"de12591002761265258":{"id":"de12591002761265258","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"8","id":"n0.6457211189497869"}],"id":"n0.41904008659164904"}],"id":"n0.521027480909916"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.3768445916296961"}],"id":"n0.485436272514691"}],"shape":{"data":{"p":{"x":67.49999999999997,"y":592.0975513428122}},"anchor":"center"},"isTextMode":true,"isInGroup":false},"de07560688735986654":{"id":"de07560688735986654","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"A","id":"n0.9194087821781627"},{"text":"\\power","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"type":"single","text":"(","id":"n0.5227018207232317"},{"text":"1","id":"n0.48687917369663425"},{"type":"single","text":")","id":"n0.6125158544864331"}],"id":"n0.5377078549036234"}],"id":"n0.7479151087422469"}},"id":"n0.7027366048708006"}],"id":"n0.36046469444330875"}],"id":"n0.9734655723816286"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.21321804258201027"}],"id":"n0.7959609052122747"}],"shape":{"data":{"p":{"x":47.12061611374398,"y":434.5}},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de8643274224119519":{"id":"de8643274224119519","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"B","id":"n0.5431289306770606"},{"text":"\\power","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"type":"single","text":"(","id":"n0.3211078559228877"},{"text":"1","id":"n0.19025502679025386"},{"type":"single","text":")","id":"n0.4846315526237035"}],"id":"n0.38824834663004637"}],"id":"n0.347841295633325"}},"id":"n0.3195185082982006"}],"id":"n0.8582264978157335"}],"id":"n0.8323956210769854"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.34565297834327935"}],"id":"n0.4432847481512767"}],"shape":{"data":{"p":{"x":241.12061611374403,"y":434.5}},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de32465357939223893":{"id":"de32465357939223893","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"6","id":"n0.6152433197825131"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"B","id":"n0.9322023330564078"}],"id":"n0.3490018088858158"}],"id":"n0.7973443846612458"}},"id":"n0.7009261711238663"}],"id":"n0.338608916966155"}],"id":"n0.8824992199297255"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.04530796262676584"}],"id":"n0.7050129613089307"}],"shape":{"data":{"p":{"x":185.1666666666667,"y":501.9308846761455}},"anchor":"center","settings":{"fontSize":"\\small"}},"isTextMode":true,"isInGroup":false},"de3070133629969003":{"id":"de3070133629969003","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"7","style":{"mathModeType":null},"id":"n0.05915943120960754"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"B","id":"n0.3598006307947079"}],"id":"n0.057562427645660774"}],"id":"n0.2763151024031658"}},"style":{"mathModeType":null},"id":"n0.9279539157137373"}],"id":"n0.9919536259761554"}],"id":"n0.38870435393783653"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.9616996535390936"}],"id":"n0.9151690602213602"}],"shape":{"data":{"p":{"x":194.99999999999997,"y":596.5}},"anchor":"center","settings":{"fontSize":"\\footnotesize"}},"isTextMode":true,"isInGroup":false},"de9991493086784236":{"id":"de9991493086784236","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"3","id":"n0.9507178809702879"},{"id":"n0.8856189379337576","text":"\\power","type":"composite","elements":{"powerValue":{"id":"n0.13468391900124765","lines":[{"id":"n0.49874743790269394","blocks":[{"id":"n0.9000944611933208","text":"c"}]}]}}}],"id":"n0.6457316797664621"}],"id":"n0.5794206571160199"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.8497989068677123"}],"id":"n0.9638126769073805"}],"shape":{"data":{"p":{"x":230.49999999999997,"y":399.09755134281215}},"anchor":"center"},"isTextMode":true,"isInGroup":false},"de505123160837305":{"id":"de505123160837305","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"4","id":"n0.5143920104505402"},{"id":"n0.7172267202056917","text":"\\power","type":"composite","elements":{"powerValue":{"id":"n0.3859980241102938","lines":[{"id":"n0.7520765167511398","blocks":[{"id":"n0.5280572274725561","text":"c"}]}]}}}],"id":"n0.14624105398909215"}],"id":"n0.9240658629296086"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.8329360619039907"}],"id":"n0.7242426280048679"}],"shape":{"data":{"p":{"x":33.99999999999997,"y":524.5975513428122}},"anchor":"center"},"isTextMode":true,"isInGroup":false},"de46759224366520025":{"id":"de46759224366520025","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"5","id":"n0.9426435995770697"},{"id":"n0.9422329265048683","text":"\\power","type":"composite","elements":{"powerValue":{"id":"n0.8660642971230104","lines":[{"id":"n0.3310335242399851","blocks":[{"id":"n0.22971630250879116","text":"c"}]}]}}}],"id":"n0.8498271822736867"}],"id":"n0.2962348922324758"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.16579421989717047"}],"id":"n0.2764398042991383"}],"shape":{"data":{"p":{"x":28.49999999999997,"y":558.0975513428122}},"anchor":"center"},"isTextMode":true,"isInGroup":false},"de008460158864032286":{"id":"de008460158864032286","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1","id":"n0.6373706111679747"},{"id":"n0.3893480616106977","text":"\\power","type":"composite","elements":{"powerValue":{"id":"n0.7399973411167047","lines":[{"id":"n0.058348275814988027","blocks":[{"id":"n0.9332623485566802","text":"c"}]}]}}}],"id":"n0.08885972025422428"}],"id":"n0.9280146770311053"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.3905452009483139"}],"id":"n0.19263014161135894"}],"shape":{"data":{"p":{"x":256,"y":585.0975513428122}},"anchor":"center"},"isTextMode":true,"isInGroup":false},"de36945179916452653":{"id":"de36945179916452653","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"2","id":"n0.4426386204838082"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.6601691946943626","text":"B"}],"id":"n0.8741041961688738"}],"id":"n0.44487811483201556"}},"id":"n0.22511830603265315"}],"id":"n0.5730628791598209"}],"id":"n0.6572493330246403"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.7813115059131732"}],"id":"n0.5005380289816999"}],"shape":{"data":{"p":{"x":168.49999999999997,"y":383.09755134281215}},"anchor":"center","settings":{"fontSize":"\\footnotesize"}},"isTextMode":true,"isInGroup":false}},"connections":[],"intersections":{"id":"di3676895024823952","items":[],"style":{}},"shapes":[{"id":"dg234635500507129","entities":[{"id":"ds24606337808294532","type":"polygon-curve","data":[{"p1":{"x":185.3017413443591,"y":74},"p2":{"x":249.96840801102576,"y":120},"cp":{"dx":21.333333333333314,"dy":-29.333333333333343},"cp2":{"dx":-20,"dy":-39.33333333333334}},{"p1":{"x":249.96840801102576,"y":120},"p2":{"x":245.30174134435907,"y":226.66666666666666},"cp":{"dx":20,"dy":39.33333333333334},"cp2":{"dx":42,"dy":-30}},{"p1":{"x":245.30174134435907,"y":226.66666666666666},"p2":{"x":141.96840801102576,"y":268.6666666666667},"cp":{"dx":-42,"dy":29.99999999999997},"cp2":{"dx":39.33333333333334,"dy":37.333333333333314}},{"p1":{"x":141.96840801102576,"y":268.6666666666667},"p2":{"x":185.3017413443591,"y":74},"cp":{"dx":-39.33333333333334,"dy":-37.333333333333314},"cp2":{"dx":-21.333333333333314,"dy":29.333333333333343}}],"style":{"strokeColor":"none","fillColor":[208,2,27,0.3]}},{"id":"ds17553065891201025","type":"polygon-curve","data":[{"p1":{"x":113.3017413443591,"y":64.66666666666667},"p2":{"x":173.96840801102576,"y":120.66666666666666},"cp":{"dx":32.00000000000003,"dy":-8.666666666666657},"cp2":{"dx":-8,"dy":-26.666666666666657}},{"p1":{"x":173.96840801102576,"y":120.66666666666666},"p2":{"x":187.3017413443591,"y":261.3333333333333},"cp":{"dx":8,"dy":26.666666666666657},"cp2":{"dx":14,"dy":-35.33333333333337}},{"p1":{"x":187.3017413443591,"y":261.3333333333333},"p2":{"x":52.968408011025744,"y":251.33333333333334},"cp":{"dx":-14,"dy":35.33333333333337},"cp2":{"dx":26.999999999999986,"dy":30.00000000000003}},{"p1":{"x":52.968408011025744,"y":251.33333333333334},"p2":{"x":113.3017413443591,"y":64.66666666666667},"cp":{"dx":-26.999999999999993,"dy":-30.00000000000003},"cp2":{"dx":-32.000000000000014,"dy":8.666666666666657}}],"style":{"fillColor":[74,144,226,0.3],"strokeColor":"none"}},{"id":"dp25394026333312114","type":"circle","data":{"p1":{"x":150.22717578353772,"y":27.476935229068133},"p2":{"x":172.46840801102576,"y":49.71816745655617},"flipX":true},"style":{"thickness":2}},{"id":"dp9831182464263055","type":"circle","data":{"p1":{"x":112.72717578353772,"y":73.47693522906813},"p2":{"x":134.96840801102576,"y":95.71816745655617},"flipX":true},"style":{"thickness":2}},{"id":"da8135694763219745","data":[{"x":153.46840801102576,"y":46},{"x":130.96840801102576,"y":75.5}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"dp023948809965321338","type":"circle","data":{"p1":{"x":199.72717578353772,"y":78.97693522906813},"p2":{"x":221.96840801102576,"y":101.21816745655617},"flipX":true},"style":{"thickness":2}},{"id":"da5056238579990056","data":[{"x":171.21840801102576,"y":44.5},{"x":204.71840801102576,"y":80.5}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da13416774805500742","data":[{"x":134.96840801102576,"y":84.59755134281215},{"x":199.72717578353775,"y":90.09755134281215}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"dp05084200863333255","type":"circle","data":{"p1":{"x":75.22717578353772,"y":142.97693522906815},"p2":{"x":97.46840801102576,"y":165.21816745655616},"flipX":true},"style":{"thickness":2}},{"id":"dp8607335030141765","type":"circle","data":{"p1":{"x":237.72717578353772,"y":161.97693522906815},"p2":{"x":259.96840801102576,"y":184.21816745655616},"flipX":true},"style":{"thickness":2}},{"id":"da015475132816799686","data":[{"x":91.21840801102576,"y":143.75},{"x":119.21840801102576,"y":95.25}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da6341423382844156","data":[{"x":217.21840801102576,"y":98.75},{"x":245.71840801102576,"y":162.25}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"dp7273147234520221","type":"circle","data":{"p1":{"x":152.22717578353772,"y":177.97693522906815},"p2":{"x":174.46840801102576,"y":200.21816745655616},"flipX":true},"style":{"thickness":2}},{"id":"da8807420698543149","data":[{"x":96.21840801102576,"y":158.25},{"x":152.22717578353775,"y":189.09755134281215}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da9193276986773158","data":[{"x":239.21840801102576,"y":178.75},{"x":174.46840801102576,"y":189.09755134281215}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da12630476544433056","data":[{"x":205.71840801102576,"y":100.5},{"x":167.21840801102576,"y":178}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"dp5495920515367643","type":"circle","data":{"p1":{"x":61.22717578353772,"y":227.47693522906815},"p2":{"x":83.46840801102576,"y":249.71816745655616},"flipX":true},"style":{"thickness":2}},{"id":"dp39942333598332236","type":"circle","data":{"p1":{"x":151.72717578353772,"y":244.47693522906815},"p2":{"x":173.96840801102576,"y":266.71816745655616},"flipX":true},"style":{"thickness":2}},{"id":"da627473150527144","data":[{"x":83.21840801102576,"y":164.75},{"x":72.34779189728174,"y":227.47693522906815}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da3046348742761984","data":[{"x":91.21840801102576,"y":163.75},{"x":155.21840801102576,"y":247.25}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da6317593217319599","data":[{"x":163.34779189728175,"y":200.21816745655616},{"x":162.84779189728175,"y":244.47693522906815}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da3756873069415476","data":[{"x":248.84779189728175,"y":184.21816745655616},{"x":173.21840801102576,"y":251.75}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da1221654260619609","data":[{"x":151.72717578353775,"y":255.59755134281215},{"x":83.71840801102576,"y":241.25}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"dl9028792956538128","linkedId":"de5735043202187369"},{"id":"dl02411659043776737","linkedId":"de5118042979405351"},{"id":"dl7569495592190025","linkedId":"de1323254760299537"},{"id":"dl6032540041583871","linkedId":"de9019134361407426"},{"id":"dl9209717141589551","linkedId":"de31837363099354143"},{"id":"dl5601841205536202","linkedId":"de03212568133696059"},{"id":"dl7623732870090665","linkedId":"de7463208319227395"},{"id":"dl6013371747462843","linkedId":"de7875117653412074"},{"id":"dl6153696511522506","linkedId":"de8836686111401333"},{"id":"dl6134891032497409","linkedId":"de4944384494771481"}]},{"id":"dg9037458531064226","entities":[{"id":"ds11734681479383213","type":"polygon-curve","data":[{"p1":{"x":496.06030805687203,"y":66.5},"p2":{"x":536.3936413902054,"y":151.33333333333334},"cp":{"dx":32.00000000000003,"dy":-8.666666666666657},"cp2":{"dx":-4,"dy":-27}},{"p1":{"x":536.3936413902054,"y":151.33333333333334},"p2":{"x":523.060308056872,"y":263.5},"cp":{"dx":4,"dy":27},"cp2":{"dx":36,"dy":-10}},{"p1":{"x":523.060308056872,"y":263.5},"p2":{"x":430.06030805687203,"y":263},"cp":{"dx":-36,"dy":10},"cp2":{"dx":33,"dy":6}},{"p1":{"x":430.06030805687203,"y":263},"p2":{"x":496.06030805687203,"y":66.5},"cp":{"dx":-33,"dy":-6},"cp2":{"dx":-32.00000000000003,"dy":8.666666666666657}}],"style":{"fillColor":[74,144,226,0.3],"strokeColor":"none"}},{"id":"ds5590765623889005","type":"polygon-curve","data":[{"p1":{"x":566.810308056872,"y":81.75},"p2":{"x":631.810308056872,"y":131.25},"cp":{"dx":23.5,"dy":-29.5},"cp2":{"dx":-15.5,"dy":-37.5}},{"p1":{"x":631.810308056872,"y":131.25},"p2":{"x":625.310308056872,"y":220.25},"cp":{"dx":15.5,"dy":37.5},"cp2":{"dx":25.5,"dy":-38}},{"p1":{"x":625.310308056872,"y":220.25},"p2":{"x":560.310308056872,"y":256.75},"cp":{"dx":-25.5,"dy":38},"cp2":{"dx":18.5,"dy":19.5}},{"p1":{"x":560.310308056872,"y":256.75},"p2":{"x":566.810308056872,"y":81.75},"cp":{"dx":-18.5,"dy":-19.5},"cp2":{"dx":-23.5,"dy":29.5}}],"style":{"strokeColor":"none","fillColor":[208,2,27,0.3]}},{"id":"dp9948128982097342","type":"circle","data":{"p1":{"x":525.319075829384,"y":29.476935229068133},"p2":{"x":547.560308056872,"y":51.71816745655617},"flipX":true},"style":{"thickness":2}},{"id":"dp2511682743188599","type":"circle","data":{"p1":{"x":487.819075829384,"y":75.47693522906813},"p2":{"x":510.06030805687203,"y":97.71816745655617},"flipX":true},"style":{"thickness":2}},{"id":"da6986992416154134","data":[{"x":528.560308056872,"y":48},{"x":506.06030805687203,"y":77.5}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"dp10931133172345242","type":"circle","data":{"p1":{"x":574.819075829384,"y":80.97693522906813},"p2":{"x":597.060308056872,"y":103.21816745655617},"flipX":true},"style":{"thickness":2}},{"id":"da3217262008599182","data":[{"x":546.310308056872,"y":46.5},{"x":579.810308056872,"y":82.5}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da21460956304500267","data":[{"x":510.06030805687203,"y":86.59755134281215},{"x":574.819075829384,"y":92.09755134281215}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"dp5291645395834803","type":"circle","data":{"p1":{"x":450.319075829384,"y":144.97693522906815},"p2":{"x":472.56030805687203,"y":167.21816745655616},"flipX":true},"style":{"thickness":2}},{"id":"dp27654504370737376","type":"circle","data":{"p1":{"x":612.819075829384,"y":163.97693522906815},"p2":{"x":635.060308056872,"y":186.21816745655616},"flipX":true},"style":{"thickness":2}},{"id":"da2737799322547254","data":[{"x":466.31030805687203,"y":145.75},{"x":494.31030805687203,"y":97.25}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da39496331184914135","data":[{"x":592.310308056872,"y":100.75},{"x":620.810308056872,"y":164.25}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"dp7992067260547593","type":"circle","data":{"p1":{"x":509.31907582938396,"y":171.3102685624015},"p2":{"x":531.560308056872,"y":193.5515007898895},"flipX":true},"style":{"thickness":2}},{"id":"da9507495588051804","data":[{"x":472.06030805687203,"y":159},{"x":509.06030805687203,"y":179}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da1437265999698425","data":[{"x":612.819075829384,"y":175.09755134281215},{"x":531.560308056872,"y":182.4308846761455}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da4730738022847163","data":[{"x":579.060308056872,"y":101.25},{"x":523.060308056872,"y":171.25}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"dp6361941094758832","type":"circle","data":{"p1":{"x":436.319075829384,"y":229.47693522906815},"p2":{"x":458.56030805687203,"y":251.71816745655616},"flipX":true},"style":{"thickness":2}},{"id":"dp5769509414488139","type":"circle","data":{"p1":{"x":509.819075829384,"y":228.47693522906815},"p2":{"x":532.060308056872,"y":250.71816745655616},"flipX":true},"style":{"thickness":2}},{"id":"da25179081461799835","data":[{"x":458.31030805687203,"y":166.75},{"x":447.439691943128,"y":229.47693522906815}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da5822604032168714","data":[{"x":468.06030805687203,"y":165},{"x":514.060308056872,"y":230}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da06301161896355345","data":[{"x":520.439691943128,"y":193.5515007898895},{"x":520.9396919431281,"y":228.47693522906815}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da5257509964164879","data":[{"x":617.060308056872,"y":184.5},{"x":532.060308056872,"y":236}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da5760415819261551","data":[{"x":509.819075829384,"y":239.59755134281215},{"x":458.56030805687203,"y":240.59755134281215}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"dp6445923675289842","type":"circle","data":{"p1":{"x":553.9857424960506,"y":139.31026856240146},"p2":{"x":576.2269747235388,"y":161.55150078988947},"flipX":true},"style":{"thickness":2}},{"id":"dp9063829027506483","type":"circle","data":{"p1":{"x":563.819075829384,"y":233.879383886256},"p2":{"x":586.060308056872,"y":256.120616113744},"flipX":true},"style":{"thickness":2}},{"id":"da2157463404431934","data":[{"x":472.06030805687203,"y":151.75},{"x":553.9857424960506,"y":150.43088467614547}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da8848573256800494","data":[{"x":471.06030805687203,"y":162.25},{"x":564.560308056872,"y":239.25}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da998567481582201","data":[{"x":565.1063586097947,"y":161.55150078988947},{"x":574.939691943128,"y":233.879383886256}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da6360072791381837","data":[{"x":623.939691943128,"y":186.21816745655616},{"x":583.060308056872,"y":236.75}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da8012918905917032","data":[{"x":614.560308056872,"y":168.75},{"x":576.060308056872,"y":153.75}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da8957443883402796","data":[{"x":585.939691943128,"y":103.21816745655617},{"x":570.560308056872,"y":139.75}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"dl39930868330505476","linkedId":"de3377854219142531"},{"id":"dl5685935255434509","linkedId":"de9746836771703111"},{"id":"dl3611342514731233","linkedId":"de7058376200954342"},{"id":"dl5726364103106318","linkedId":"de10690752715792029"},{"id":"dl5160035243965109","linkedId":"de3042818168372794"},{"id":"dl7021802241262947","linkedId":"de0849863605010528"},{"id":"dl6444658726131196","linkedId":"de061258972971343084"},{"id":"dl18893064902735235","linkedId":"de5679455674005585"},{"id":"dl5487531539350314","linkedId":"de9216647693979059"},{"id":"dl3336750163238349","linkedId":"de5471652702069676"},{"id":"dl4594374506513228","linkedId":"de6254772879152124"},{"id":"dl13952756081935225","linkedId":"de7724690333940571"}]},{"id":"dp5641002620887252","type":"right-arrow","data":{"p1":{"x":300,"y":155.97693522906815},"p2":{"x":392,"y":187.5},"arrowPercentage":0.6956521739130435,"sizePercentage":0.5407510235991501},"style":{"strokeColor":"none","fillColor":[155,155,155,1]}},{"id":"dg9347311456990142","entities":[{"id":"ds6820478388967135","type":"polygon-curve","data":[{"p1":{"x":496.0603080568721,"y":418},"p2":{"x":536.3936413902054,"y":502.83333333333337},"cp":{"dx":32.00000000000003,"dy":-8.666666666666657},"cp2":{"dx":-4,"dy":-27}},{"p1":{"x":536.3936413902054,"y":502.83333333333337},"p2":{"x":523.0603080568721,"y":615},"cp":{"dx":4,"dy":27},"cp2":{"dx":36,"dy":-10}},{"p1":{"x":523.0603080568721,"y":615},"p2":{"x":430.0603080568721,"y":614.5},"cp":{"dx":-36,"dy":10},"cp2":{"dx":33,"dy":6}},{"p1":{"x":430.0603080568721,"y":614.5},"p2":{"x":496.0603080568721,"y":418},"cp":{"dx":-33,"dy":-6},"cp2":{"dx":-32.00000000000003,"dy":8.666666666666657}}],"style":{"fillColor":[74,144,226,0.3],"strokeColor":"none"}},{"id":"ds0876193766431137","type":"polygon-curve","data":[{"p1":{"x":566.8103080568721,"y":433.25},"p2":{"x":631.8103080568721,"y":482.75},"cp":{"dx":23.5,"dy":-29.5},"cp2":{"dx":-15.5,"dy":-37.5}},{"p1":{"x":631.8103080568721,"y":482.75},"p2":{"x":625.3103080568721,"y":571.75},"cp":{"dx":15.5,"dy":37.5},"cp2":{"dx":25.5,"dy":-38}},{"p1":{"x":625.3103080568721,"y":571.75},"p2":{"x":560.3103080568721,"y":608.25},"cp":{"dx":-25.5,"dy":38},"cp2":{"dx":18.5,"dy":19.5}},{"p1":{"x":560.3103080568721,"y":608.25},"p2":{"x":566.8103080568721,"y":433.25},"cp":{"dx":-18.5,"dy":-19.5},"cp2":{"dx":-23.5,"dy":29.5}}],"style":{"strokeColor":"none","fillColor":[208,2,27,0.3]}},{"id":"dp6815962896395329","type":"circle","data":{"p1":{"x":525.319075829384,"y":380.97693522906815},"p2":{"x":547.5603080568721,"y":403.21816745655616},"flipX":true},"style":{"thickness":2}},{"id":"dp036774241120755446","type":"circle","data":{"p1":{"x":487.8190758293841,"y":426.97693522906815},"p2":{"x":510.0603080568721,"y":449.21816745655616},"flipX":true},"style":{"thickness":2}},{"id":"da9837849572324335","data":[{"x":528.5603080568721,"y":399.5},{"x":506.0603080568721,"y":429}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"dp4600145255402004","type":"circle","data":{"p1":{"x":574.819075829384,"y":432.47693522906815},"p2":{"x":597.0603080568721,"y":454.71816745655616},"flipX":true},"style":{"thickness":2}},{"id":"da8881068738417672","data":[{"x":546.3103080568721,"y":398},{"x":579.8103080568721,"y":434}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da6616177855884817","data":[{"x":606.75,"y":409.5},{"x":591.25,"y":433.5}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"dp8755588131635565","type":"circle","data":{"p1":{"x":450.3190758293841,"y":496.47693522906815},"p2":{"x":472.5603080568721,"y":518.7181674565561},"flipX":true},"style":{"thickness":2}},{"id":"dp655673614996505","type":"circle","data":{"p1":{"x":612.819075829384,"y":515.4769352290682},"p2":{"x":635.0603080568721,"y":537.7181674565561},"flipX":true},"style":{"thickness":2}},{"id":"da8362363064317184","data":[{"x":466.3103080568721,"y":497.25},{"x":494.3103080568721,"y":448.75}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da7870859767861258","data":[{"x":592.3103080568721,"y":452.25},{"x":620.8103080568721,"y":515.75}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"dp8185485372696937","type":"circle","data":{"p1":{"x":509.319075829384,"y":522.8102685624015},"p2":{"x":531.5603080568721,"y":545.0515007898895},"flipX":true},"style":{"thickness":2}},{"id":"da6384058872291676","data":[{"x":472.0603080568721,"y":510.5},{"x":509.0603080568721,"y":530.5}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da10277872191631854","data":[{"x":418.75,"y":553.25},{"x":511.75,"y":540.75}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da2498124273602984","data":[{"x":425.0603080568721,"y":524.5975513428122},{"x":509.319075829384,"y":533.9308846761455}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"dp9896404561095602","type":"circle","data":{"p1":{"x":436.3190758293841,"y":580.9769352290682},"p2":{"x":458.5603080568721,"y":603.2181674565561},"flipX":true},"style":{"thickness":2}},{"id":"dp5987718533212627","type":"circle","data":{"p1":{"x":509.8190758293841,"y":579.9769352290682},"p2":{"x":532.0603080568721,"y":602.2181674565561},"flipX":true},"style":{"thickness":2}},{"id":"da8664331109588541","data":[{"x":458.3103080568721,"y":518.25},{"x":447.4396919431281,"y":580.9769352290682}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da925070125767582","data":[{"x":468.0603080568721,"y":516.5},{"x":514.0603080568721,"y":581.5}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da5371111299026543","data":[{"x":520.4396919431281,"y":545.0515007898895},{"x":520.9396919431281,"y":579.9769352290682}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da05570368984594487","data":[{"x":419.25,"y":560.75},{"x":510.25,"y":585.75}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da34722863097204004","data":[{"x":509.8190758293841,"y":591.0975513428122},{"x":458.5603080568721,"y":592.0975513428122}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"dp7747127492672876","type":"circle","data":{"p1":{"x":553.9857424960508,"y":490.81026856240146},"p2":{"x":576.2269747235389,"y":513.0515007898895},"flipX":true},"style":{"thickness":2}},{"id":"dp9135559161348474","type":"circle","data":{"p1":{"x":563.819075829384,"y":585.3793838862559},"p2":{"x":586.0603080568721,"y":607.6206161137441},"flipX":true},"style":{"thickness":2}},{"id":"da5551288880263132","data":[{"x":629,"y":575.75},{"x":572,"y":511.25}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da3681731491861491","data":[{"x":626,"y":590.25},{"x":586.0603080568721,"y":596.5}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da32399195557307814","data":[{"x":565.1063586097948,"y":513.0515007898895},{"x":574.9396919431281,"y":585.3793838862559}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da929792628957095","data":[{"x":623.9396919431281,"y":537.7181674565561},{"x":583.0603080568721,"y":588.25}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da7109910300716575","data":[{"x":614.5603080568721,"y":520.25},{"x":576.0603080568721,"y":505.25}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da28113175928056755","data":[{"x":585.9396919431281,"y":454.71816745655616},{"x":570.5603080568721,"y":491.25}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"dp9914981183417868","type":"circle","data":{"p1":{"x":599.319075829384,"y":387.97693522906815},"p2":{"x":621.5603080568721,"y":410.21816745655616},"flipX":true},"style":{"thickness":2}},{"id":"dp14480133318917998","type":"circle","data":{"p1":{"x":402.8190758293841,"y":513.4769352290682},"p2":{"x":425.0603080568721,"y":535.7181674565561},"flipX":true},"style":{"thickness":2}},{"id":"dp8998449140330051","type":"circle","data":{"p1":{"x":397.3190758293841,"y":546.9769352290682},"p2":{"x":419.5603080568721,"y":569.2181674565561},"flipX":true},"style":{"thickness":2}},{"id":"dp4360324949125065","type":"circle","data":{"p1":{"x":624.819075829384,"y":573.9769352290682},"p2":{"x":647.0603080568721,"y":596.2181674565561},"flipX":true},"style":{"thickness":2}},{"id":"dl2954501872797144","linkedId":"de8638865150933372"},{"id":"dl5362110062676295","linkedId":"de2908296551539664"},{"id":"dl6973577069037016","linkedId":"de04805762837656724"},{"id":"dl8880007083481107","linkedId":"de588362433308294"},{"id":"dl956461148817658","linkedId":"de45201336284664273"},{"id":"dl29944173765873705","linkedId":"de5435926234374486"},{"id":"dl26880502544132523","linkedId":"de03143524405385634"},{"id":"dl2817069591940813","linkedId":"de0859208809459453"},{"id":"dl9247040601712","linkedId":"de030069601839159077"},{"id":"dl962081113332186","linkedId":"de32525387455748045"},{"id":"dl19369942537782925","linkedId":"de3192619109950017"},{"id":"dl680019734678101","linkedId":"de7184182056565798"},{"id":"dl7566240272460596","linkedId":"de3411185373599821"},{"id":"dl7976307438628529","linkedId":"de5839989731199371"},{"id":"dl9035545488818915","linkedId":"de6695614353438804"},{"id":"dl1354908988892234","linkedId":"de17654312581252363"}]},{"id":"dp7797432637286774","type":"right-arrow","data":{"p1":{"x":498.88076619273295,"y":304.85770142180115},"p2":{"x":567.119233807267,"y":336.38076619273295},"arrowPercentage":0.6956521739130435,"sizePercentage":0.5407510235991501,"rotation":90},"style":{"strokeColor":"none","fillColor":[155,155,155,1]}},{"id":"ds851871903110963","type":"polygon-curve","data":[{"p1":{"x":116.12061611374398,"y":418},"p2":{"x":156.4539494470773,"y":502.83333333333337},"cp":{"dx":32.00000000000003,"dy":-8.666666666666657},"cp2":{"dx":-4,"dy":-27}},{"p1":{"x":156.4539494470773,"y":502.83333333333337},"p2":{"x":143.12061611374398,"y":615},"cp":{"dx":4,"dy":27},"cp2":{"dx":36,"dy":-10}},{"p1":{"x":143.12061611374398,"y":615},"p2":{"x":50.12061611374398,"y":614.5},"cp":{"dx":-36,"dy":10},"cp2":{"dx":33,"dy":6}},{"p1":{"x":50.12061611374398,"y":614.5},"p2":{"x":116.12061611374398,"y":418},"cp":{"dx":-33,"dy":-6},"cp2":{"dx":-32.00000000000003,"dy":8.666666666666657}}],"style":{"fillColor":[74,144,226,0.3],"strokeColor":"none"}},{"id":"ds5474486965849934","type":"polygon-curve","data":[{"p1":{"x":186.87061611374403,"y":433.25},"p2":{"x":251.87061611374403,"y":482.75},"cp":{"dx":23.5,"dy":-29.5},"cp2":{"dx":-15.5,"dy":-37.5}},{"p1":{"x":251.87061611374403,"y":482.75},"p2":{"x":245.37061611374403,"y":571.75},"cp":{"dx":15.5,"dy":37.5},"cp2":{"dx":25.5,"dy":-38}},{"p1":{"x":245.37061611374403,"y":571.75},"p2":{"x":180.37061611374403,"y":608.25},"cp":{"dx":-25.5,"dy":38},"cp2":{"dx":18.5,"dy":19.5}},{"p1":{"x":180.37061611374403,"y":608.25},"p2":{"x":186.87061611374403,"y":433.25},"cp":{"dx":-18.5,"dy":-19.5},"cp2":{"dx":-23.5,"dy":29.5}}],"style":{"strokeColor":"none","fillColor":[208,2,27,0.3]}},{"id":"dp4436972325926303","type":"circle","data":{"p1":{"x":119.87938388625591,"y":372.47693522906815},"p2":{"x":142.12061611374403,"y":394.71816745655616},"flipX":true},"style":{"thickness":2}},{"id":"dp41732723610441735","type":"circle","data":{"p1":{"x":107.87938388625597,"y":426.97693522906815},"p2":{"x":130.12061611374398,"y":449.21816745655616},"flipX":true},"style":{"thickness":2}},{"id":"da3812629556517646","data":[{"x":128,"y":394.5},{"x":118.99999999999997,"y":426.97693522906815}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"dp8001106714865494","type":"circle","data":{"p1":{"x":194.8793838862559,"y":432.47693522906815},"p2":{"x":217.12061611374403,"y":454.71816745655616},"flipX":true},"style":{"thickness":2}},{"id":"da7035437940309908","data":[{"x":173,"y":393.5},{"x":199.87061611374403,"y":434}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da3626864124494753","data":[{"x":226.8103080568719,"y":409.5},{"x":211.3103080568719,"y":433.5}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"dp053638326690359506","type":"circle","data":{"p1":{"x":70.37938388625597,"y":496.47693522906815},"p2":{"x":92.62061611374398,"y":518.7181674565561},"flipX":true},"style":{"thickness":2}},{"id":"dp24290483412383357","type":"circle","data":{"p1":{"x":232.8793838862559,"y":515.4769352290682},"p2":{"x":255.12061611374406,"y":537.7181674565561},"flipX":true},"style":{"thickness":2}},{"id":"da3619860928724281","data":[{"x":86.37061611374398,"y":497.25},{"x":114.37061611374398,"y":448.75}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da43113232257494816","data":[{"x":212.37061611374403,"y":452.25},{"x":240.87061611374403,"y":515.75}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"dp5672939586504162","type":"circle","data":{"p1":{"x":129.3793838862559,"y":522.8102685624015},"p2":{"x":151.62061611374403,"y":545.0515007898895},"flipX":true},"style":{"thickness":2}},{"id":"da6057330837751351","data":[{"x":92.12061611374398,"y":510.5},{"x":129.12061611374398,"y":530.5}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da5389989036206069","data":[{"x":38.81030805687189,"y":553.25},{"x":131.8103080568719,"y":540.75}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da8650024903950211","data":[{"x":45.12061611374398,"y":524.5975513428122},{"x":129.3793838862559,"y":533.9308846761455}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"dp9227064516113586","type":"circle","data":{"p1":{"x":56.379383886255965,"y":580.9769352290682},"p2":{"x":78.62061611374398,"y":603.2181674565561},"flipX":true},"style":{"thickness":2}},{"id":"dp3187860701534553","type":"circle","data":{"p1":{"x":129.87938388625597,"y":579.9769352290682},"p2":{"x":152.12061611374403,"y":602.2181674565561},"flipX":true},"style":{"thickness":2}},{"id":"da7162956050359766","data":[{"x":78.37061611374398,"y":518.25},{"x":67.49999999999997,"y":580.9769352290682}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da8491180239278711","data":[{"x":88.12061611374398,"y":516.5},{"x":134.12061611374398,"y":581.5}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da8570737491426299","data":[{"x":140.49999999999991,"y":545.0515007898895},{"x":140.99999999999991,"y":579.9769352290682}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da03165174004372884","data":[{"x":39.31030805687189,"y":560.75},{"x":130.3103080568719,"y":585.75}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da36347467382392895","data":[{"x":129.87938388625597,"y":591.0975513428122},{"x":78.62061611374398,"y":592.0975513428122}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"dp14831035625224898","type":"circle","data":{"p1":{"x":174.04605055292265,"y":490.81026856240146},"p2":{"x":196.28728278041078,"y":513.0515007898895},"flipX":true},"style":{"thickness":2}},{"id":"dp49962866637464387","type":"circle","data":{"p1":{"x":183.8793838862559,"y":585.3793838862559},"p2":{"x":206.12061611374403,"y":607.6206161137441},"flipX":true},"style":{"thickness":2}},{"id":"da4890793744205246","data":[{"x":249.0603080568719,"y":575.75},{"x":192.0603080568719,"y":511.25}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da7353756123092572","data":[{"x":246.0603080568719,"y":590.25},{"x":206.12061611374403,"y":596.5}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da060523248299078736","data":[{"x":185.1666666666667,"y":513.0515007898895},{"x":194.99999999999997,"y":585.3793838862559}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da9572926499341807","data":[{"x":243.99999999999997,"y":537.7181674565561},{"x":203.12061611374403,"y":588.25}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da15040543681006802","data":[{"x":234.62061611374403,"y":520.25},{"x":196.12061611374403,"y":505.25}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"da05786476901546256","data":[{"x":205.99999999999997,"y":454.71816745655616},{"x":190.62061611374403,"y":491.25}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"headScale":0.6,"style":{"thickness":2}},{"id":"dp8640583704149731","type":"circle","data":{"p1":{"x":219.3793838862559,"y":387.97693522906815},"p2":{"x":241.62061611374403,"y":410.21816745655616},"flipX":true},"style":{"thickness":2}},{"id":"dp7690880405721836","type":"circle","data":{"p1":{"x":22.879383886255965,"y":513.4769352290682},"p2":{"x":45.12061611374398,"y":535.7181674565561},"flipX":true},"style":{"thickness":2}},{"id":"dp7926329165819135","type":"circle","data":{"p1":{"x":17.379383886255965,"y":546.9769352290682},"p2":{"x":39.62061611374398,"y":569.2181674565561},"flipX":true},"style":{"thickness":2}},{"id":"dp8903694068507191","type":"circle","data":{"p1":{"x":244.8793838862559,"y":573.9769352290682},"p2":{"x":267.12061611374406,"y":596.2181674565561},"flipX":true},"style":{"thickness":2}},{"id":"dp8344232129518299","type":"right-arrow","data":{"p1":{"x":286.6666666666667,"y":487.97693522906826},"p2":{"x":378.6666666666667,"y":519.5},"arrowPercentage":0.6956521739130435,"sizePercentage":0.5407510235991501,"rotation":180},"style":{"strokeColor":"none","fillColor":[155,155,155,1]}},{"id":"dp8440737755198686","type":"circle","data":{"p1":{"x":157.3793838862559,"y":371.97693522906815},"p2":{"x":179.62061611374403,"y":394.21816745655616},"flipX":true},"style":{"thickness":2}}],"settings":{"grid":true,"diagramHeight":651},"id":"n0.6768416598589522"}],"id":"n0.22972741688823972"}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":521,"delayRenderCache":{"av":521,"map":{}}}

==> figs/docs/d856a46e-5d9a-48aa-ad7d-b2c514a6fa4f <==
{"id":"r0.34972806533295375","lines":[{"blocks":[{"text":"\\diagram","type":"composite","elements":{},"connections":[],"intersections":{"id":"di018738070182718003","items":[],"style":{}},"shapes":[{"id":"dp5595920893313384","type":"ellipse","data":{"p1":{"x":135.29440727711722,"y":186.99030499710676},"p2":{"x":168.71968329997304,"y":220.4155810199626}},"style":{"fillColor":"none"}},{"id":"dp5483194175802013","type":"ellipse","data":{"p1":{"x":174.25037935120338,"y":90.42576935089271},"p2":{"x":207.6756553740592,"y":123.85104537374855}},"style":{"fillColor":"none"}},{"id":"dp8514133519092584","type":"ellipse","data":{"p1":{"x":185.96670401123384,"y":189.40727418009203},"p2":{"x":219.3919800340896,"y":222.83255020294786},"rotation":12.59},"style":{"fillColor":"none"}},{"id":"dp09725013994802012","type":"ellipse","data":{"p1":{"x":265.7964198266168,"y":104.81157571131483},"p2":{"x":299.2216958494729,"y":138.2368517341706},"rotation":11.34},"style":{"fillColor":[255,255,255,1]}},{"id":"dp3830620809519649","type":"ellipse","data":{"p1":{"x":260.5652175137361,"y":185.2413112718566},"p2":{"x":293.9904935365919,"y":218.66658729471243},"rotation":1.24},"style":{"fillColor":"none"}},{"id":"dp4389166881626114","type":"ellipse","data":{"p1":{"x":354.72685914559,"y":180.33705910353098},"p2":{"x":388.1521351684457,"y":213.7623351263867},"rotation":312.14},"style":{"fillColor":"none"}},{"id":"dp6323885562173717","type":"ellipse","data":{"p1":{"x":350.80345741092947,"y":79.96336472513114},"p2":{"x":384.22873343378535,"y":113.38864074798697}},"style":{"fillColor":"none"}},{"id":"dp44188316196919253","type":"ellipse","data":{"p1":{"x":432.349497886343,"y":115.48105741170646},"p2":{"x":465.77477390919876,"y":148.90633343456227}},"style":{"fillColor":"none"}},{"id":"da973947306017195","data":[{"x":156.33333333333334,"y":188},{"x":179,"y":118.66666666666667}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da5678832648178884","data":[{"x":190.96301736263126,"y":123.85104537374855},{"x":201.66666666666666,"y":189.33333333333331}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da9980161894520267","data":[{"x":207.6756553740592,"y":107.13840736232062},{"x":266.1226902403077,"y":118.23799610169955}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da23464194780621406","data":[{"x":279.2228402170017,"y":137.91058132047988},{"x":277.639523585014,"y":185.24522504965404}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da7001095341229502","data":[{"x":295.29829411481217,"y":111.25897098062337},{"x":350.80345741092947,"y":96.67600273655906}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da9074907784707391","data":[{"x":367.51609542235735,"y":113.38864074798697},{"x":371.8046279406934,"y":180.89935177084863}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da3093235587089789","data":[{"x":386.75,"y":190.5},{"x":438.3333333333333,"y":144.66666666666669}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da27378080850877873","data":[{"x":296.25,"y":131.16666666666669},{"x":359.04694881946455,"y":185.83644535632817}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}}],"settings":{"grid":true},"id":"n0.932893615456784"}],"id":"n0.11142037881430733"}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":7,"delayRenderCache":{"av":7,"map":{}}}

==> figs/docs/f458c498-f74c-4c19-be54-4ee1550cd8da <==
{"id":"r0.050871064024779145","lines":[{"id":"n0.952291796451851","blocks":[]},{"id":"n0.6536761371441988","blocks":[{"id":"n0.4664334835344386","text":"\\diagram","type":"composite","elements":{"de868514552120158":{"id":"de868514552120158","lines":[{"id":"n0.7987499443991857","blocks":[{"id":"n0.243405749114191","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.3381627961485085","lines":[{"id":"n0.7088049490303754","blocks":[{"id":"n0.09668097704103973","text":"i"}]}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"}}]}],"shape":{"data":{"p":{"x":260.66666666666663,"y":39.000000000000014}},"anchor":"left-top"},"isTextMode":true},"de930759547802749":{"id":"de930759547802749","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.5217457767328295","text":"j"}],"id":"n0.4683829264401853"}],"id":"n0.9185195730806524"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.7098444893417251"}],"id":"n0.6518291198920956"}],"shape":{"data":{"p":{"x":414,"y":264.3333333333333}},"anchor":"left-top"},"isTextMode":true},"de08901392316798229":{"id":"de08901392316798229","lines":[{"id":"n0.3844804168047755","blocks":[{"id":"n0.4172598195881463","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.3564762211179968","lines":[{"id":"n0.7330555367408589","blocks":[{"id":"n0.8652105188690826","text":"e"},{"id":"n0.08182675553148755","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.07007988175367763","lines":[{"id":"n0.8968250605176507","blocks":[{"id":"n0.7786912812082876","text":"1"}]}]}}}]}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"}}]}],"shape":{"data":{"p":{"x":192,"y":68.66666666666667}},"anchor":"left-top","style":{"textColor":[247,31,31,0.7],"strokeColor":[247,31,31,0.7]}},"isTextMode":true},"de8580282487537589":{"id":"de8580282487537589","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"e","id":"n0.14596208858085147"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.810801156379783","text":"0"}],"id":"n0.7974959438820612"}],"id":"n0.33986995934465214"}},"id":"n0.19881609116026322"}],"id":"n0.6292335645650926"}],"id":"n0.17848119058242595"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.7097014454397639"}],"id":"n0.8113094976574295"}],"shape":{"data":{"p":{"x":466.00000000000006,"y":202.00000000000003}},"anchor":"left-top","style":{"textColor":[70,114,191,0.7]}},"isTextMode":true}},"connections":[],"intersections":{"id":"di018738070182718003","items":[],"style":{}},"shapes":[{"id":"dp06408659454009968","type":"ellipse","data":{"p1":{"x":154.29440727711722,"y":200.3236383304401},"p2":{"x":187.71968329997304,"y":233.74891435329593}},"style":{"fillColor":"none"}},{"id":"dp15508359634159774","type":"ellipse","data":{"p1":{"x":193.25037935120338,"y":103.75910268422604},"p2":{"x":226.6756553740592,"y":137.18437870708186}},"style":{"fillColor":[247,31,31,1]}},{"id":"dp8097019890836532","type":"ellipse","data":{"p1":{"x":204.96670401123384,"y":202.74060751342537},"p2":{"x":238.3919800340896,"y":236.16588353628117},"rotation":12.59},"style":{"fillColor":"none"}},{"id":"dp4757669275034335","type":"ellipse","data":{"p1":{"x":284.7964198266168,"y":118.14490904464816},"p2":{"x":318.2216958494729,"y":151.57018506750393},"rotation":11.34},"style":{"fillColor":[255,255,255,1]}},{"id":"dp9187055951977288","type":"ellipse","data":{"p1":{"x":279.5652175137361,"y":198.57464460518992},"p2":{"x":312.9904935365919,"y":231.99992062804577},"rotation":1.24},"style":{"fillColor":[247,31,31,1]}},{"id":"dp21680508026957224","type":"ellipse","data":{"p1":{"x":373.72685914559,"y":193.6703924368643},"p2":{"x":407.1521351684457,"y":227.09566845972},"rotation":312.14},"style":{"fillColor":"none"}},{"id":"dp39295355389948394","type":"ellipse","data":{"p1":{"x":369.80345741092947,"y":93.29669805846447},"p2":{"x":403.22873343378535,"y":126.7219740813203}},"style":{"fillColor":"none"}},{"id":"dp4079796727614313","type":"ellipse","data":{"p1":{"x":451.349497886343,"y":128.8143907450398},"p2":{"x":484.77477390919876,"y":162.2396667678956}},"style":{"fillColor":[70,114,191,1]}},{"id":"da9300741244764887","data":[{"x":175.33333333333334,"y":201.33333333333334},{"x":198,"y":132}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da7263674163314402","data":[{"x":209.96301736263126,"y":137.18437870708186},{"x":220.66666666666666,"y":202.66666666666666}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da09089499085321284","data":[{"x":226.6756553740592,"y":120.47174069565395},{"x":285.1226902403077,"y":131.57132943503288}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da49174943306574437","data":[{"x":298.2228402170017,"y":151.2439146538132},{"x":296.639523585014,"y":198.57855838298735}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da4532159493604795","data":[{"x":314.29829411481217,"y":124.5923043139567},{"x":369.80345741092947,"y":110.00933606989238}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da7249309179969847","data":[{"x":386.51609542235735,"y":126.7219740813203},{"x":390.8046279406934,"y":194.23268510418194}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da11931863075143423","data":[{"x":406.49823487933577,"y":204.0411894408334},{"x":457.3333333333333,"y":158}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"dg16418477169893309","entities":[{"id":"dp2379444195445377","type":"doc-arc","data":{"p1":{"x":373.9385150374127,"y":193.50136724720377},"p2":{"x":407.3637910602688,"y":226.92664327005954},"rotation":68.87,"angle2":180,"angle1":0},"style":{"fillColor":[247,31,31,1]}},{"id":"da6507719950991051","data":[{"x":384.6264935223915,"y":194.62504291691712},{"x":396.67581257528997,"y":225.8029676003462}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"fillColor":[247,31,31,1]}}]},{"id":"dg36593882891554275","entities":[{"id":"dp041752381357595514","type":"doc-arc","data":{"p1":{"x":373.4385150374126,"y":193.75136724720372},"p2":{"x":406.8637910602687,"y":227.17664327005943},"rotation":248.87,"angle2":180,"angle1":0},"style":{"fillColor":[70,114,191,1]}},{"id":"da20455661826554605","data":[{"x":396.1758125752898,"y":226.05296760034608},{"x":384.12649352239146,"y":194.875042916917}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"fillColor":[70,114,191,1]}}],"data":{"rotation":180}},{"id":"da9489169839601992","data":[{"x":315.25,"y":144.5},{"x":378.04694881946455,"y":199.16977868966148}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"dg5652411428605313","entities":[{"id":"dp8654203585535216","type":"doc-arc","data":{"p1":{"x":285.271848370746,"y":118.08470058053712},"p2":{"x":318.6971243936021,"y":151.5099766033929},"rotation":68.87,"angle2":180,"angle1":0},"style":{"fillColor":[247,31,31,1]}},{"id":"da659743535265545","data":[{"x":295.9598268557248,"y":119.20837625025047},{"x":308.0091459086233,"y":150.38630093367954}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"fillColor":[247,31,31,1]}}]},{"id":"dg620070924902498","entities":[{"id":"dp5973364928269425","type":"doc-arc","data":{"p1":{"x":284.4385150374126,"y":118.25136724720372},"p2":{"x":317.8637910602687,"y":151.67664327005943},"rotation":248.87,"angle2":180,"angle1":0},"style":{"fillColor":[70,114,191,1]}},{"id":"da8183730653674541","data":[{"x":307.1758125752898,"y":150.55296760034608},{"x":295.12649352239146,"y":119.37504291691701}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"fillColor":[70,114,191,1]}}],"data":{"rotation":180}},{"id":"dg98400416948265","entities":[{"id":"dp1929183412233384","type":"doc-arc","data":{"p1":{"x":369.9385150374127,"y":92.83470058053709},"p2":{"x":403.3637910602688,"y":126.25997660339286},"rotation":68.87,"angle2":180,"angle1":0},"style":{"fillColor":[247,31,31,1]}},{"id":"da3196295031083498","data":[{"x":380.6264935223915,"y":93.95837625025044},{"x":392.67581257528997,"y":125.13630093367951}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"fillColor":[247,31,31,1]}}]},{"id":"dg9842661150192447","entities":[{"id":"dp6659296752512429","type":"doc-arc","data":{"p1":{"x":369.4385150374126,"y":93.08470058053703},"p2":{"x":402.8637910602687,"y":126.50997660339274},"rotation":248.87,"angle2":180,"angle1":0},"style":{"fillColor":[70,114,191,1]}},{"id":"da017615596299715985","data":[{"x":392.1758125752898,"y":125.3863009336794},{"x":380.12649352239146,"y":94.20837625025032}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"fillColor":[70,114,191,1]}}],"data":{"rotation":180}},{"id":"ds7766139750547119","type":"polygon-curve","data":[{"p1":{"x":281.75,"y":117.25},"p2":{"x":416.6666666666667,"y":96},"cp":{"dx":31.5,"dy":-25},"cp2":{"dx":3.3333333333333144,"dy":-30}},{"p1":{"x":416.6666666666667,"y":96},"p2":{"x":416.6666666666667,"y":160.66666666666666},"cp":{"dx":-3.3333333333333144,"dy":30},"cp2":{"dx":-9.333333333333371,"dy":-11.333333333333343}},{"p1":{"x":416.6666666666667,"y":160.66666666666666},"p2":{"x":493.33333333333337,"y":126},"cp":{"dx":9.333333333333371,"dy":11.333333333333343},"cp2":{"dx":-21.999999999999943,"dy":-52}},{"p1":{"x":493.33333333333337,"y":126},"p2":{"x":381.25,"y":237.75},"cp":{"dx":21.999999999999886,"dy":52},"cp2":{"dx":43,"dy":10}},{"p1":{"x":381.25,"y":237.75},"p2":{"x":281.75,"y":117.25},"cp":{"dx":-43,"dy":-10},"cp2":{"dx":-31.5,"dy":25}}],"style":{"strokeType":"--","strokeColor":[70,114,191,0.5],"thickness":2}},{"id":"ds6603486926868913","type":"polygon-curve","data":[{"p1":{"x":252,"y":176},"p2":{"x":180.66666666666666,"y":114},"cp":{"dx":-3.3333333333333712,"dy":-29.333333333333343},"cp2":{"dx":-18.666666666666686,"dy":50}},{"p1":{"x":180.66666666666666,"y":114},"p2":{"x":420.6666666666667,"y":79.33333333333333},"cp":{"dx":18.666666666666686,"dy":-50},"cp2":{"dx":-12.666666666666686,"dy":-12.666666666666671}},{"p1":{"x":420.6666666666667,"y":79.33333333333333},"p2":{"x":424,"y":220.66666666666669},"cp":{"dx":12.666666666666686,"dy":12.666666666666671},"cp2":{"dx":10,"dy":-29.333333333333314}},{"p1":{"x":424,"y":220.66666666666669},"p2":{"x":293.41704601787,"y":243.63840736232063},"cp":{"dx":-10,"dy":29.333333333333314},"cp2":{"dx":43,"dy":10}},{"p1":{"x":293.41704601787,"y":243.63840736232063},"p2":{"x":252,"y":176},"cp":{"dx":-43,"dy":-10},"cp2":{"dx":3.3333333333333712,"dy":29.333333333333343}}],"style":{"strokeType":"--","strokeColor":[247,31,31,0.5],"thickness":2}},{"id":"da709763924720936","data":[{"x":269.3333333333333,"y":62},{"x":294.6666666666667,"y":114.66666666666666}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"style":{"thickness":1,"strokeColor":[0,0,0,1]},"headScale":0.7},{"id":"da8285094661779413","data":[{"x":412,"y":269.3333333333333},{"x":398.6666666666667,"y":230.66666666666669}],"head":"fh>","tail":"no","shaft":"-","mVer":1,"style":{"thickness":1,"strokeColor":[0,0,0,1]},"headScale":0.7}],"settings":{"grid":true}}]},{"id":"n0.48440111412063036","blocks":[],"style":null}],"pageSettings":{"pageSize":{"width":677,"sizeUnit":"px"}},"___version":2,"version":2,"av":808,"delayRenderCache":{"av":808,"map":{}}}
